Gamma-ray spectral modulations of Galactic pulsars caused by photon-ALPs mixing

Well-motivated extensions of the standard model predict ultra-light and fundamental pseudo-scalar particles (e.g., axions or axion-like particles: ALPs). Similarly to the Primakoff-effect for axions, ALPs can mix with photons and consequently be searched for in laboratory experiments and with astrophysical observations. Here, we search for energy-dependent modulations of high-energy gamma-ray spectra that are tell-tale signatures of photon-ALPs mixing. To this end, we analyze the data recorded with the Fermi -LAT from Galactic pulsars selected to have a line of sight crossing spiral arms at a large pitch angle. The large-scale Galactic magnetic field traces the shape of spiral arms, such that a sizable photon-ALP conversion probability is expected for the sources considered. In nine years of Fermi -LAT data, we detect significant spectral features in the selected source-sample consistent with photon-ALPs oscillation with a combined statistical significance of 5.52 {\sigma} . Notably, sources with neighboring lines of sight share similar spectral features. From a common fit to all sources, we determine the most-likely parameters for mass $m_{a}$ and coupling $g_{a\gamma\gamma}$ to be $m_a=(3.6 \substack{+0.5_ \mathrm{stat.}\\-0.2_ \mathrm{stat.}}\pm 0.2_\mathrm{syst.} )$ neV and $g_{a\gamma\gamma}=(2.3\substack{+0.3_ \mathrm{stat.}\\-0.4_ \mathrm{stat.}}\pm 0.4_\mathrm{syst.})\times 10^{-10}$ GeV$^{-1}$. In the error budget, we consider instrumental effects, scaling of the adopted Galactic magnetic field model ($\pm~20~\%$), and uncertainties on the distance of individual sources. We note that an astrophysical interpretation of the detected modulation is not obvious.

==> unicode-math/um-doc-legacyfontdimen.tex <==
%%^^A%% um-doc-legacyfontdimen.tex -- part of UNICODE-MATH <wspr.io/unicode-math>

\section{Legacy \TeX\ font dimensions}

\centerline{%
\begin{tabular}[t]{@{}lp{4cm}@{}}
\toprule
\multicolumn{2}{@{}c@{}}{Text fonts} \\
\midrule
$\phi_1$ & slant per pt                \\
$\phi_2$ & interword space             \\
$\phi_3$ & interword stretch           \\
$\phi_4$ & interword shrink            \\
$\phi_5$ & x-height                    \\
$\phi_6$ & quad width                  \\
$\phi_7$ & extra space                 \\
$\phi_8$ & cap height (\XeTeX\ only)   \\
\bottomrule
\end{tabular}
\quad
\begin{tabular}[t]{@{}lp{4cm}@{}}
\toprule
\multicolumn{2}{@{}c@{}}{Maths font, \cs{fam}2} \\
\midrule
$\sigma_5$    & x height                    \\
$\sigma_6$    & quad                        \\
$\sigma_8$    & num1                        \\
$\sigma_9$    & num2                        \\
$\sigma_{10}$ & num3                        \\
$\sigma_{11}$ & denom1                      \\
$\sigma_{12}$ & denom2                      \\
$\sigma_{13}$ & sup1                        \\
$\sigma_{14}$ & sup2                        \\
$\sigma_{15}$ & sup3                        \\
$\sigma_{16}$ & sub1                        \\
$\sigma_{17}$ & sub2                        \\
$\sigma_{18}$ & sup drop                    \\
$\sigma_{19}$ & sub drop                    \\
$\sigma_{20}$ & delim1                      \\
$\sigma_{21}$ & delim2                      \\
$\sigma_{22}$ & axis height                 \\
\bottomrule
\end{tabular}
\quad
\begin{tabular}[t]{@{}lp{4cm}@{}}
\toprule
\multicolumn{2}{@{}c@{}}{Maths font, \cs{fam}3} \\
\midrule
$\xi_8$    & default rule thickness      \\
$\xi_9$    & big op spacing1             \\
$\xi_{10}$ & big op spacing2             \\
$\xi_{11}$ & big op spacing3             \\
$\xi_{12}$ & big op spacing4             \\
$\xi_{13}$ & big op spacing5             \\
\bottomrule
\end{tabular}
}

\endinput

% /©
%
% ------------------------------------------------
% The UNICODE-MATH package  <wspr.io/unicode-math>
% ------------------------------------------------
% This package is free software and may be redistributed and/or modified under
% the conditions of the LaTeX Project Public License, version 1.3c or higher
% (your choice): <http://www.latex-project.org/lppl/>.
% ------------------------------------------------
% Copyright 2006-2018  Will Robertson, LPPL "maintainer"
% Copyright 2010-2017  Philipp Stephani
% Copyright 2011-2017  Joseph Wright
% Copyright 2012-2015  Khaled Hosny
% ------------------------------------------------
%
% ©/


==> unicode-math/um-doc-main.tex <==
%%^^A%% um-doc-main.tex -- part of UNICODE-MATH <wspr.io/unicode-math>

\begin{abstract}
\noindent
This document describes the \pkg{unicode-math} package, which is
intended as an implementation of Unicode
maths for \LaTeX\ using the \XeTeX\ and Lua\TeX\ typesetting engines.
With this package, changing maths fonts is as easy as changing
text fonts --- and there are more and more maths fonts appearing now.
Maths input can also be simplified with Unicode since literal glyphs may be
entered instead of control sequences in your document source.

The package provides support for both \XeTeX\ and Lua\TeX. The different
engines provide differing levels of support for Unicode maths.
Please let us know of any troubles.

Alongside this documentation file, you should be able to find a minimal
example demonstrating the use of the package,
`\texttt{unimath-example.ltx}'. It also comes with a separate document,
`\texttt{unimath-symbols.pdf}',
containing a complete listing of mathematical symbols defined by
\pkg{unicode-math}, including comparisons between different fonts.

Finally, while the STIX fonts may be used with this package, accessing
their alphabets in their `private user area' is not yet supported.
(Of these additional alphabets there is a separate caligraphic design
distinct to the script design already included.)
Better support for the STIX fonts is planned for an upcoming revision of the
package after any problems have been ironed out with the initial version.

\end{abstract}

\newpage
\tableofcontents

\clearpage
\section{Introduction}

This document describes the \pkg{unicode-math} package, which is an
\emph{experimental} implementation of a macro to Unicode glyph encoding for
mathematical characters.

Users who desire to specify maths alphabets only (Greek and Latin letters,
and Arabic numerals)
may wish to use Andrew Moschou's \pkg{mathspec} package instead.
(\XeTeX-only at time of writing.)

\section{Acknowledgements}

Many thanks to:
Microsoft for developing the mathematics extension to OpenType as part of
Microsoft Office~2007;
Jonathan Kew for implementing Unicode math support in \XeTeX;
Taco Hoekwater for implementing Unicode math support in \LuaTeX;
Barbara Beeton for her prodigious effort compiling the definitive list of Unicode math
glyphs and their \LaTeX\ names (inventing them where necessary), and also
for her thoughtful replies to my sometimes incessant questions;
Philipp Stephani for extending the package to support \LuaTeX.
Ross Moore and Chris Rowley have provided moral and technical support
from the very early days with great insight into the issues we face trying
to extend and use \TeX\ in the future.
Apostolos Syropoulos, Joel Salomon, Khaled Hosny, and Mariusz Wodzicki
have been fantastic beta testers.

\section{Getting started}

Load \pkg{unicode-math} as a regular \LaTeX\ package. It should be loaded
after any other maths or font-related package in case it needs to overwrite
their definitions. Here's an example using the filename syntax to load the \TeX\ Gyre Pagella Math font: (this works for both \XeLaTeX\ and \LuaLaTeX)
\begin{Verbatim}
\usepackage{amsmath} % if desired
\usepackage{unicode-math}
\setmathfont{texgyrepagella-math.otf}
\end{Verbatim}

Once the package is loaded, traditional TFM-based maths fonts are no longer supported;
you can only switch to a different OpenType maths font using the \cs{setmathfont} command.
If you do not load an OpenType maths font before |\begin{document}|, Latin Modern Math will be loaded automatically.

\subsection{New commands}
\LaTeX, since the first version of \LaTeXe, changed the math group
selection from, say, |{\bf x}| to |\mathbf{x}|. It introduced commands
such as |\mathbf|, |\mathit|, |\mathsf|, |\mathtt| and |\mathcal|,
besides |\mathnormal|.  This was not only done to maintain the analogy
with |\textbf|, |\textit| and so on, but with the precise purpose of
loading the needed math groups (or math families) on demand and not
allocating them if not required by the document.

The introduction of \pkg{unicode-math} posed some problems fitting into this design. For
instance, there is a big difference between say |fit| as an operator
name in boldface type and the product of three boldface variables.
With legacy \TeX{} engines, |\mathbf{fit}| would use a ligature and
the same would happen with the input |\mathbf{f}\mathbf{i}\mathbf{t}|.
For the latter case, the user should probably use |\mathbf{f\/}|.

However, there is another important point from a \emph{conceptual}
point of view. A boldface variable name should be printed using the
\emph{math font}, whereas a boldface operator name should be printed
using the \emph{text font}. OpenType math fonts make this distinction
feasible, because they contain several math alphabets. Of course a
boldface text~`x' will not differ much (or at all) from a boldface
math~`x', but this is not the point: they \emph{should} be considered
different, because the former is |U+0078| in Unicode, the latter is
|U+1D431|.

It was clear that \emph{two} different commands are needed: one for using text boldface in math,
one for using math boldface. Only the document's author can know
whether one or the other is needed. The decision was to split off
the two meanings with a command like |\mathbf| for the boldface text font
in math and a command like |\symbf| (for the bold math font).

The five new symbol font commands that behave in this way are: \cs{symup},
\cs{symit}, \cs{symbf}, \cs{symsf}, and \cs{symit}.
These commands switch to single-letter mathematical symbols
(generally within the same OpenType font).

The legacy \cs{math..} commands switch to text fonts that are set up to behave
correctly in mathematics, and should be used for multi-letter identifiers.  These
could be denoted `text math alphabets'; further details are discussed
in \secref{mathselect}.  Additional similar `text math alphabet'
commands can be defined using the \cs{setmathfontface} command
discussed in \secref{mathselect}.  To control the behaviour of the
default text math alphabet commands to behave in a
backwards-compatible mode, see the package options described in
\secref{textmathlegacy}.


\begin{table}[t!]
  \topcaption{New \pkg{unicode-math} commands which overlap with legacy
  math commands. For new documents the \texttt{sym} versions are recommended.}
  \tablabel{symvsmath}
  \centering
  \begin{tabular}[t]{ll}
    \toprule
    Command & Synonym \\
    \midrule
    \cs{symnormal}  & \cs{mathnormal} \\
    \cs{symliteral} &                 \\
    &  \\
    &  \\
    &  \\
    \cs{symbb}      & \cs{mathbb}     \\
    \cs{symbbit}    & \cs{mathbbit}   \\
    \cs{symcal}     & \cs{mathcal}    \\
    \cs{symscr}     & \cs{mathscr}    \\
    \cs{symfrak}    & \cs{mathfrak}   \\
    \cs{symsfup}    & \cs{mathsfup}   \\
    \cs{symsfit}    & \cs{mathsfit}   \\
    \bottomrule
  \end{tabular}\qquad
  \begin{tabular}[t]{ll}
    \toprule
    Command & Synonym \\
    \midrule
    &  \\
    &  \\
    \cs{symbfsf}    & \cs{mathbfsf}   \\
    \cs{symbfup}    & \cs{mathbfup}   \\
    \cs{symbfit}    & \cs{mathbfit}   \\
    &  \\
    &  \\
    \cs{symbfcal}   & \cs{mathbfcal}  \\
    \cs{symbfscr}   & \cs{mathbfscr}  \\
    \cs{symbffrak}  & \cs{mathbffrak} \\
    \cs{symbfsfup}  & \cs{mathbfsfup} \\
    \cs{symbfsfit}  & \cs{mathbfsfit} \\
    \bottomrule
  \end{tabular}
\end{table}

In addition, \pkg{unicode-math} also provides a number of commands (such as
|\symcal|) to select specific `symbol alphabets' within the unicode
maths font, with usage, e.g., |$\symcal{G}$|${}\to\symcal{G}$.  The
full listing is shown in \Tabref{symvsmath}.  For backwards
compatibility, many of these are also defined with `familiar' synonyms
such as |\mathcal|.  However, where possible the `sym' prefix
commands should be preferred, as certain synonyms may become
deprecated in time. The |\symliteral| command is described in
\secref{math-style}.

Using the |\sym..| commands, the glyphs used to produce PDF output are Unicode-encoded,
and therefore a symbol such as $\symcal{G}$ can be copy-pasted into another programme
(or even into the source of another \LaTeX\ document using \pkg{unicode-math}) without
loss of meaning.
This is an important aspect of Unicode mathematics, but the \pkg{unicode-math} package
is not `pure' in the sense that the package also provides other mechanisms to change
the fonts used in the PDF output; the philosophy of the package is to provide mechanisms
for technical authors to invent and experiment with new syntaxes for their work.


\subsection{Package options}
Package options may be set when the package as loaded or at any later
stage with the \cs{unimathsetup} command. Therefore, the following two
examples are equivalent:
\begin{Verbatim}
\usepackage[math-style=TeX]{unicode-math}
% OR
\usepackage{unicode-math}
\unimathsetup{math-style=TeX}
\end{Verbatim}
Note, however, that some package options affects how maths is initialised
and changing an option such as |math-style| will not take effect until a
new maths font is set up.

Package options may \emph{also} be used when declaring new maths fonts,
passed via options to the \cs{setmathfont} command.
Therefore, the following two examples are equivalent:
\begin{Verbatim}
\unimathsetup{math-style=TeX}
\setmathfont{texgyrepagella-math.otf}
% OR
\setmathfont{texgyrepagella-math.otf}[math-style=TeX]
\end{Verbatim}

A summary list of package options is shown in \tabref{pkgopt}.
See following sections for more information.

\begin{table}\centering
  \topcaption{Package options.}
  \tablabel{pkgopt}
  \begin{tabular}{lll}
    \toprule
    Option & Description & See\dots \\
    \midrule
    |math-style| & Style of letters & \secref*{math-style} \\
    |bold-style| & Style of bold letters & \secref*{bold-style} \\
    |sans-style| & Style of sans serif letters & \secref*{sans-style} \\
    |nabla|      & Style of the nabla symbol & \secref*{nabla} \\
    |partial|    & Style of the partial symbol & \secref*{partial} \\
    |colon| & Behaviour of \cs{colon} & \secref*{colon} \\
    |slash-delimiter| & Glyph to use for `stretchy' slash & \secref*{slash-delimiter} \\
    \bottomrule
  \end{tabular}
\end{table}


\section{Unicode maths font setup}

In the ideal case, a single Unicode font will contain all maths glyphs we
need. The file |unicode-math-table.tex| (based on Barbara Beeton's \STIX\ table)
provides the mapping between Unicode
maths glyphs and macro names (all 3298 — or however many — of them!). A
single command
\codeline{\cmd\setmathfont\marg{font name}\oarg{font features}}
implements this for every every symbol and alphabetic variant.
That means |x| to $x$, |\xi| to $\xi$, |\leq| to $\leq$, etc., |\symscr{H}|
to $\symscr{H}$ and so on, all for Unicode glyphs within a single font.

This package deals well with Unicode characters for maths
input. This includes using literal Greek letters in formulae,
resolving to upright or italic depending on preference.

Font features specific to \pkg{unicode-math} are shown in \tabref{mathfontfeatures}.
Package options (see \tabref{pkgopt}) may also be used.
Other \pkg{fontspec} features are also valid.

\begin{table}\centering
  \topcaption{Maths font options.}
  \tablabel{mathfontfeatures}
  \begin{tabular}{lll}
    \toprule
    Option & Description & See\dots \\
    \midrule
    |range| & Style of letters & \secref{range} \\
    |script-font| & Font to use for sub- and super-scripts & \secref{sscript} \\
    |script-features| & Font features for sub- and super-scripts & \secref{sscript} \\
    |sscript-font| & Font to use for nested sub- and super-scripts & \secref{sscript} \\
    |sscript-features| & Font features for nested sub- and super-scripts & \secref{sscript} \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Using multiple fonts}
\seclabel{range}

There will probably be few cases where a single Unicode maths font suffices
(simply due to glyph coverage). The \STIX\ font comes to mind as a
possible exception. It will therefore be necessary to delegate specific
Unicode ranges of glyphs to separate fonts:
  \codeline{\cmd\setmathfont\marg{font name}|[range=|\meta{unicode range}|,|\meta{font features}|]|}
where \meta{unicode range} is a comma-separated list of Unicode slot numbers and ranges such as |{"27D0-"27EB,"27FF,"295B-"297F}|.
Note that \TeX's syntax for accessing the slot number of a character, such as |`\+|, will also work here.
Only numerical slots can be used in ranged declarations.

You may also use the macro for accessing the glyph, such as |range=|\cs{int}, or whole collection of symbols with the same math type, such as |range=\mathopen|, or complete math styles such as |range=\symbb| (or just |range=bb|).

\subsubsection{Control over alphabet ranges}

As discussed earlier, Unicode mathematics consists of a number of `alphabet styles' within a single font. In \pkg{unicode-math}, these ranges are indicated with the following (hopefully self-explanatory) labels:
\begin{quote}\ttfamily
\ExplSyntaxOn
\clist_const:Nn \g__um_named_ranges_clist {
up    ,
it    ,
bb    ,
bbit  ,
scr   ,
cal   ,
bfcal ,
frak  ,
tt    ,
sfup  ,
sfit  ,
bfup  ,
bfit  ,
bfscr ,
bffrak,
bfsfup,
bfsfit,
}
\clist_use:Nn \g__um_named_ranges_clist {\,,\,~}
\ExplSyntaxOff
\end{quote}
Fonts can be selected (for predefined ranges only) using the following syntax, in which case all other maths font setup remains untouched:
\begin{itemize}
\item |[range=bb]| to use the font for `|bb|' letters only.
\item |[range=bfsfit/{greek,Greek}]| for Greek lowercase and uppercase only (also with |latin|, |Latin|, |num| as possible options for Latin lower-/upper-case and numbers, resp.).
\item |[range=up->sfup]| to map to different output styles.
\end{itemize}

A common request is to load numerals only from a specific font. This can be
achieved with an option such as |range=up/{num}|.

Note that `meta-styles' such as `|bf|' and `|sf|' are not included in the list above since they are context dependent. Use |[range=bfup]| and |[range=bfit]| to effect changes to the particular ranges selected by `|bf|' (and similarly for `|sf|').

If a particular math style is not defined in the font, we fall back onto the lower-base plane (i.e., `upright') glyphs.
Therefore, to use an \ascii-encoded fractur font, for example, write
\begin{Verbatim}
  \setmathfont{SomeFracturFont}[range=frak]
\end{Verbatim}
and because the math plane fractur glyphs will be missing, \pkg{unicode-math} will know to use the \ascii\ ones instead.
If necessary this behaviour can be forced with |[range=frak->up]|, since the `|up|' range corresponds to \ascii\ letters.

%If you wanted to swap the maths symbols with sans serif forms, it would be possible to write |[range={up->sfup,it->sfit}]|.
%Note, however, that at present Unicode does not encode glyphs for sans serif Greek (\tabref{mathalphabets}).

Users of the impressive Minion Math fonts (commercial) may use remapping to access the bold glyphs using:
\begin{Verbatim}
  \setmathfont{MinionMath-Regular.otf}
  \setmathfont{MinionMath-Bold.otf}[range={bfup->up,bfit->it}]
\end{Verbatim}
To set up the complete range of optical sizes for these fonts, a font declaration such as the following may be used: (adjust may be desired according to the font size of the document)
\begin{Verbatim}
\setmathfont{Minion Math}[
 SizeFeatures = {
  {Size =      -6.01,  Font = MinionMath-Tiny},
  {Size =  6.01-8.41,  Font = MinionMath-Capt},
  {Size =  8.41-13.01, Font = MinionMath-Regular},
  {Size = 13.01-19.91, Font = MinionMath-Subh},
  {Size = 19.91-,      Font = MinionMath-Disp}
 }]

\setmathfont{Minion Math}[range = {bfup->up,bfit->it},
 SizeFeatures = {
  {Size =      -6.01,  Font = MinionMath-BoldTiny},
  {Size =  6.01-8.41,  Font = MinionMath-BoldCapt},
  {Size =  8.41-13.01, Font = MinionMath-Bold},
  {Size = 13.01-19.91, Font = MinionMath-BoldSubh},
  {Size = 19.91-,      Font = MinionMath-BoldDisp}
 }]
\end{Verbatim}


\subsection{Script and scriptscript fonts/features}
\seclabel{sscript}

Cambria Math uses OpenType font features to activate smaller optical sizes
for scriptsize and scriptscriptsize symbols (the $B$ and $C$, respectively,
in $A_{B_C}$).
Other typefaces (such as Minion Math) may use entirely separate font files.

The features |script-font| and |sscript-font| allow alternate fonts to be
selected for the script and scriptscript sizes, and |script-features| and
|sscript-features| to apply different OpenType features to them.

By default |script-features| is defined as |Style=MathScript| and |sscript-features| is |Style=MathScriptScript|.
These correspond to the two levels of OpenType's |ssty| feature tag.
If the |(s)script-features| options are specified manually, you must
additionally specify the |Style| options as above.


\subsection{Maths `versions'}

\LaTeX\ uses a concept known as `maths versions' to switch math fonts
mid-document.
This is useful because it is more efficient than loading a complete maths
font from scratch every time---especially with thousands of glyphs in the case of Unicode maths!
The canonical example for maths versions is to select a `bold' maths font
which might be suitable for section headings, say.
(Not everyone agrees with this typesetting choice, though; be careful.)

To select a new maths font in a particular version, use the syntax
  \codeline{\cmd\setmathfont\marg{font name}|[version=|\meta{version name}|,|\meta{font features}|]|}
and to switch between maths versions mid-document use the standard \LaTeX\ command
\cmd\mathversion\marg{version name}.

Note there are currently open issues regarding the interaction between the |version|
and the |range| features, so please proceed with caution.

\subsection{Legacy maths `alphabet' commands}
\seclabel{mathselect}

\LaTeX\ traditionally uses \cs{DeclareMathAlphabet} and \cs{SetMathAlphabet} to define document commands such as \cs{mathit}, \cs{mathbf}, and so on.
While these commands can still be used, \pkg{unicode-math} defines a wrapper command to assist with the creation of new such maths alphabet commands.
This command is known as \cs{setmathface} in symmetry with \pkg{fontspec}'s \cs{newfontface} command; it takes syntax:
\begin{quote}
  \cmd\setmathfontface\meta{command}\marg{font name}|[|\meta{font features}|]|

  \makebox[0pt][l]{\cmd\setmathfontface\meta{command}\marg{font name}|[||version=|\meta{version name}|,|\meta{font features}|]|}
\end{quote}
For example, if you want to define a new legacy maths alphabet font \cs{mathittt}:
\begin{verbatim}
  \setmathfontface\mathittt{texgyrecursor-italic.otf}
  ...
  $\mathittt{foo} = \mathittt{a} + \mathittt{b}$
\end{verbatim}


\subsubsection{Default `text math' fonts}

The five `text math' fonts, discussed above, are: \cs{mathrm}, \cs{mathbf}, \cs{mathit}, \cs{mathsf}, and \cs{mathtt}.
These commands are also defined with their original definition under synonyms \cs{mathtextrm}, \cs{mathtextbf}, and so on.
(These definitions hold regardless of package option, in case you need to be sure.)

When selecting document fonts using \pkg{fontspec} commands such as \cs{setmainfont}, \pkg{unicode-math} inserts some additional code into \pkg{fontspec} that keeps the current default fonts `in sync' with their corresponding \cs{mathrm} commands, etc.

For example, in standard \LaTeX, \cs{mathsf} doesn't change even if the main document font is changed using |\renewcommand\sfdefault{...}|. With \pkg{unicode-math} loaded, after writing |\setsansfont{Helvetica}|, \cs{mathsf} will now be set in Helvetica.

If the \cs{mathsf} font is set explicitly at any time in the preamble, this `auto-following' does not occur. The legacy math font switches can be defined either with commands defined by \pkg{fontspec} (|\setmathrm|, |\setmathsf|, etc.) or using the more general |\setmathfontface\mathsf| interface defined by \pkg{unicode-math}.


\subsubsection{Replacing `text math' fonts by symbols}
\seclabel{textmathlegacy}

For certain types of documents that use legacy input syntax, it may be preferable to have |\mathbf| behave as if it were |\symbf| en masse (et cetera respectively).
A series of package options (\tabref{legacyfontswitch}) are provided to facilitate switching the definition of \cs{mathXYZ} for the five legacy text math font definitions.

For example, if in a particular document |\mathbf| is used only for choosing symbols of vectors and matrices, a dedicated symbol font (|\symbf|) will produce better spacing and will better match the main math font.
In that case loading |unicode-math| with the |mathbf=sym| will achieve the desired result.

\begin{table}
  \centering
  \topcaption{Maths text font configuration options. Note that \cs{mathup} and \cs{mathrm} are aliases of each other and cannot be configured separately.}
  \tablabel{legacyfontswitch}
  \begin{tabular}{lll}
    \toprule
    Defaults (from `text' font) & From `maths symbols' \\
    \midrule
    |mathrm=text| &   |mathrm=sym |  \\
    |mathup=text|\rlap{$^\ast$} &   |mathup=sym|{}\rlap{$^\ast$}  \\
    |mathit=text| &   |mathit=sym |  \\
    |mathsf=text| &   |mathsf=sym |  \\
    |mathbf=text| &   |mathbf=sym |  \\
    |mathtt=text| &   |mathtt=sym |  \\
    \bottomrule
  \end{tabular}
\end{table}


\subsubsection{Operator font}

\LaTeX\ defines an internal command \cs{operator@font} for typesetting elements such as |\sin| and |\cos|.
This font is selected from the legacy |operators| NFSS `MathAlphabet', which is no longer relevant in the context of \pkg{unicode-math}.
By default, the \cs{operator@font} command is defined to switch to the \cs{mathrm} font.
You may now change these using the command:
\begin{Verbatim}
\setoperatorfont\mathit
\end{Verbatim}
Or, to select a \pkg{unicode-math} range:
\begin{Verbatim}
\setoperatorfont\symscr
\end{Verbatim}
\setoperatorfont\symscr
For example, after the latter above, |$\sin x$| will produce `$\sin x$'.

\mathversion{normal}
\setoperatorfont\mathrm


\section{Maths input}

\XeTeX's Unicode support allows maths input through two methods. Like
classical \TeX, macros such as \cmd\alpha, \cmd\sum, \cmd\pm, \cmd\leq, and
so on, provide verbose access to the entire repertoire of characters defined
by Unicode. The literal characters themselves may be used instead, for more
readable input files.

\subsection{Math `style'}
\seclabel{math-style}

Classically, \TeX\ uses italic lowercase Greek letters and \emph{upright}
uppercase Greek letters for variables in mathematics. This is contrary to
the \textsc{iso} standards of using italic forms for both upper- and lowercase.
Furthermore, in various historical contexts, often associated with French typesetting, it was common to use upright uppercase \emph{Latin} letters as well as upright
upper- and lowercase Greek, but italic lowercase latin. Finally, it is not unknown to use upright letters
for all characters, as seen in the Euler fonts.

The \pkg{unicode-math} package accommodates these possibilities with the
option \opt{math-style} that takes one of four (case sensitive) arguments:
\opt{TeX}, \opt{ISO}, \opt{french}, or \opt{upright}.\footnote{Interface inspired by Walter Schmidt's \pkg{lucimatx} package.}
The \opt{math-style} options' effects are shown in brief in \tabref{math-style}.

The philosophy behind the interface to the mathematical symbols
lies in \LaTeX's attempt of separating content and formatting. Because input
source text may come from a variety of places, the upright and
`mathematical' italic Latin and Greek alphabets are \emph{unified} from the
point of view of having a specified meaning in the source text. That is, to
get a mathematical ‘$x$’, either the \ascii\ (`keyboard') letter |x| may
be typed, or the actual Unicode character may be used. Similarly for Greek
letters. The upright or italic forms are then chosen based on the
|math-style| package option.

If glyphs are desired that do not map as per the package option (for
example, an upright `g' is desired but typing |$g$| yields `$g$'),
\emph{markup} is required to specify this; to follow from the example:
|\symup{g}|.
Maths style commands such as \cmd\symup\ are detailed later.

For compatibility and consistency, however, upright and italic Greek letters
can be `forced` using \verb|up| or \verb|it| prefixes before their names.
For example, \cs{Gamma} will give an upright or italic Gamma depending on the
\opt{math-style}, but \cs{upGamma} and \cs{itGamma} will always give upright
or italic Gammas, respectively.

\paragraph{`Literal' interface}
Some may not like this convention of normalising their input.
For them, an upright |x| is an upright `x' and that's that.
(This will be the case when obtaining source text from copy/pasting PDF or
Microsoft Word documents, for example.)
For these users, the |literal| option to |math-style| will effect this behaviour.
The \cs{symliteral}\marg{syms} command can also be used, regardless of package setting, to force the style to match the literal input characters.
This is a `mirror' to \cs{symnormal}\marg{syms} (also alias \cs{mathnormal}) which `resets' the character mapping in its argument to that originally set up through package options.


\begin{table}
  \centering
  \topcaption{Effects of the \opt{math-style} package option.}
  \tablabel{math-style}
  \begin{tabular}{@{}>{\ttfamily}lcc@{}}
    \toprule
      & \multicolumn{2}{c}{Example} \\
       \cmidrule(l){2-3}
      \rmfamily Package option & Latin & Greek \\
    \midrule
      math-style=ISO & $(a,z,B,X)$ & $\symit{(\alpha,\beta,\Gamma,\Xi)}$ \\
      math-style=TeX & $(a,z,B,X)$ & $(\symit\alpha,\symit\beta,\symup\Gamma,\symup\Xi)$ \\
      math-style=french & $(a,z,\symup B,\symup X)$ & $(\symup\alpha,\symup\beta,\symup\Gamma,\symup\Xi)$ \\
      math-style=upright & $(\symup a,\symup z,\symup B,\symup X)$ & $(\symup\alpha,\symup\beta,\symup\Gamma,\symup\Xi)$ \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{`Full-width' letters}
Unicode contains `full-width' versions of ASCII from \unichar{FF01}.
The numerals and latin letters in this range are defined by \pkg{unicode-math}
to map to their standard ASCII counterparts, which are then controlled by the relevant \opt{math-style} setting.
Other full-width symbols are not currently included but can be if there is sufficient need or desire.

\subsection{Bold style}
\seclabel{bold-style}

Similar as in the previous section, ISO standards differ somewhat to \TeX's
conventions (and classical typesetting) for `boldness' in mathematics. In
the past, it has been customary to use bold \emph{upright} letters to denote
things like vectors and matrices. For example, \( \symbfup{M} =
(\mitM_x,\mitM_y,\mitM_z) \). Presumably, this was due to the relatively
scarcity of bold italic fonts in the pre-digital typesetting era.
It has been suggested by some that \emph{italic} bold symbols should be used nowadays instead, but this practise is certainly not widespread.

Bold Greek letters have simply been bold variant glyphs of their regular
weight, as in \( \mbfitxi = (\mitxi_\mitr,\mitxi_\mitphi,\mitxi_\mittheta)
\).
Confusingly, the syntax in \LaTeX\ traditionally has been different for obtaining `normal' bold symbols in Latin and Greek: \cmd\mathbf\ in the former (`$\symbfup{M}$'), and \cmd\bm\ (or
\cmd\boldsymbol, deprecated) in the latter (`$\mbfitxi$').

In \pkg{unicode-math}, the \cmd\symbf\ command works directly with both
Greek and Latin maths characters and depending on package option
either switches to upright for Latin letters (|bold-style=TeX|) as well or
keeps them italic (|bold-style=ISO|).
To match the package options for non-bold characters, with option
|bold-style=upright| all bold characters are upright, and
|bold-style=literal| does not change the upright/italic shape of the letter.
The \opt{bold-style} options' effects are shown in brief in \tabref{bold-style}.

Upright and italic bold mathematical letters input as direct Unicode
characters are normalised with the same rules. For example, with
|bold-style=TeX|, a literal bold italic latin character will be typeset
upright.

Note that \opt{bold-style} is independent of \opt{math-style}, although if
the former is not specified then matching defaults are chosen based on the
latter.

\begin{table}
  \centering
  \topcaption{Effects of the \opt{bold-style} package option.}
  \tablabel{bold-style}
  \begin{tabular}{@{}>{\ttfamily}lcc@{}}
    \toprule
      & \multicolumn{2}{c}{Example} \\
       \cmidrule(l){2-3}
      \rmfamily Package option & Latin & Greek \\
    \midrule
      bold-style=ISO & $(\symbfit a, \symbfit z, \symbfit B, \symbfit X)$ & $(\symbfit\alpha, \symbfit\beta, \symbfit\Gamma, \symbfit\Xi)$ \\
      bold-style=TeX & $(\symbfup a,\symbfup z,\symbfup B,\symbfup X)$ & $(\symbfit\alpha, \symbfit\beta,\symbfup \Gamma,\symbfup \Xi)$ \\
      bold-style=upright & $(\symbfup a,\symbfup z,\symbfup B,\symbfup X)$ & $(\symbfup \alpha,\symbfup \beta,\symbfup \Gamma,\symbfup \Xi)$ \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Sans serif style}
\seclabel{sans-style}

Unicode contains upright and italic, medium and bold mathematical style characters.
These may be explicitly selected with the \cs{symsfup}, \cs{symsfit}, \cs{symbfsfup}, and \cs{symbfsfit}
commands discussed in \secref{all-math-alphabets}.

How should the generic \cs{symsf} behave? Unlike bold, sans serif is used much more sparingly
in mathematics. I've seen recommendations to typeset tensors in sans serif italic
or sans serif italic bold (e.g., examples in the \pkg{isomath} and \pkg{mattens} packages).
But \LaTeX's \cs{mathsf} is \textsl{upright} sans serif.

Therefore, the package options |[sans-style=upright]| and |[sans-style=italic]| control the behaviour of \cs{symsf}.
The |upright| style sets up the command to use upright sans serif, including Greek;
the |italic| style switches to using italic in both Latin and Greek.
In other words, this option simply changes the meaning of \cs{symsf} to either \cs{symsfup} or \cs{symsfit}, respectively.
Please let me know if more granular control is necessary here.

There is also a |[sans-style=literal]| setting, set automatically with |[math-style=literal]|, which retains the uprightness of the input characters used when selecting the sans serif output.

\subsubsection{What about bold sans serif?}

While you might want your bold upright and your sans serif italic, I don't believe you'd also want your bold sans serif upright (etc.).
Therefore, bold sans serif follows from the setting for sans serif; it is completely independent of the setting for bold.

In other words, \cs{symbfsf} is either \cs{symbfsfup} or \cs{symbfsfit} based on |[sans-style=upright]| or |[sans-style=italic]|, respectively. And \texttt{[sans-style = literal]} causes \cs{symbfsf} to retain the same italic or upright shape as the input, and turns it bold sans serif.

N.B.: there is no medium-weight sans serif Greek range in Unicode.
Therefore, |\symsf{\alpha}| does not make sense (it produces `$\symsf{\alpha}$'), while |\symbfsf{\alpha}| gives `$\symbfsfup{\alpha}$' or `$\symbfsfit{\alpha}$' according to the |sans-style|.

\subsection{All (the rest) of the mathematical styles}
\seclabel{all-math-alphabets}

Unicode contains separate codepoints for most if not all variations of style
shape one may wish to use in mathematical notation. The complete list is shown
in \tabref{mathalphabets}. Some of these have been covered in the previous sections.

The math font switching commands do not nest; therefore if you want
sans serif bold, you must write |\symbfsf{...}| rather than |\symbf{\symsf{...}}|.
This may change in the future.

\begin{table}
\caption{Mathematical styles defined in Unicode. Black dots indicate an style exists in the font specified; blue dots indicate shapes that should always be taken from the upright font even in the italic style. See main text for description of \cs{mathbbit}.}
\tablabel{mathalphabets}
\centering
\def\Y{\textbullet}
\def\M{\textcolor[rgb]{0.5,0.5,1}{\textbullet}}
\begin{tabular}{@{} lll l ccc @{}}
\toprule
\multicolumn{3}{c}{Font} & & \multicolumn{3}{c}{Alphabet} \\
\cmidrule(r){1-3}
\cmidrule(l){5-7}
Style & Shape & Series & Switch & Latin & Greek & Numerals \\
\midrule
Serif      & Upright & Normal & \cs{symup}     & \Y & \Y & \Y  \\
           &         & Bold   & \cs{symbfup}   & \Y & \Y & \Y  \\
           & Italic  & Normal & \cs{symit}     & \Y & \Y & \M  \\
           &         & Bold   & \cs{symbfit}   & \Y & \Y & \M  \\
Sans serif & Upright & Normal & \cs{symsfup}   & \Y &    & \Y  \\
           & Italic  & Normal & \cs{symsfit}   & \Y &    & \M  \\
           & Upright & Bold   & \cs{symbfsfup} & \Y & \Y & \Y  \\
           & Italic  & Bold   & \cs{symbfsfit} & \Y & \Y & \M  \\
Typewriter & Upright & Normal & \cs{symtt}     & \Y &    & \Y  \\
Double-struck & Upright & Normal & \cs{symbb}     & \Y &    & \Y  \\
              & Italic  & Normal & \cs{symbbit}   & \Y &    &  \\
Script     & Upright & Normal & \cs{symscr}    & \Y &    &     \\
           &         & Bold   & \cs{symbfscr}  & \Y &    &     \\
Fraktur    & Upright & Normal & \cs{symfrak}   & \Y &    &     \\
           &         & Bold   & \cs{symbffrac} & \Y &    &     \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Scope of the functionality of the \cs{sym..} commands}

The \cs{sym..} commands are designed to affect only the follow sets of input letters: numerals ($0$--$9$), Latin ($a$--$z$, $A$--$Z$), Greek ($\alpha$--$\omega$, $\Alpha$--$\Omega$,), and the \cs{partial} and \cs{nabla} symbols ($\partial$, $\nabla$).
These are the only symbols for which Unicode defines separate codepoints with varying mathematical style.

There is currently no scope for including other symbols in the \cs{sym..} commands, such as writing |\symbf{\int}| for a bold integral symbol.
Therefore the commands provided by \pkg{unicode-math} should not be compared to those provided by the \pkg{bm} package.

\subsubsection{Double-struck}

The double-struck style (also known as `blackboard bold') consists of
upright Latin letters $\{\symbb{a}$--$\symbb{z}$,$\symbb{A}$$\symbb{Z}\}$,
numerals $\symbb{0}$--$\symbb{9}$, summation symbol $\symbb\sum$, and four
Greek letters only: $\{\symbb{\gamma\pi\Gamma\Pi}\}$.

While |\symbb{\sum}| does produce a double-struck summation symbol,
its limits aren't properly aligned. Therefore,
either the literal character or the control sequence \cs{Bbbsum} are
recommended instead.

There are also five Latin \emph{italic} double-struck letters: $\symbbit{Ddeij}$.
These can be accessed (if not with their literal characters or control sequences)
with the \cs{mathbbit} style switch, but note that only those five letters
will give the expected output.

\subsubsection{Caligraphic vs.\ Script variants}

The Unicode maths encoding contains a style for `Script' letters,
and while by default \cs{mathcal} and \cs{mathscr}
are synonyms, there are some situations when a
separate `Caligraphic' style is needed as well.

If a font contains alternate glyphs for a separate caligraphic style,
they can be selected explicitly as shown below.
This feature is currently only supported by the XITS~Math font, where
the caligraphic letters are accessed with the same glyph slots as the
script letters but with the first stylistic set feature (|ss01|) applied.
An example is shown below.
\begin{quote}
\setmathfont{xits-math.otf}
\setmathfont{xits-math.otf}[range=cal,StylisticSet=1]
The Script style (\cs{mathscr}) in XITS Math is: $\symscr{ABCXYZ}$\par
The Caligraphic style (\cs{mathcal}) in XITS Math is: $\symcal{ABCXYZ}$
\end{quote}


\subsection{Miscellanea}

\subsubsection{Nabla}
\seclabel{nabla}

 The symbol $\nabla$ comes in the six forms shown in \tabref{nabla}.
 We want an individual option to specify whether we want upright or italic
 nabla by default (when either upright or italic nabla is used in the
 source). \TeX\ classically uses an upright nabla, and \textsc{iso}
 standards agree with this convention.
 The package options |nabla=upright| (default) and
 |nabla=italic| switch between the two choices, and |nabla=literal| respects
 the shape of the input character.
|nabla=literal| is activated automatically after |math-style=literal|.

These settings are then inherited through \cmd\symbf; \cmd\symit\ and \cmd\symup\ can be used to force the shape of the nabla one way or the other.


\begin{table}
  \begin{minipage}[b]{0.49\textwidth}
  \centering
  \topcaption{The various forms of nabla.}
  \tablabel{nabla}
  \let \tmpshow\empty
  \begin{tabular}{@{}llc@{}}
    \toprule
    \multicolumn{2}{@{}l}{Description} & Glyph \\
    \cmidrule(r){1-2}\cmidrule(l){3-3}
    Upright & Serif      & $\symup\nabla$     \\
            & Bold serif & $\symbfup\nabla$   \\
            & Bold sans  & $\symbfsfup\nabla$ \\
    \cmidrule(lr){1-2}\cmidrule(lr){3-3}
    Italic & Serif       & $\symit\nabla$     \\
           & Bold serif  & $\symbfit\nabla$   \\
           & Bold sans   & $\symbfsfit\nabla$ \\
    \bottomrule
  \end{tabular}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.49\textwidth}
  \centering
  \topcaption{The partial differential.}
  \tablabel{partial}
  \begin{tabular}{@{}llc@{}}
    \toprule
    \multicolumn{2}{@{}l}{Description} & Glyph \\
    \cmidrule(r){1-2}\cmidrule(l){3-3}
    Regular   & Upright & $\symup\partial$     \\
              & Italic  & $\symit\partial$     \\
    Bold      & Upright & $\symbfup\partial$   \\
              & Italic  & $\symbfit\partial$   \\
    Sans bold & Upright & $\symbfsfup\partial$ \\
              & Italic  & $\symbfsfit\partial$ \\
    \bottomrule
  \end{tabular}
  \end{minipage}
\end{table}


\subsubsection{Partial}
\seclabel{partial}

The same logic as for nabla applies to the symbols \unichar{2202} partial differential and \unichar{1D715} math italic partial differential.
However, in practice these symbols are often designed identically in an italic style.

If the font you are using supports it, use the |partial=upright| or |partial=italic| (default) package options to specify
which one you would like, or |partial=literal| to have the same character
used in the output as was used for the input.
|partial=literal| is activated following |math-style=literal|.

See \tabref{partial} for the variations on the partial differential symbol.


\subsubsection{Primes}

Primes ($x'$) may be input in several ways. You may use any combination
the \ascii\ straight quote (\texttt{\char`\'}) or the Unicode prime \unichar{2032}
($'$); when multiple primes occur next to each other, they chain
together to form double, triple, or quadruple primes if the font contains
pre-drawn glyphs. The individual prime glyphs are accessed, as usual,
with the \cs{prime} command, and the double-, triple-, and quadruple-prime
glyphs are available with \cs{dprime}, \cs{trprime}, and \cs{qprime},
respectively.

If the font does not contain the pre-drawn glyphs or more than four primes
are used, the single prime glyph is used multiple times with a negative
kern to get the spacing right. There is no user interface to adjust this
negative kern yet (because I haven't decided what it should look like);
if you need to, write something like this:
\begin{Verbatim}
\ExplSyntaxOn
\muskip_gset:Nn \g_@@_primekern_muskip { -\thinmuskip/2 }
\ExplySyntaxOff
\end{Verbatim}
Backwards or reverse primes behave in exactly the same way; use the \ascii\
back tick (\texttt{\char`\`}) or the Unicode reverse prime \unichar{2035}
({\umfont\char"2035}).
The command to access the backprime is \cs{backprime}, and
multiple backwards primes can accessed with \cs{backdprime},
\cs{backtrprime}, and \cs{backqprime}.

In all cases above, no error checking is performed if you attempt to
access a multi-prime glyph in a font that doesn't contain one. For this
reason, it may be safer to write |x''''| instead of |x\qprime|
in general.

If you ever need to enter the straight quote |'| or the backtick |`| in
maths mode, these glyphs can be accessed with \cs{mathstraightquote} and
\cs{mathbacktick}.

\subsubsection{Unicode subscripts and superscripts}

You may, if you wish, use Unicode subscripts and superscripts in your
source document. For basic expressions, the use of these characters
can make the input more readable.
Adjacent sub- or super-scripts will be concatenated into a single
expression.

The range of subscripts and superscripts supported by this package
are shown in \figref{superscripts,subscripts}. Please request more if
you think it is appropriate.

\begin{figure}\centering
\fbox{\fontspec{CharisSILR.ttf}\Large
A
^^^^2070 ^^^^00b9 ^^^^00b2 ^^^^00b3 ^^^^2074 ^^^^2075 ^^^^2076 ^^^^2077
^^^^2078 ^^^^2079 ^^^^207a ^^^^207b ^^^^207c ^^^^207d ^^^^207e ^^^^2071
^^^^207f ^^^^207f ^^^^02b0 ^^^^02b2 ^^^^02b3 ^^^^02b7 ^^^^02b8
Z}
\caption{
  The Unicode superscripts supported as input characters.
  These are the literal glyphs from Charis SIL,
  not the output seen when used for maths input.
  The `A' and `Z' are to provide context for the size and
  location of the superscript glyphs.
}
\figlabel{superscripts}
\end{figure}

\begin{figure}\centering
\fbox{\fontspec{CharisSILR.ttf}\Large
A
^^^^2080 ^^^^2081 ^^^^2082 ^^^^2083 ^^^^2084 ^^^^2085 ^^^^2086 ^^^^2087
^^^^2088 ^^^^2089 ^^^^208a ^^^^208b ^^^^208c ^^^^208d ^^^^208e ^^^^2090
^^^^2091 ^^^^1d62 ^^^^2092 ^^^^1d63 ^^^^1d64 ^^^^1d65 ^^^^2093 ^^^^1d66
^^^^1d67 ^^^^1d68 ^^^^1d69 ^^^^1d6a
Z}
\caption{
  The Unicode subscripts supported as input characters.
  See note from \figref{superscripts}.
}
\figlabel{subscripts}
\end{figure}

\subsubsection{Colon}
\seclabel{colon}

The colon is one of the few confusing characters of Unicode maths.
In \TeX, \texttt{:} is defined as a colon with relation spacing: `$a:b$'.
While \cs{colon} is defined as a colon with punctuation spacing: `$a\colon b$'.

In Unicode, \unichar{003A} {colon} is defined as a punctuation symbol,
while \unichar{2236} {ratio} is the colon-like symbol used in mathematics to denote
ratios and other things.

This breaks the usual straightforward mapping from control sequence to Unicode input character
to (the same) Unicode glyph.

To preserve input compatibility, we remap the \ascii\ input character `\texttt{:}' to \unichar{2236}.
Typing a literal \unichar{2236} char will result in the same output.
If \pkg{amsmath} is loaded, then the definition of \cs{colon} is inherited from there
(it looks like a punctuation colon with additional space around it).
Otherwise, \cs{colon} is made to output a colon with \cs{mathpunct} spacing.

The package option |colon=literal| forces \ascii\ input `|:|' to be printed as \cs{mathcolon} instead.


\subsubsection{Slashes and backslashes}
\seclabel{slash-delimiter}

There are several slash-like symbols defined in Unicode. The complete list is shown in \tabref{slashes}.

\begin{table}\centering
\caption{Slashes and backslashes.}
\tablabel{slashes}
\begin{tabular}{@{}cl@{}cl@{}}
\toprule
Slot & Name & Glyph & Command  \\
\midrule
\unichar{002F} & \textsc{solidus}                 & \umfont \char"002F & \cs{slash} \\
\unichar{2044} & \textsc{fraction slash}          & \umfont \char"2044 & \cs{fracslash} \\
\unichar{2215} & \textsc{division slash}          & \umfont \char"2215 & \cs{divslash} \\
\unichar{29F8} & \textsc{big solidus}             & \umfont \char"29F8 & \cs{xsol} \\
\midrule
\unichar{005C} & \textsc{reverse solidus}         & \umfont \char"005C & \cs{backslash} \\
\unichar{2216} & \textsc{set minus}               & \umfont \char"2216 & \cs{smallsetminus} \\
\unichar{29F5} & \textsc{reverse solidus operator}& \umfont \char"29F5 & \cs{setminus} \\
\unichar{29F9} & \textsc{big reverse solidus}     & \umfont \char"29F9 & \cs{xbsol} \\
\bottomrule
\end{tabular}
\end{table}

In regular \LaTeX\ we can write \cs{left}\cs{slash}\dots\cs{right}\cs{backslash}
and so on and obtain extensible delimiter-like symbols. Not all of the Unicode slashes
are suitable for this (and do not have the font support to do it).

\paragraph{Slash}

Of \unichar{2044} {fraction slash}, TR25 says that it is:
\begin{quote}
\dots used to build up simple fractions in running text\dots
however parsers of mathematical texts should be prepared to handle fraction slash
when it is received from other sources.
\end{quote}

\unichar{2215} {division slash} should be used when division is represented
without a built-up fraction; $\pi\approx22/7$, for example.

\unichar{29F8} {big solidus} is a `big operator' (like $\sum$).

\paragraph{Backslash}

The \unichar{005C} {reverse solidus} character \cs{backslash} is used for denoting
double cosets: $A\backslash B$. (So I'm led to believe.)
It may be used as a `stretchy' delimiter if supported by the font.

MathML uses \unichar{2216} {set minus} like this: $A\smallsetminus B$.\footnote{\S4.4.5.11 \url{http://www.w3.org/TR/MathML3/}}
The \LaTeX\ command name \cs{smallsetminus} is used for backwards compatibility.

Presumably, \unichar{29F5} {reverse solidus operator} is intended to
be used in a similar way, but it could also (perhaps?) be used to
represent `inverse division': $\pi\approx7\mathbin{\backslash}22$.^^A
\footnote{This is valid syntax in the Octave and Matlab programming languages,
in which it means matrix inverse pre-multiplication. I.e., $A\mathbin{\backslash} B\equiv A^{-1}B$.}
The \LaTeX\ name for this character is \cs{setminus}.

Finally, \unichar{29F9} {big reverse solidus} is a `big operator' (like $\sum$).

\paragraph{How to use all of these things}

Unfortunately, font support for the above characters/glyphs is rather inconsistent.
In Cambria Math, the only slash that grows (say when writing
\[
\left.\left[\begin{array}{cc} a & b \\ c & d\end{array}\right]\middle\slash
      \left[\begin{array}{cc} 1 & 1 \\ 1 & 0\end{array}\right] \right.\quad )
\]
is the \textsc{fraction slash}, which we just established above is
sort of only supposed to be used in text.

Of the above characters, the following are allowed to be used after
\cs{left}, \cs{middle}, and \cs{right}:
\begin{itemize}
\item \cs{fracslash};
\item \cs{slash}; and,
\item \cs{backslash} (the only reverse slash).
\end{itemize}

However, we assume that there is only \emph{one} stretchy slash
in the font; this is assumed by default to be \unichar{002F} {solidus}.
Writing \cs{left/} or \cs{left}\cs{slash} or \cs{left}\cs{fracslash}
will all result in the same stretchy delimiter being used.

The delimiter used can be changed with the |slash-delimiter| package option.
Allowed values are |ascii|, |frac|, and |div|, corresponding to the respective
Unicode slots.

For example: as mentioned above, Cambria Math's stretchy slash is
\unichar{2044} {fraction slash}. When using Cambria Math, then
\pkg{unicode-math} should be loaded with the |slash-delimiter=frac| option.
(This should be a font option rather than a package option, but
it will change soon.)

\subsubsection{Behaviour of hyphens in mathematics}
\seclabel{hyphen}

Unicode defines the following related characters:
\begin{itemize}
\item \unichar{0002D}{hyphen-minus}
\item \unichar{02212}{minus sign}
\item \unichar{02010}{hyphen} (\cs{mathhyphen})
\end{itemize}
The first two of these characters in the input will all behave as the binary operator
`minus sign'.
The third is defined by \pkg{unicode-math} as a `math letter' for constructions
like \verb|$R‐\text{Mod}$| ($R‐\text{Mod}$).
If more control is needed surrounding these symbols, additional options can be added to the package;
please get in touch if this is the case for you.


\subsubsection{Growing and non-growing accents}
\seclabel{growing-accents}

There are a few accents for which \TeX\ has both non-growing and growing
versions.  Among these are \cs{hat} and \cs{tilde}; the corresponding growing
versions are called \cs{widehat} and \cs{widetilde}, respectively.

Older versions of \XeTeX\ and \LuaTeX\ did not support this distinction,
however, and \emph{all} accents there were growing automatically. (I.e.,
\cs{hat} and \cs{widehat} are equivalent.) As of \LuaTeX\ v0.65 and \XeTeX\
v0.9998, these wide/non-wide commands will again behave in their expected
manner.


\subsubsection{Negations and the \cs{not} command}
\seclabel{negations}

The \cs{not} command in classic \LaTeXe\ was a mathematical slash modifying glyph that allowed for `negating` maths symbols where pre-built glyphs were not available. While Unicode encodes a slot for this modifying slash, it is only well-supported in \LuaTeX\ and not in \XeTeX.

To provide more flexibility, the \pkg{unicode-math} package defines \cs{not} to search for a predefined `negated' definitions for its argument and use that if available. This method can be used for fine-tuning in cases where spacing needs to be adjusted.

A `negated definition` is any symbol command prefixed by either \verb|n| or \verb|not|. For example, \pkg{unicode-math} by default defines both \cs{leftarrow} ($\leftarrow$) and \cs{nleftarrow} ($\nleftarrow$).

To define custom negated definitions for either symbols (e.g., \verb|\not=|) or commands (e.g., \verb|\not\equal|), use the \cs{NewNotCommand}\marg{symbol or cmd}\marg{definition} command. Its usage is as follows:
\begin{verbatim}
\NewNegationCommand {=} {\neq}
\NewNegationCommand {\equal} {\neq}
\end{verbatim}
If the command has already been defined, an error will result and \verb|\RenewNegationCommand| can be used to overwrite the original definition.


\subsubsection{Pre-drawn fraction characters}

Pre-drawn fractions \unichar{00BC}--\unichar{00BE}, \unichar{2150}--\unichar{215E}
are not suitable for use in mathematics output. However, they can be useful
as input characters to abbreviate common fractions.
\begin{center}
\fontspec{DejaVuSerif.ttf} ^^A available in TeX Live 2012 if not earlier
¼ ½ ¾  ↉ ⅐ ⅑ ⅒ ⅓ ⅔ ⅕ ⅖ ⅗ ⅘ ⅙ ⅚ ⅛ ⅜ ⅝ ⅞
\end{center}
For example, instead of writing `|\tfrac12 x|', you may consider it more readable to have
`|½x|' in the source instead.

If the \cs{tfrac} command exists (i.e., if \pkg{amsmath} is loaded or
you have specially defined \cs{tfrac} for this purpose), it will be used
to typeset the fractions. If not, regular \cs{frac} will be used. The command
to use (\cs{tfrac} or \cs{frac}) can be forced either way with the package
option |active-frac=small| or |active-frac=normalsize|, respectively.

\subsubsection{Circles}

Unicode defines a large number of different types of circles for a variety
of mathematical purposes. There are thirteen alone just considering the
all white and all black ones, shown in \tabref{circles}.

\LaTeX\ defines considerably fewer: \cs{circ} and \cs{bigcirc} for white;
\cs{bullet} for black. This package maps those commands to \cs{vysmwhtcircle},
\cs{mdlgwhtcircle}, and \cs{smblkcircle}, respectively.

\begin{table}\centering
\def\showchar#1#2#3{ \textsc{u}+{\small\ttfamily #1} & \texttt{\string#3} & \umfont \char"#1 \\}
\begin{tabular}{@{}llc@{}}
\toprule
Slot & Command & Glyph \\
\midrule
\showchar{00B7}{centerdot}{\cdotp}
\showchar{22C5}{small middle dot}{\cdot}
\showchar{2219}{bullet operator}{\vysmblkcircle}
\showchar{2022}{round bullet, filled}{\smblkcircle}
\showchar{2981}{z notation spot}{\mdsmblkcircle}
\showchar{26AB}{medium black circle}{\mdblkcircle}
\showchar{25CF}{circle, filled}{\mdlgblkcircle}
\showchar{2B24}{black large circle}{\lgblkcircle}
\bottomrule
\end{tabular}
\def\showchar#1#2#3{ \umfont \char"#1 & \texttt{\string#3} & \textsc{u}+{\small\ttfamily #1} \\}
\begin{tabular}{@{}cll@{}}
\toprule
Glyph & Command & Slot \\
\midrule
\\
\\
\showchar{2218}{composite function (small circle)}{\vysmwhtcircle}
\showchar{25E6}{white bullet}{\smwhtcircle}
\showchar{26AC}{medium small white circle}{\mdsmwhtcircle}
\showchar{26AA}{medium white circle}{\mdwhtcircle}
\showchar{25CB}{large circle}{\mdlgwhtcircle}
\showchar{25EF}{large circle}{\lgwhtcircle}
\bottomrule
\end{tabular}
\caption{Filled and hollow Unicode circles.}
\tablabel{circles}
\end{table}

\subsubsection{Triangles}

While there aren't as many different sizes of triangle as there are circle,
there's some important distinctions to make between a few similar characters. See \tabref{uptriangles} for the full summary.

These triangles all have different intended meanings. Note for backwards
compatibility with \TeX, \unichar{25B3} has \emph{two} different mappings
in \pkg{unicode-math}. \cs{bigtriangleup} is intended as a binary operator
whereas \cs{triangle} is intended to be used as a letter-like symbol.

But you're better off if you're using the latter form to indicate an
increment to use the glyph intended for this purpose, \unichar{2206}: $\increment x$.

Finally, given that $\triangle$ and $\increment$ are provided for you
already, it is better off to only use upright Greek Delta $\Delta$ if you're
actually using it as a symbolic entity such as a variable on its own.

\begin{table}\centering
\begin{tabular}{@{}llcl@{}}
\toprule
Slot & Command & Glyph & Class \\
\midrule
\unichar{25B5} & \cs{vartriangle}      & \umfont \char"25B5 & binary \\
\unichar{25B3} & \cs{bigtriangleup}    & \umfont \char"25B3 & binary \\
\unichar{25B3} & \cs{triangle}         & \umfont \char"25B3 & ordinary \\
\unichar{2206} & \cs{increment}        & \umfont \char"2206 & ordinary \\
\unichar{0394} & \cs{mathup}\cs{Delta} & \umfont \char"0394 & ordinary \\
\bottomrule
\end{tabular}
\caption{Different upwards pointing triangles.}
\tablabel{uptriangles}
\end{table}

\iffalse
\subsubsection{Normalising some input characters}

I believe
all variant forms should be used as legal input that is normalised to
a consistent output glyph, because we want to be fault-tolerant in the input.
Here are the duplicates:
\begin{quote}\obeylines
\unichar {251} {latin small letter alpha}
\unichar {25B} {latin small letter epsilon}
\unichar {263} {latin small letter gamma}
\unichar {269} {latin small letter iota}
\unichar {278} {latin small letter phi}
\unichar {28A} {latin small letter upsilon}
\unichar {190} {latin capital letter epsilon}
\unichar {194} {latin capital letter gamma}
\unichar {196} {latin capital letter iota}
\unichar {1B1} {latin capital letter upsilon}
\end{quote}

(Not yet implemented.)
\fi

\section{Advanced}

\subsection{Warning messages}

This package can produce a number of informational messages to try and inform the user when something might be going wrong due to package conflicts or something else.
As an experimental feature, these can be turn off on an individual basis with the package option |warnings-off| which takes a comma-separated list of warnings to suppress.
A warning will give you its name when printed on the console output; e.g.,
\begin{Verbatim}
  * unicode-math warning: "mathtools-colon"
  *
  * ... <warning message> ...
\end{Verbatim}
This warning could be suppressed by loading the package as follows:
\begin{Verbatim}
  \usepackage[warnings-off={mathtools-colon}]{unicode-math}
\end{Verbatim}

\subsection{Programmer's interface}

(Tentative and under construction.)
If you are writing some code that needs to know the current
maths style (\cs{mathbf}, \cs{mathit}, etc.), you can query the
variable \cs{l_@@_mathstyle_tl}. It will contain the maths style
without the leading `math' string; for example,
|\symbf { \show \l_@@_mathstyle_tl }|
will produce `bf'.

\endinput

% /©
%
% ------------------------------------------------
% The UNICODE-MATH package  <wspr.io/unicode-math>
% ------------------------------------------------
% This package is free software and may be redistributed and/or modified under
% the conditions of the LaTeX Project Public License, version 1.3c or higher
% (your choice): <http://www.latex-project.org/lppl/>.
% ------------------------------------------------
% Copyright 2006-2018  Will Robertson, LPPL "maintainer"
% Copyright 2010-2017  Philipp Stephani
% Copyright 2011-2017  Joseph Wright
% Copyright 2012-2015  Khaled Hosny
% ------------------------------------------------
%
% ©/


==> unicode-math/um-doc-mathfontdimen.tex <==
%%^^A%% um-doc-mathfontdimen.tex -- part of UNICODE-MATH <wspr.io/unicode-math>

\section{\Hologo{XeTeX} math font dimensions}

These are the extended \cmd\fontdimen s available for suitable fonts
in \XeTeX. Note that Lua\TeX\ takes an alternative route, and this package
will eventually provide a wrapper interface to the two (I hope).

\newcounter{mfdimen}
\setcounter{mfdimen}{9}
\newcommand\mathfontdimen[2]{^^A
  \stepcounter{mfdimen}^^A
  \themfdimen & {\scshape\small #1} & #2\vspace{0.5ex} \tabularnewline}

\begin{longtable}{
  @{}c>{\raggedright\parfillskip=0pt}p{4cm}>{\raggedright}p{7cm}@{}}
\toprule \cmd\fontdimen & Dimension name & Description\tabularnewline\midrule \endhead
\bottomrule\endfoot
\mathfontdimen{Script\-Percent\-Scale\-Down}
{Percentage of scaling down for script level 1. Suggested value: 80\%.}
\mathfontdimen{Script\-Script\-Percent\-Scale\-Down}
{Percentage of scaling down for script level 2 (Script\-Script). Suggested value: 60\%.}
\mathfontdimen{Delimited\-Sub\-Formula\-Min\-Height}
{Minimum height required for a delimited expression to be treated as a subformula. Suggested value: normal line height\,×\,1.5.}
\mathfontdimen{Display\-Operator\-Min\-Height}
{Minimum height of n-ary operators (such as integral and summation) for formulas in display mode.}
\mathfontdimen{Math\-Leading}
{White space to be left between math formulas to ensure proper line spacing. For example, for applications that treat line gap as a part of line ascender, formulas with ink  going above (os2.sTypoAscender + os2.sTypoLineGap – MathLeading) or with ink going below os2.sTypoDescender will result in increasing line height.}
\mathfontdimen{Axis\-Height}
{Axis height of the font. }
\mathfontdimen{Accent\-Base\-Height}
{Maximum (ink) height of accent base that does not require raising the accents. Suggested: x-height of the font (os2.sxHeight) plus any possible overshots. }
\mathfontdimen{Flattened\-Accent\-Base\-Height}
{Maximum (ink) height of accent base that does not require flattening the accents. Suggested: cap height of the font (os2.sCapHeight).}
\mathfontdimen{Subscript\-Shift\-Down}
{The standard shift down applied to subscript elements. Positive for moving in the downward direction. Suggested: os2.ySubscriptYOffset.}
\mathfontdimen{Subscript\-Top\-Max}
{Maximum allowed height of the (ink) top of subscripts that does not require moving subscripts further down. Suggested: /5 x-height.}
\mathfontdimen{Subscript\-Baseline\-Drop\-Min}
{Minimum allowed drop of the baseline of subscripts relative to the (ink) bottom of the base. Checked for bases that are treated as a box or extended shape. Positive for subscript baseline dropped below the base bottom.}
\mathfontdimen{Superscript\-Shift\-Up}
{Standard shift up applied to superscript elements. Suggested: os2.ySuperscriptYOffset.}
\mathfontdimen{Superscript\-Shift\-Up\-Cramped}
{Standard shift of superscripts relative to the base, in cramped style.}
\mathfontdimen{Superscript\-Bottom\-Min}
{Minimum allowed height of the (ink) bottom of superscripts that does not require moving subscripts further up. Suggested: ¼ x-height.}
\mathfontdimen{Superscript\-Baseline\-Drop\-Max}
{Maximum allowed drop of the baseline of superscripts relative to the (ink) top of the base. Checked for bases that are treated as a box or extended shape. Positive for superscript baseline below the base top.}
\mathfontdimen{Sub\-Superscript\-Gap\-Min}
{Minimum gap between the superscript and subscript ink. Suggested: 4×default rule thickness.}
\mathfontdimen{Superscript\-Bottom\-Max\-With\-Subscript}
{The maximum level to which the (ink) bottom of superscript can be pushed to increase the gap between superscript and subscript, before subscript starts being moved down.
Suggested: /5 x-height.}
\mathfontdimen{Space\-After\-Script}
{Extra white space to be added after each subscript and superscript. Suggested: 0.5pt for a 12 pt font.}
\mathfontdimen{Upper\-Limit\-Gap\-Min}
{Minimum gap between the (ink) bottom of the upper limit, and the (ink) top of the base operator. }
\mathfontdimen{Upper\-Limit\-Baseline\-Rise\-Min}
{Minimum distance between baseline of upper limit and (ink) top of the base operator.}
\mathfontdimen{Lower\-Limit\-Gap\-Min}
{Minimum gap between (ink) top of the lower limit, and (ink) bottom of the base operator.}
\mathfontdimen{Lower\-Limit\-Baseline\-Drop\-Min}
{Minimum distance between baseline of the lower limit and (ink) bottom of the base operator.}
\mathfontdimen{Stack\-Top\-Shift\-Up}
{Standard shift up applied to the top element of a stack.}
\mathfontdimen{Stack\-Top\-Display\-Style\-Shift\-Up}
{Standard shift up applied to the top element of a stack in display style.}
\mathfontdimen{Stack\-Bottom\-Shift\-Down}
{Standard shift down applied to the bottom element of a stack. Positive for moving in the downward direction.}
\mathfontdimen{Stack\-Bottom\-Display\-Style\-Shift\-Down}
{Standard shift down applied to the bottom element of a stack in display style. Positive for moving in the downward direction.}
\mathfontdimen{Stack\-Gap\-Min}
{Minimum gap between (ink) bottom of the top element of a stack, and the (ink) top of the bottom element. Suggested: 3×default rule thickness.}
\mathfontdimen{Stack\-Display\-Style\-Gap\-Min}
{Minimum gap between (ink) bottom of the top element of a stack, and the (ink) top of the bottom element in display style. Suggested: 7×default rule thickness.}
\mathfontdimen{Stretch\-Stack\-Top\-Shift\-Up}
{Standard shift up applied to the top element of the stretch stack.}
\mathfontdimen{Stretch\-Stack\-Bottom\-Shift\-Down}
{Standard shift down applied to the bottom element of the stretch stack. Positive for moving in the downward direction.}
\mathfontdimen{Stretch\-Stack\-Gap\-Above\-Min}
{Minimum gap between the ink of the stretched element, and the (ink) bottom of the element above. Suggested: Upper\-Limit\-Gap\-Min}
\mathfontdimen{Stretch\-Stack\-Gap\-Below\-Min}
{Minimum gap between the ink of the stretched element, and the (ink) top of the element below. Suggested: Lower\-Limit\-Gap\-Min.}
\mathfontdimen{Fraction\-Numerator\-Shift\-Up}
{Standard shift up applied to the numerator. }
\mathfontdimen{Fraction\-Numerator\-Display\-Style\-Shift\-Up}
{Standard shift up applied to the numerator in display style. Suggested: Stack\-Top\-Display\-Style\-Shift\-Up.}
\mathfontdimen{Fraction\-Denominator\-Shift\-Down}
{Standard shift down applied to the denominator. Positive for moving in the downward direction.}
\mathfontdimen{Fraction\-Denominator\-Display\-Style\-Shift\-Down}
{Standard shift down applied to the denominator in display style. Positive for moving in the downward direction. Suggested: Stack\-Bottom\-Display\-Style\-Shift\-Down.}
\mathfontdimen{Fraction\-Numerator\-Gap\-Min}
{Minimum tolerated gap between the (ink) bottom of the numerator and the ink of the fraction bar. Suggested: default rule thickness}
\mathfontdimen{Fraction\-Num\-Display\-Style\-Gap\-Min}
{Minimum tolerated gap between the (ink) bottom of the numerator and the ink of the fraction bar in display style. Suggested: 3×default rule thickness.}
\mathfontdimen{Fraction\-Rule\-Thickness}
{Thickness of the fraction bar. Suggested: default rule thickness.}
\mathfontdimen{Fraction\-Denominator\-Gap\-Min}
{Minimum tolerated gap between the (ink) top of the denominator and the ink of the fraction bar. Suggested: default rule thickness}
\mathfontdimen{Fraction\-Denom\-Display\-Style\-Gap\-Min}
{Minimum tolerated gap between the (ink) top of the denominator and the ink of the fraction bar in display style. Suggested: 3×default rule thickness.}
\mathfontdimen{Skewed\-Fraction\-Horizontal\-Gap}
{Horizontal distance between the top and bottom elements of a skewed fraction.}
\mathfontdimen{Skewed\-Fraction\-Vertical\-Gap}
{Vertical distance between the ink of the top and bottom elements of a skewed fraction.}
\mathfontdimen{Overbar\-Vertical\-Gap}
{Distance between the overbar and the (ink) top of he base. Suggested: 3×default rule thickness.}
\mathfontdimen{Overbar\-Rule\-Thickness}
{Thickness of overbar. Suggested: default rule thickness.}
\mathfontdimen{Overbar\-Extra\-Ascender}
{Extra white space reserved above the overbar. Suggested: default rule thickness.}
\mathfontdimen{Underbar\-Vertical\-Gap}
{Distance between underbar and (ink) bottom of the base. Suggested: 3×default rule thickness.}
\mathfontdimen{Underbar\-Rule\-Thickness}
{Thickness of underbar. Suggested: default rule thickness.}
\mathfontdimen{Underbar\-Extra\-Descender}
{Extra white space reserved below the underbar. Always positive. Suggested: default rule thickness.}
\mathfontdimen{Radical\-Vertical\-Gap}
{Space between the (ink) top of the expression and the bar over it. Suggested: 1¼ default rule thickness.}
\mathfontdimen{Radical\-Display\-Style\-Vertical\-Gap}
{Space between the (ink) top of the expression and the bar over it. Suggested: default rule thickness + ¼ x-height. }
\mathfontdimen{Radical\-Rule\-Thickness}
{Thickness of the radical rule. This is the thickness of the rule in designed or constructed radical signs. Suggested: default rule thickness.}
\mathfontdimen{Radical\-Extra\-Ascender}
{Extra white space reserved above the radical. Suggested: Radical\-Rule\-Thickness.}
\mathfontdimen{Radical\-Kern\-Before\-Degree}
{Extra horizontal kern before the degree of a radical, if such is present. Suggested: 5/18 of em.}
\mathfontdimen{Radical\-Kern\-After\-Degree}
{Negative kern after the degree of a radical, if such is present. Suggested: −10/18 of em.}
\mathfontdimen{Radical\-Degree\-Bottom\-Raise\-Percent}
{Height of the bottom of the radical degree, if such is present, in proportion to the ascender of the radical sign. Suggested: 60\%.}
\end{longtable}

\endinput

% /©
%
% ------------------------------------------------
% The UNICODE-MATH package  <wspr.io/unicode-math>
% ------------------------------------------------
% This package is free software and may be redistributed and/or modified under
% the conditions of the LaTeX Project Public License, version 1.3c or higher
% (your choice): <http://www.latex-project.org/lppl/>.
% ------------------------------------------------
% Copyright 2006-2018  Will Robertson, LPPL "maintainer"
% Copyright 2010-2017  Philipp Stephani
% Copyright 2011-2017  Joseph Wright
% Copyright 2012-2015  Khaled Hosny
% ------------------------------------------------
%
% ©/


==> unicode-math/um-doc-nfsssummary.tex <==
%%^^A%% um-doc-nfsssummary.tex -- part of UNICODE-MATH <wspr.io/unicode-math>

\section{Documenting maths support in the NFSS}

In the following, \meta{NFSS decl.} stands for something like |{T1}{lmr}{m}{n}|.

\begin{description}
\item[Maths symbol fonts] Fonts for symbols: $\propto$, $\leq$, $\rightarrow$

\cmd\DeclareSymbolFont\marg{name}\meta{NFSS decl.}\\
Declares a named maths font such as |operators| from which symbols are defined with \cmd\DeclareMathSymbol.

\item[Maths alphabet fonts] Fonts for {\font\1=cmmi10 at 10pt\1 ABC}\,–\,{\font\1=cmmi10 at 10pt\1 xyz}, {\font\1=eufm10 at 10pt\1 ABC}\,–\,{\font\1=cmsy10 at 10pt\1 XYZ}, etc.

\cmd\DeclareMathAlphabet\marg{cmd}\meta{NFSS decl.}

For commands such as \cmd\mathbf, accessed
through maths mode that are unaffected by the current text font, and which are used for
alphabetic symbols in the \ascii\ range.

\cmd\DeclareSymbolFontAlphabet\marg{cmd}\marg{name}

Alternative (and optimisation) for \cmd\DeclareMathAlphabet\ if a single font is being used
for both alphabetic characters (as above) and symbols.

\item[Maths `versions'] Different maths weights can be defined with the following, switched
in text with the \cmd\mathversion\marg{maths version} command.

\cmd\SetSymbolFont\marg{name}\marg{maths version}\meta{NFSS decl.}\\
\cmd\SetMathAlphabet\marg{cmd}\marg{maths version}\meta{NFSS decl.}

\item[Maths symbols] Symbol definitions in maths for both characters (=) and macros (\cmd\eqdef):
\cmd\DeclareMathSymbol\marg{symbol}\marg{type}\marg{named font}\marg{slot}
This is the macro that actually defines which font each symbol comes from and how they behave.
\end{description}
Delimiters and radicals use wrappers around \TeX's \cmd\delimiter/\cmd\radical\ primitives,
which are re-designed in \XeTeX. The syntax used in \LaTeX's NFSS is therefore not so relevant here.
\begin{description}
\item[Delimiters] A special class of maths symbol which enlarge themselves in certain contexts.

\cmd\DeclareMathDelimiter\marg{symbol}\marg{type}\marg{sym.\ font}\marg{slot}\marg{sym.\ font}\marg{slot}

\item[Radicals] Similar to delimiters (\cmd\DeclareMathRadical\ takes the same syntax) but
behave `weirdly'.
\end{description}
In those cases, glyph slots in \emph{two} symbol fonts are required; one for the small (`regular') case,
the other for situations when the glyph is larger. This is not the case in \XeTeX.

Accents are not included yet.

\paragraph{Summary}

For symbols, something like:
\begin{Verbatim}
\def\DeclareMathSymbol#1#2#3#4{
  \global\mathchardef#1"\mathchar@type#2
    \expandafter\hexnumber@\csname sym#2\endcsname
    {\hexnumber@{\count\z@}\hexnumber@{\count\tw@}}}
\end{Verbatim}
For characters, something like:
\begin{Verbatim}
\def\DeclareMathSymbol#1#2#3#4{
  \global\mathcode`#1"\mathchar@type#2
    \expandafter\hexnumber@\csname sym#2\endcsname
    {\hexnumber@{\count\z@}\hexnumber@{\count\tw@}}}
\end{Verbatim}
\endinput

% /©
%
% ------------------------------------------------
% The UNICODE-MATH package  <wspr.io/unicode-math>
% ------------------------------------------------
% This package is free software and may be redistributed and/or modified under
% the conditions of the LaTeX Project Public License, version 1.3c or higher
% (your choice): <http://www.latex-project.org/lppl/>.
% ------------------------------------------------
% Copyright 2006-2018  Will Robertson, LPPL "maintainer"
% Copyright 2010-2017  Philipp Stephani
% Copyright 2011-2017  Joseph Wright
% Copyright 2012-2015  Khaled Hosny
% ------------------------------------------------
%
% ©/


==> unicode-math/um-doc-stixextract.tex <==
%%^^A%% um-doc-stixextract.tex -- part of UNICODE-MATH <wspr.io/unicode-math>

\section{\STIX\ table data extraction}\label{part:awk}

The source for the \TeX\ names for the very large number of mathematical
glyphs are provided via Barbara Beeton's table file for the \STIX\ project
(|ams.org/STIX|). A version is located at
|http://www.ams.org/STIX/bnb/stix-tbl.asc|
but check |http://www.ams.org/STIX/| for more up-to-date info.

This table is converted into a form suitable for reading by \TeX.
A single file is produced containing all (more than 3298) symbols.
Future optimisations might include generating various (possibly overlapping) subsets
so not all definitions must be read just to redefine a small range of symbols.
Performance for now seems to be acceptable without such measures.

This file is currently developed outside this DTX file. It will be
incorporated when the final version is ready. (I know this is not how
things are supposed to work!)

\endinput

% /©
%
% ------------------------------------------------
% The UNICODE-MATH package  <wspr.io/unicode-math>
% ------------------------------------------------
% This package is free software and may be redistributed and/or modified under
% the conditions of the LaTeX Project Public License, version 1.3c or higher
% (your choice): <http://www.latex-project.org/lppl/>.
% ------------------------------------------------
% Copyright 2006-2018  Will Robertson, LPPL "maintainer"
% Copyright 2010-2017  Philipp Stephani
% Copyright 2011-2017  Joseph Wright
% Copyright 2012-2015  Khaled Hosny
% ------------------------------------------------
%
% ©/


==> unicode-math/um-doc-style.tex <==
%%^^A%% um-doc-style.tex -- part of UNICODE-MATH <wspr.io/unicode-math>

\makeatletter
\input{unicode-math.dtx}
\GetFileInfo{unicode-math.dtx}
\let\umfiledate\filedate
\let\umfileversion\fileversion

\CheckSum{0}
\EnableCrossrefs
\CodelineIndex
\setcounter{IndexColumns}{2}

\usepackage[svgnames]{xcolor}
\usepackage[inline]{enumitem}
\usepackage{amsmath,array,booktabs,calc,enumitem,fancyvrb,graphicx,ifthen,longtable,refstyle,subfig,topcapt,url,varioref,underscore}
\setcounter{LTchunksize}{100}
\usepackage[slash-delimiter=frac,nabla=literal]{unicode-math}
\usepackage{metalogo,hologo}

\fvset{fontsize=\small,xleftmargin=2em}
\usepackage[it]{titlesec}

\setmainfont{texgyrepagella}%
 [
  Extension = .otf ,
  UprightFont = *-regular ,
  ItalicFont = *-italic ,
  BoldFont = *-bold ,
  BoldItalicFont = *-bolditalic ,
 ]
\setsansfont{Iwona}%
 [
  Scale=MatchLowercase,
  Extension = .otf,
  UprightFont = *-Regular,
  ItalicFont  = *-Italic,
  BoldFont    = *-Bold,
  BoldItalicFont = *-BoldItalic,
 ]
\setmonofont{Inconsolatazi4-Regular.otf}%
 [
  Scale=MatchLowercase,
  BoldFont=Inconsolatazi4-Bold.otf
 ]

\setmathfont{texgyrepagella-math.otf}
\setmathfont[version=xits]{xits-math.otf}
\newfontface\umfont{xits-math.otf}

\usepackage{hypdoc}
\hypersetup{linktocpage}

% work around some issue turning | into "j" inside mathsf in the definition of \Module:
% (also prettify)
\def\Module#1{{\footnotesize\color{red}$\langle$\texttt{#1}$\rangle$}}

\linespread{1.1}
\frenchspacing

\definecolor{niceblue}{rgb}{0.2,0.4,0.8}

\def\theCodelineNo{\textcolor{niceblue}{\sffamily\tiny\arabic{CodelineNo}}}

\newcommand*\name[1]{{#1}}
\newcommand*\pkg[1]{\textsf{#1}}
\newcommand*\feat[1]{\texttt{#1}}
\newcommand*\opt[1]{\texttt{#1}}

\newcommand*\note[1]{\unskip\footnote{#1}}

\let\latin\textit
\def\eg{\latin{e.g.}}
\def\Eg{\latin{E.g.}}
\def\ie{\latin{i.e.}}
\def\etc{\@ifnextchar.{\latin{etc}}{\latin{etc.}\@}}

\def\STIX{\textsc{stix}}
\def\MacOSX{Mac~OS~X}
\def\ascii{\textsc{ascii}}
\def\OMEGA{Omega}

\newcounter{argument}

\makeatletter
\g@addto@macro\endmacro{\setcounter{argument}{0}}
\makeatother

\newcommand*\darg[1]{%
  \stepcounter{argument}%
  {\ttfamily\char`\#\theargument~:~}#1\par\noindent\ignorespaces
}
\newcommand*\doarg[1]{%
  \stepcounter{argument}%
  {\ttfamily\makebox[0pt][r]{[}\char`\#\theargument]:~}#1\par\noindent\ignorespaces
}

\newcommand\codeline[1]{\par{\centering#1\par\noindent}\ignorespaces}

\newcommand\unichar[1]{\textsc{u}+\texttt{\small#1}}

\setlength\parindent{2em}

\def \MakePrivateLetters {%
  \catcode`\@=11\relax
  \catcode`\_=11\relax
  \catcode`\:=11\relax
}

\makeatother

\endinput

% /©
%
% ------------------------------------------------
% The UNICODE-MATH package  <wspr.io/unicode-math>
% ------------------------------------------------
% This package is free software and may be redistributed and/or modified under
% the conditions of the LaTeX Project Public License, version 1.3c or higher
% (your choice): <http://www.latex-project.org/lppl/>.
% ------------------------------------------------
% Copyright 2006-2018  Will Robertson, LPPL "maintainer"
% Copyright 2010-2017  Philipp Stephani
% Copyright 2011-2017  Joseph Wright
% Copyright 2012-2015  Khaled Hosny
% ------------------------------------------------
%
% ©/


==> unicode-math/unicode-math-table.tex <==
%%^^A%% unicode-math-table.tex -- part of UNICODE-MATH <wspr.io/unicode-math>
%%^^A%% Source file of the math symbols.

\UnicodeMathSymbol{"00021}{\mathexclam               }{\mathclose}{exclamation mark}%
\UnicodeMathSymbol{"00023}{\mathoctothorpe           }{\mathord}{number sign}%
\UnicodeMathSymbol{"00024}{\mathdollar               }{\mathord}{dollar sign}%
\UnicodeMathSymbol{"00025}{\mathpercent              }{\mathord}{percent sign}%
\UnicodeMathSymbol{"00026}{\mathampersand            }{\mathord}{ampersand}%
\UnicodeMathSymbol{"00028}{\lparen                   }{\mathopen}{left parenthesis}%
\UnicodeMathSymbol{"00029}{\rparen                   }{\mathclose}{right parenthesis}%
\UnicodeMathSymbol{"0002B}{\mathplus                 }{\mathbin}{plus sign b:}%
\UnicodeMathSymbol{"0002C}{\mathcomma                }{\mathpunct}{comma}%
\UnicodeMathSymbol{"0002E}{\mathperiod               }{\mathord}{full stop, period}%
\UnicodeMathSymbol{"0002F}{\mathslash                }{\mathord}{solidus}%
\UnicodeMathSymbol{"0003A}{\mathcolon                }{\mathpunct}{colon}%
\UnicodeMathSymbol{"0003B}{\mathsemicolon            }{\mathpunct}{semicolon p:}%
\UnicodeMathSymbol{"0003C}{\less                     }{\mathrel}{less-than sign r:}%
\UnicodeMathSymbol{"0003D}{\equal                    }{\mathrel}{equals sign r:}%
\UnicodeMathSymbol{"0003E}{\greater                  }{\mathrel}{greater-than sign r:}%
\UnicodeMathSymbol{"0003F}{\mathquestion             }{\mathord}{question mark}%
\UnicodeMathSymbol{"00040}{\mathatsign               }{\mathord}{commercial at}%
\UnicodeMathSymbol{"0005B}{\lbrack                   }{\mathopen}{left square bracket}%
\UnicodeMathSymbol{"0005C}{\backslash                }{\mathord}{reverse solidus}%
\UnicodeMathSymbol{"0005D}{\rbrack                   }{\mathclose}{right square bracket}%
\UnicodeMathSymbol{"0007B}{\lbrace                   }{\mathopen}{left curly bracket}%
\UnicodeMathSymbol{"0007C}{\vert                     }{\mathfence}{vertical bar}%
\UnicodeMathSymbol{"0007D}{\rbrace                   }{\mathclose}{right curly bracket}%
\UnicodeMathSymbol{"000A3}{\mathsterling             }{\mathord}{pound sign}%
\UnicodeMathSymbol{"000A5}{\mathyen                  }{\mathord}{yen sign}%
\UnicodeMathSymbol{"000A7}{\mathsection              }{\mathord}{section symbol}%
\UnicodeMathSymbol{"000AC}{\neg                      }{\mathord}{/neg /lnot not sign}%
\UnicodeMathSymbol{"000B1}{\pm                       }{\mathbin}{plus-or-minus sign}%
\UnicodeMathSymbol{"000B6}{\mathparagraph            }{\mathord}{paragraph symbol}%
\UnicodeMathSymbol{"000B7}{\cdotp                    }{\mathbin}{/centerdot b: middle dot}%
\UnicodeMathSymbol{"000D7}{\times                    }{\mathbin}{multiply sign}%
\UnicodeMathSymbol{"000F0}{\matheth                  }{\mathalpha}{eth}%
\UnicodeMathSymbol{"000F7}{\div                      }{\mathbin}{divide sign}%
\UnicodeMathSymbol{"001B5}{\Zbar                     }{\mathord}{impedance (latin capital letter z with stroke)}%
\UnicodeMathSymbol{"00300}{\grave                    }{\mathaccent}{grave accent}%
\UnicodeMathSymbol{"00301}{\acute                    }{\mathaccent}{acute accent}%
\UnicodeMathSymbol{"00302}{\hat                      }{\mathaccent}{circumflex accent}%
\UnicodeMathSymbol{"00302}{\widehat                  }{\mathaccentwide}{circumflex accent}%
\UnicodeMathSymbol{"00303}{\tilde                    }{\mathaccent}{tilde}%
\UnicodeMathSymbol{"00303}{\widetilde                }{\mathaccentwide}{tilde}%
\UnicodeMathSymbol{"00304}{\bar                      }{\mathaccent}{macron}%
\UnicodeMathSymbol{"00305}{\overbar                  }{\mathaccent}{overbar embellishment}%
\UnicodeMathSymbol{"00305}{\wideoverbar              }{\mathaccentwide}{stretchy overbar embellishment}%
\UnicodeMathSymbol{"00306}{\breve                    }{\mathaccent}{breve}%
\UnicodeMathSymbol{"00306}{\widebreve                }{\mathaccentwide}{stretchy breve}%
\UnicodeMathSymbol{"00307}{\dot                      }{\mathaccent}{dot above}%
\UnicodeMathSymbol{"00308}{\ddot                     }{\mathaccent}{dieresis}%
\UnicodeMathSymbol{"00309}{\ovhook                   }{\mathaccent}{combining hook above}%
\UnicodeMathSymbol{"0030A}{\ocirc                    }{\mathaccent}{ring}%
\UnicodeMathSymbol{"0030C}{\check                    }{\mathaccent}{caron}%
\UnicodeMathSymbol{"0030C}{\widecheck                }{\mathaccentwide}{stretchy caron}%
\UnicodeMathSymbol{"00310}{\candra                   }{\mathaccent}{candrabindu (non-spacing)}%
\UnicodeMathSymbol{"00312}{\oturnedcomma             }{\mathaccent}{combining turned comma above}%
\UnicodeMathSymbol{"00315}{\ocommatopright           }{\mathaccent}{combining comma above right}%
\UnicodeMathSymbol{"0031A}{\droang                   }{\mathaccent}{left angle above (non-spacing)}%
\UnicodeMathSymbol{"00330}{\wideutilde               }{\mathbotaccentwide}{under tilde accent (multiple characters and non-spacing)}%
\UnicodeMathSymbol{"00332}{\mathunderbar             }{\mathbotaccentwide}{combining low line}%
\UnicodeMathSymbol{"00338}{\notaccent                }{\mathaccentoverlay}{combining long solidus overlay}%
\UnicodeMathSymbol{"0034D}{\underleftrightarrow      }{\mathbotaccentwide}{underleftrightarrow accent}%
\UnicodeMathSymbol{"00391}{\mupAlpha                 }{\mathalpha}{capital alpha, greek}%
\UnicodeMathSymbol{"00392}{\mupBeta                  }{\mathalpha}{capital beta, greek}%
\UnicodeMathSymbol{"00393}{\mupGamma                 }{\mathalpha}{capital gamma, greek}%
\UnicodeMathSymbol{"00394}{\mupDelta                 }{\mathalpha}{capital delta, greek}%
\UnicodeMathSymbol{"00395}{\mupEpsilon               }{\mathalpha}{capital epsilon, greek}%
\UnicodeMathSymbol{"00396}{\mupZeta                  }{\mathalpha}{capital zeta, greek}%
\UnicodeMathSymbol{"00397}{\mupEta                   }{\mathalpha}{capital eta, greek}%
\UnicodeMathSymbol{"00398}{\mupTheta                 }{\mathalpha}{capital theta, greek}%
\UnicodeMathSymbol{"00399}{\mupIota                  }{\mathalpha}{capital iota, greek}%
\UnicodeMathSymbol{"0039A}{\mupKappa                 }{\mathalpha}{capital kappa, greek}%
\UnicodeMathSymbol{"0039B}{\mupLambda                }{\mathalpha}{capital lambda, greek}%
\UnicodeMathSymbol{"0039C}{\mupMu                    }{\mathalpha}{capital mu, greek}%
\UnicodeMathSymbol{"0039D}{\mupNu                    }{\mathalpha}{capital nu, greek}%
\UnicodeMathSymbol{"0039E}{\mupXi                    }{\mathalpha}{capital xi, greek}%
\UnicodeMathSymbol{"0039F}{\mupOmicron               }{\mathalpha}{capital omicron, greek}%
\UnicodeMathSymbol{"003A0}{\mupPi                    }{\mathalpha}{capital pi, greek}%
\UnicodeMathSymbol{"003A1}{\mupRho                   }{\mathalpha}{capital rho, greek}%
\UnicodeMathSymbol{"003A3}{\mupSigma                 }{\mathalpha}{capital sigma, greek}%
\UnicodeMathSymbol{"003A4}{\mupTau                   }{\mathalpha}{capital tau, greek}%
\UnicodeMathSymbol{"003A5}{\mupUpsilon               }{\mathalpha}{capital upsilon, greek}%
\UnicodeMathSymbol{"003A6}{\mupPhi                   }{\mathalpha}{capital phi, greek}%
\UnicodeMathSymbol{"003A7}{\mupChi                   }{\mathalpha}{capital chi, greek}%
\UnicodeMathSymbol{"003A8}{\mupPsi                   }{\mathalpha}{capital psi, greek}%
\UnicodeMathSymbol{"003A9}{\mupOmega                 }{\mathalpha}{capital omega, greek}%
\UnicodeMathSymbol{"003B1}{\mupalpha                 }{\mathalpha}{small alpha, greek}%
\UnicodeMathSymbol{"003B2}{\mupbeta                  }{\mathalpha}{small beta, greek}%
\UnicodeMathSymbol{"003B3}{\mupgamma                 }{\mathalpha}{small gamma, greek}%
\UnicodeMathSymbol{"003B4}{\mupdelta                 }{\mathalpha}{small delta, greek}%
\UnicodeMathSymbol{"003B5}{\mupvarepsilon            }{\mathalpha}{rounded small varepsilon    , greek}%
\UnicodeMathSymbol{"003B6}{\mupzeta                  }{\mathalpha}{small zeta, greek}%
\UnicodeMathSymbol{"003B7}{\mupeta                   }{\mathalpha}{small eta, greek}%
\UnicodeMathSymbol{"003B8}{\muptheta                 }{\mathalpha}{straight theta, small theta, greek}%
\UnicodeMathSymbol{"003B9}{\mupiota                  }{\mathalpha}{small iota, greek}%
\UnicodeMathSymbol{"003BA}{\mupkappa                 }{\mathalpha}{small kappa, greek}%
\UnicodeMathSymbol{"003BB}{\muplambda                }{\mathalpha}{small lambda, greek}%
\UnicodeMathSymbol{"003BC}{\mupmu                    }{\mathalpha}{small mu, greek}%
\UnicodeMathSymbol{"003BD}{\mupnu                    }{\mathalpha}{small nu, greek}%
\UnicodeMathSymbol{"003BE}{\mupxi                    }{\mathalpha}{small xi, greek}%
\UnicodeMathSymbol{"003BF}{\mupomicron               }{\mathalpha}{small omicron, greek}%
\UnicodeMathSymbol{"003C0}{\muppi                    }{\mathalpha}{small pi, greek}%
\UnicodeMathSymbol{"003C1}{\muprho                   }{\mathalpha}{small rho, greek}%
\UnicodeMathSymbol{"003C2}{\mupvarsigma              }{\mathalpha}{terminal sigma, greek}%
\UnicodeMathSymbol{"003C3}{\mupsigma                 }{\mathalpha}{small sigma, greek}%
\UnicodeMathSymbol{"003C4}{\muptau                   }{\mathalpha}{small tau, greek}%
\UnicodeMathSymbol{"003C5}{\mupupsilon               }{\mathalpha}{small upsilon, greek}%
\UnicodeMathSymbol{"003C6}{\mupvarphi                }{\mathalpha}{curly or open small phi, greek}%
\UnicodeMathSymbol{"003C7}{\mupchi                   }{\mathalpha}{small chi, greek}%
\UnicodeMathSymbol{"003C8}{\muppsi                   }{\mathalpha}{small psi, greek}%
\UnicodeMathSymbol{"003C9}{\mupomega                 }{\mathalpha}{small omega, greek}%
\UnicodeMathSymbol{"003D1}{\mupvartheta              }{\mathalpha}{/vartheta - curly or open theta}%
\UnicodeMathSymbol{"003D5}{\mupphi                   }{\mathalpha}{/straightphi - small phi, greek}%
\UnicodeMathSymbol{"003D6}{\mupvarpi                 }{\mathalpha}{rounded small pi (pomega), greek}%
\UnicodeMathSymbol{"003DC}{\upDigamma                }{\mathalpha}{capital digamma}%
\UnicodeMathSymbol{"003DD}{\updigamma                }{\mathalpha}{old greek small letter digamma}%
\UnicodeMathSymbol{"003F0}{\mupvarkappa              }{\mathalpha}{rounded small kappa, greek}%
\UnicodeMathSymbol{"003F1}{\mupvarrho                }{\mathalpha}{rounded small rho, greek}%
\UnicodeMathSymbol{"003F4}{\mupvarTheta              }{\mathalpha}{greek capital theta symbol}%
\UnicodeMathSymbol{"003F5}{\mupepsilon               }{\mathalpha}{greek lunate varepsilon symbol}%
\UnicodeMathSymbol{"003F6}{\upbackepsilon            }{\mathord}{greek reversed lunate epsilon symbol}%
\UnicodeMathSymbol{"02010}{\mathhyphen               }{\mathalpha}{hyphen}%
\UnicodeMathSymbol{"02015}{\horizbar                 }{\mathord}{horizontal bar}%
\UnicodeMathSymbol{"02016}{\Vert                     }{\mathfence}{double vertical bar}%
\UnicodeMathSymbol{"02017}{\twolowline               }{\mathord}{double low line (spacing)}%
\UnicodeMathSymbol{"02020}{\dagger                   }{\mathbin}{dagger relation}%
\UnicodeMathSymbol{"02021}{\ddagger                  }{\mathbin}{double dagger relation}%
\UnicodeMathSymbol{"02022}{\smblkcircle              }{\mathbin}{/bullet b: round bullet, filled}%
\UnicodeMathSymbol{"02025}{\enleadertwodots          }{\mathord}{double baseline dot (en leader)}%
\UnicodeMathSymbol{"02026}{\unicodeellipsis          }{\mathord}{ellipsis (horizontal)}%
\UnicodeMathSymbol{"02032}{\prime                    }{\mathord}{prime or minute, not superscripted}%
\UnicodeMathSymbol{"02033}{\dprime                   }{\mathord}{double prime or second, not superscripted}%
\UnicodeMathSymbol{"02034}{\trprime                  }{\mathord}{triple prime (not superscripted)}%
\UnicodeMathSymbol{"02035}{\backprime                }{\mathord}{reverse prime, not superscripted}%
\UnicodeMathSymbol{"02036}{\backdprime               }{\mathord}{double reverse prime, not superscripted}%
\UnicodeMathSymbol{"02037}{\backtrprime              }{\mathord}{triple reverse prime, not superscripted}%
\UnicodeMathSymbol{"02038}{\caretinsert              }{\mathord}{caret (insertion mark)}%
\UnicodeMathSymbol{"0203C}{\Exclam                   }{\mathord}{double exclamation mark}%
\UnicodeMathSymbol{"02040}{\tieconcat                }{\mathbin}{character tie, z notation sequence concatenation}%
\UnicodeMathSymbol{"02043}{\hyphenbullet             }{\mathord}{rectangle, filled (hyphen bullet)}%
\UnicodeMathSymbol{"02044}{\fracslash                }{\mathbin}{fraction slash}%
\UnicodeMathSymbol{"02047}{\Question                 }{\mathord}{double question mark}%
\UnicodeMathSymbol{"02050}{\closure                  }{\mathrel}{close up}%
\UnicodeMathSymbol{"02057}{\qprime                   }{\mathord}{quadruple prime, not superscripted}%
\UnicodeMathSymbol{"020AC}{\euro                     }{\mathord}{euro sign}%
\UnicodeMathSymbol{"020D0}{\leftharpoonaccent        }{\mathaccent}{combining left harpoon above}%
\UnicodeMathSymbol{"020D0}{\overleftharpoon          }{\mathaccentwide}{combining left harpoon above}%
\UnicodeMathSymbol{"020D1}{\rightharpoonaccent       }{\mathaccent}{combining right harpoon above}%
\UnicodeMathSymbol{"020D1}{\overrightharpoon         }{\mathaccentwide}{combining right harpoon above}%
\UnicodeMathSymbol{"020D2}{\vertoverlay              }{\mathaccent}{combining long vertical line overlay}%
\UnicodeMathSymbol{"020D6}{\overleftarrow            }{\mathaccentwide}{combining left arrow above}%
\UnicodeMathSymbol{"020D7}{\overrightarrow           }{\mathaccentwide}{combining left arrow above}%
\UnicodeMathSymbol{"020D7}{\vec                      }{\mathaccent}{combining right arrow above}%
\UnicodeMathSymbol{"020DB}{\dddot                    }{\mathaccent}{combining three dots above}%
\UnicodeMathSymbol{"020DC}{\ddddot                   }{\mathaccent}{combining four dots above}%
\UnicodeMathSymbol{"020DD}{\enclosecircle            }{\mathord}{combining enclosing circle}%
\UnicodeMathSymbol{"020DE}{\enclosesquare            }{\mathord}{combining enclosing square}%
\UnicodeMathSymbol{"020DF}{\enclosediamond           }{\mathord}{combining enclosing diamond}%
\UnicodeMathSymbol{"020E1}{\overleftrightarrow       }{\mathaccentwide}{combining left right arrow above}%
\UnicodeMathSymbol{"020E4}{\enclosetriangle          }{\mathord}{combining enclosing upward pointing triangle}%
\UnicodeMathSymbol{"020E7}{\annuity                  }{\mathaccent}{combining annuity symbol}%
\UnicodeMathSymbol{"020E8}{\threeunderdot            }{\mathbotaccent}{combining triple underdot}%
\UnicodeMathSymbol{"020E9}{\widebridgeabove          }{\mathaccent}{combining wide bridge above}%
\UnicodeMathSymbol{"020EC}{\underrightharpoondown    }{\mathbotaccentwide}{combining rightwards harpoon with barb downwards}%
\UnicodeMathSymbol{"020ED}{\underleftharpoondown     }{\mathbotaccentwide}{combining leftwards harpoon with barb downwards}%
\UnicodeMathSymbol{"020EE}{\underleftarrow           }{\mathbotaccentwide}{combining left arrow below}%
\UnicodeMathSymbol{"020EF}{\underrightarrow          }{\mathbotaccentwide}{combining right arrow below}%
\UnicodeMathSymbol{"020F0}{\asteraccent              }{\mathaccent}{combining asterisk above}%
\UnicodeMathSymbol{"02102}{\BbbC                     }{\mathalpha}{/bbb c, open face c}%
\UnicodeMathSymbol{"02107}{\Eulerconst               }{\mathord}{euler constant}%
\UnicodeMathSymbol{"0210A}{\mscrg                    }{\mathalpha}{/scr g, script letter g}%
\UnicodeMathSymbol{"0210B}{\mscrH                    }{\mathalpha}{hamiltonian (script capital h)}%
\UnicodeMathSymbol{"0210C}{\mfrakH                   }{\mathalpha}{/frak h, upper case h}%
\UnicodeMathSymbol{"0210D}{\BbbH                     }{\mathalpha}{/bbb h, open face h}%
\UnicodeMathSymbol{"0210E}{\Planckconst              }{\mathord}{planck constant}%
\UnicodeMathSymbol{"0210F}{\hslash                   }{\mathalpha}{/hslash - variant planck's over 2pi}%
\UnicodeMathSymbol{"02110}{\mscrI                    }{\mathalpha}{/scr i, script letter i}%
\UnicodeMathSymbol{"02111}{\Im                       }{\mathalpha}{imaginary part}%
\UnicodeMathSymbol{"02112}{\mscrL                    }{\mathalpha}{lagrangian (script capital l)}%
\UnicodeMathSymbol{"02113}{\ell                      }{\mathalpha}{cursive small l}%
\UnicodeMathSymbol{"02115}{\BbbN                     }{\mathalpha}{/bbb n, open face n}%
\UnicodeMathSymbol{"02118}{\wp                       }{\mathalpha}{weierstrass p}%
\UnicodeMathSymbol{"02119}{\BbbP                     }{\mathalpha}{/bbb p, open face p}%
\UnicodeMathSymbol{"0211A}{\BbbQ                     }{\mathalpha}{/bbb q, open face q}%
\UnicodeMathSymbol{"0211B}{\mscrR                    }{\mathalpha}{/scr r, script letter r}%
\UnicodeMathSymbol{"0211C}{\Re                       }{\mathalpha}{real part}%
\UnicodeMathSymbol{"0211D}{\BbbR                     }{\mathalpha}{/bbb r, open face r}%
\UnicodeMathSymbol{"02124}{\BbbZ                     }{\mathalpha}{/bbb z, open face z}%
\UnicodeMathSymbol{"02127}{\mho                      }{\mathord}{conductance}%
\UnicodeMathSymbol{"02128}{\mfrakZ                   }{\mathalpha}{/frak z, upper case z}%
\UnicodeMathSymbol{"02129}{\turnediota               }{\mathalpha}{turned iota}%
\UnicodeMathSymbol{"0212B}{\Angstrom                 }{\mathalpha}{angstrom capital a, ring}%
\UnicodeMathSymbol{"0212C}{\mscrB                    }{\mathalpha}{bernoulli function (script capital b)}%
\UnicodeMathSymbol{"0212D}{\mfrakC                   }{\mathalpha}{black-letter capital c}%
\UnicodeMathSymbol{"0212F}{\mscre                    }{\mathalpha}{/scr e, script letter e}%
\UnicodeMathSymbol{"02130}{\mscrE                    }{\mathalpha}{/scr e, script letter e}%
\UnicodeMathSymbol{"02131}{\mscrF                    }{\mathalpha}{/scr f, script letter f}%
\UnicodeMathSymbol{"02132}{\Finv                     }{\mathord}{turned capital f}%
\UnicodeMathSymbol{"02133}{\mscrM                    }{\mathalpha}{physics m-matrix (script capital m)}%
\UnicodeMathSymbol{"02134}{\mscro                    }{\mathalpha}{order of (script small o)}%
\UnicodeMathSymbol{"02135}{\aleph                    }{\mathalpha}{aleph, hebrew}%
\UnicodeMathSymbol{"02136}{\beth                     }{\mathalpha}{beth, hebrew}%
\UnicodeMathSymbol{"02137}{\gimel                    }{\mathalpha}{gimel, hebrew}%
\UnicodeMathSymbol{"02138}{\daleth                   }{\mathalpha}{daleth, hebrew}%
\UnicodeMathSymbol{"0213C}{\Bbbpi                    }{\mathord}{double-struck small pi}%
\UnicodeMathSymbol{"0213D}{\Bbbgamma                 }{\mathalpha}{double-struck small gamma}%
\UnicodeMathSymbol{"0213E}{\BbbGamma                 }{\mathalpha}{double-struck capital gamma}%
\UnicodeMathSymbol{"0213F}{\BbbPi                    }{\mathalpha}{double-struck capital pi}%
\UnicodeMathSymbol{"02140}{\Bbbsum                   }{\mathop}{double-struck n-ary summation}%
\UnicodeMathSymbol{"02141}{\Game                     }{\mathord}{turned sans-serif capital g}%
\UnicodeMathSymbol{"02142}{\sansLturned              }{\mathord}{turned sans-serif capital l}%
\UnicodeMathSymbol{"02143}{\sansLmirrored            }{\mathord}{reversed sans-serif capital l}%
\UnicodeMathSymbol{"02144}{\Yup                      }{\mathord}{turned sans-serif capital y}%
\UnicodeMathSymbol{"02145}{\mitBbbD                  }{\mathord}{double-struck italic capital d}%
\UnicodeMathSymbol{"02146}{\mitBbbd                  }{\mathord}{double-struck italic small d}%
\UnicodeMathSymbol{"02147}{\mitBbbe                  }{\mathord}{double-struck italic small e}%
\UnicodeMathSymbol{"02148}{\mitBbbi                  }{\mathord}{double-struck italic small i}%
\UnicodeMathSymbol{"02149}{\mitBbbj                  }{\mathord}{double-struck italic small j}%
\UnicodeMathSymbol{"0214A}{\PropertyLine             }{\mathord}{property line}%
\UnicodeMathSymbol{"0214B}{\upand                    }{\mathbin}{turned ampersand}%
\UnicodeMathSymbol{"02190}{\leftarrow                }{\mathrel}{/leftarrow /gets a: leftward arrow}%
\UnicodeMathSymbol{"02191}{\uparrow                  }{\mathrel}{upward arrow}%
\UnicodeMathSymbol{"02192}{\rightarrow               }{\mathrel}{/rightarrow /to a: rightward arrow}%
\UnicodeMathSymbol{"02193}{\downarrow                }{\mathrel}{downward arrow}%
\UnicodeMathSymbol{"02194}{\leftrightarrow           }{\mathrel}{left and right arrow}%
\UnicodeMathSymbol{"02195}{\updownarrow              }{\mathrel}{up and down arrow}%
\UnicodeMathSymbol{"02196}{\nwarrow                  }{\mathrel}{nw pointing arrow}%
\UnicodeMathSymbol{"02197}{\nearrow                  }{\mathrel}{ne pointing arrow}%
\UnicodeMathSymbol{"02198}{\searrow                  }{\mathrel}{se pointing arrow}%
\UnicodeMathSymbol{"02199}{\swarrow                  }{\mathrel}{sw pointing arrow}%
\UnicodeMathSymbol{"0219A}{\nleftarrow               }{\mathrel}{not left arrow}%
\UnicodeMathSymbol{"0219B}{\nrightarrow              }{\mathrel}{not right arrow}%
\UnicodeMathSymbol{"0219C}{\leftwavearrow            }{\mathrel}{left arrow-wavy}%
\UnicodeMathSymbol{"0219D}{\rightwavearrow           }{\mathrel}{right arrow-wavy}%
\UnicodeMathSymbol{"0219E}{\twoheadleftarrow         }{\mathrel}{left two-headed arrow}%
\UnicodeMathSymbol{"0219F}{\twoheaduparrow           }{\mathrel}{up two-headed arrow}%
\UnicodeMathSymbol{"021A0}{\twoheadrightarrow        }{\mathrel}{right two-headed arrow}%
\UnicodeMathSymbol{"021A1}{\twoheaddownarrow         }{\mathrel}{down two-headed arrow}%
\UnicodeMathSymbol{"021A2}{\leftarrowtail            }{\mathrel}{left arrow-tailed}%
\UnicodeMathSymbol{"021A3}{\rightarrowtail           }{\mathrel}{right arrow-tailed}%
\UnicodeMathSymbol{"021A4}{\mapsfrom                 }{\mathrel}{maps to, leftward}%
\UnicodeMathSymbol{"021A5}{\mapsup                   }{\mathrel}{maps to, upward}%
\UnicodeMathSymbol{"021A6}{\mapsto                   }{\mathrel}{maps to, rightward}%
\UnicodeMathSymbol{"021A7}{\mapsdown                 }{\mathrel}{maps to, downward}%
\UnicodeMathSymbol{"021A8}{\updownarrowbar           }{\mathord}{up down arrow with base (perpendicular)}%
\UnicodeMathSymbol{"021A9}{\hookleftarrow            }{\mathrel}{left arrow-hooked}%
\UnicodeMathSymbol{"021AA}{\hookrightarrow           }{\mathrel}{right arrow-hooked}%
\UnicodeMathSymbol{"021AB}{\looparrowleft            }{\mathrel}{left arrow-looped}%
\UnicodeMathSymbol{"021AC}{\looparrowright           }{\mathrel}{right arrow-looped}%
\UnicodeMathSymbol{"021AD}{\leftrightsquigarrow      }{\mathrel}{left and right arr-wavy}%
\UnicodeMathSymbol{"021AE}{\nleftrightarrow          }{\mathrel}{not left and right arrow}%
\UnicodeMathSymbol{"021AF}{\downzigzagarrow          }{\mathrel}{downwards zigzag arrow}%
\UnicodeMathSymbol{"021B0}{\Lsh                      }{\mathrel}{/lsh a:}%
\UnicodeMathSymbol{"021B1}{\Rsh                      }{\mathrel}{/rsh a:}%
\UnicodeMathSymbol{"021B2}{\Ldsh                     }{\mathrel}{left down angled arrow}%
\UnicodeMathSymbol{"021B3}{\Rdsh                     }{\mathrel}{right down angled arrow}%
\UnicodeMathSymbol{"021B4}{\linefeed                 }{\mathord}{rightwards arrow with corner downwards}%
\UnicodeMathSymbol{"021B5}{\carriagereturn           }{\mathord}{downwards arrow with corner leftward = carriage return}%
\UnicodeMathSymbol{"021B6}{\curvearrowleft           }{\mathrel}{left curved arrow}%
\UnicodeMathSymbol{"021B7}{\curvearrowright          }{\mathrel}{right curved arrow}%
\UnicodeMathSymbol{"021B8}{\barovernorthwestarrow    }{\mathord}{north west arrow to long bar}%
\UnicodeMathSymbol{"021B9}{\barleftarrowrightarrowbar}{\mathord}{leftwards arrow to bar over rightwards arrow to bar}%
\UnicodeMathSymbol{"021BA}{\acwopencirclearrow       }{\mathord}{anticlockwise open circle arrow}%
\UnicodeMathSymbol{"021BB}{\cwopencirclearrow        }{\mathord}{clockwise open circle arrow}%
\UnicodeMathSymbol{"021BC}{\leftharpoonup            }{\mathrel}{left harpoon-up}%
\UnicodeMathSymbol{"021BD}{\leftharpoondown          }{\mathrel}{left harpoon-down}%
\UnicodeMathSymbol{"021BE}{\upharpoonright           }{\mathrel}{/upharpoonright /restriction a: up harpoon-right}%
\UnicodeMathSymbol{"021BF}{\upharpoonleft            }{\mathrel}{up harpoon-left}%
\UnicodeMathSymbol{"021C0}{\rightharpoonup           }{\mathrel}{right harpoon-up}%
\UnicodeMathSymbol{"021C1}{\rightharpoondown         }{\mathrel}{right harpoon-down}%
\UnicodeMathSymbol{"021C2}{\downharpoonright         }{\mathrel}{down harpoon-right}%
\UnicodeMathSymbol{"021C3}{\downharpoonleft          }{\mathrel}{down harpoon-left}%
\UnicodeMathSymbol{"021C4}{\rightleftarrows          }{\mathrel}{right arrow over left arrow}%
\UnicodeMathSymbol{"021C5}{\updownarrows             }{\mathrel}{up arrow, down arrow}%
\UnicodeMathSymbol{"021C6}{\leftrightarrows          }{\mathrel}{left arrow over right arrow}%
\UnicodeMathSymbol{"021C7}{\leftleftarrows           }{\mathrel}{two left arrows}%
\UnicodeMathSymbol{"021C8}{\upuparrows               }{\mathrel}{two up arrows}%
\UnicodeMathSymbol{"021C9}{\rightrightarrows         }{\mathrel}{two right arrows}%
\UnicodeMathSymbol{"021CA}{\downdownarrows           }{\mathrel}{two down arrows}%
\UnicodeMathSymbol{"021CB}{\leftrightharpoons        }{\mathrel}{left harpoon over right}%
\UnicodeMathSymbol{"021CC}{\rightleftharpoons        }{\mathrel}{right harpoon over left}%
\UnicodeMathSymbol{"021CD}{\nLeftarrow               }{\mathrel}{not implied by}%
\UnicodeMathSymbol{"021CE}{\nLeftrightarrow          }{\mathrel}{not left and right double arrows}%
\UnicodeMathSymbol{"021CF}{\nRightarrow              }{\mathrel}{not implies}%
\UnicodeMathSymbol{"021D0}{\Leftarrow                }{\mathrel}{is implied by}%
\UnicodeMathSymbol{"021D1}{\Uparrow                  }{\mathrel}{up double arrow}%
\UnicodeMathSymbol{"021D2}{\Rightarrow               }{\mathrel}{implies}%
\UnicodeMathSymbol{"021D3}{\Downarrow                }{\mathrel}{down double arrow}%
\UnicodeMathSymbol{"021D4}{\Leftrightarrow           }{\mathrel}{left and right double arrow}%
\UnicodeMathSymbol{"021D5}{\Updownarrow              }{\mathrel}{up and down double arrow}%
\UnicodeMathSymbol{"021D6}{\Nwarrow                  }{\mathrel}{nw pointing double arrow}%
\UnicodeMathSymbol{"021D7}{\Nearrow                  }{\mathrel}{ne pointing double arrow}%
\UnicodeMathSymbol{"021D8}{\Searrow                  }{\mathrel}{se pointing double arrow}%
\UnicodeMathSymbol{"021D9}{\Swarrow                  }{\mathrel}{sw pointing double arrow}%
\UnicodeMathSymbol{"021DA}{\Lleftarrow               }{\mathrel}{left triple arrow}%
\UnicodeMathSymbol{"021DB}{\Rrightarrow              }{\mathrel}{right triple arrow}%
\UnicodeMathSymbol{"021DC}{\leftsquigarrow           }{\mathrel}{leftwards squiggle arrow}%
\UnicodeMathSymbol{"021DD}{\rightsquigarrow          }{\mathrel}{rightwards squiggle arrow}%
\UnicodeMathSymbol{"021DE}{\nHuparrow                }{\mathord}{upwards arrow with double stroke}%
\UnicodeMathSymbol{"021DF}{\nHdownarrow              }{\mathord}{downwards arrow with double stroke}%
\UnicodeMathSymbol{"021E0}{\leftdasharrow            }{\mathord}{leftwards dashed arrow}%
\UnicodeMathSymbol{"021E1}{\updasharrow              }{\mathord}{upwards dashed arrow}%
\UnicodeMathSymbol{"021E2}{\rightdasharrow           }{\mathord}{rightwards dashed arrow}%
\UnicodeMathSymbol{"021E3}{\downdasharrow            }{\mathord}{downwards dashed arrow}%
\UnicodeMathSymbol{"021E4}{\barleftarrow             }{\mathrel}{leftwards arrow to bar}%
\UnicodeMathSymbol{"021E5}{\rightarrowbar            }{\mathrel}{rightwards arrow to bar}%
\UnicodeMathSymbol{"021E6}{\leftwhitearrow           }{\mathord}{leftwards white arrow}%
\UnicodeMathSymbol{"021E7}{\upwhitearrow             }{\mathord}{upwards white arrow}%
\UnicodeMathSymbol{"021E8}{\rightwhitearrow          }{\mathord}{rightwards white arrow}%
\UnicodeMathSymbol{"021E9}{\downwhitearrow           }{\mathord}{downwards white arrow}%
\UnicodeMathSymbol{"021EA}{\whitearrowupfrombar      }{\mathord}{upwards white arrow from bar}%
\UnicodeMathSymbol{"021F4}{\circleonrightarrow       }{\mathrel}{right arrow with small circle}%
\UnicodeMathSymbol{"021F5}{\downuparrows             }{\mathrel}{downwards arrow leftwards of upwards arrow}%
\UnicodeMathSymbol{"021F6}{\rightthreearrows         }{\mathrel}{three rightwards arrows}%
\UnicodeMathSymbol{"021F7}{\nvleftarrow              }{\mathrel}{leftwards arrow with vertical stroke}%
\UnicodeMathSymbol{"021F8}{\nvrightarrow             }{\mathrel}{rightwards arrow with vertical stroke}%
\UnicodeMathSymbol{"021F9}{\nvleftrightarrow         }{\mathrel}{left right arrow with vertical stroke}%
\UnicodeMathSymbol{"021FA}{\nVleftarrow              }{\mathrel}{leftwards arrow with double vertical stroke}%
\UnicodeMathSymbol{"021FB}{\nVrightarrow             }{\mathrel}{rightwards arrow with double vertical stroke}%
\UnicodeMathSymbol{"021FC}{\nVleftrightarrow         }{\mathrel}{left right arrow with double vertical stroke}%
\UnicodeMathSymbol{"021FD}{\leftarrowtriangle        }{\mathrel}{leftwards open-headed arrow}%
\UnicodeMathSymbol{"021FE}{\rightarrowtriangle       }{\mathrel}{rightwards open-headed arrow}%
\UnicodeMathSymbol{"021FF}{\leftrightarrowtriangle   }{\mathrel}{left right open-headed arrow}%
\UnicodeMathSymbol{"02200}{\forall                   }{\mathord}{for all}%
\UnicodeMathSymbol{"02201}{\complement               }{\mathord}{complement sign}%
\UnicodeMathSymbol{"02202}{\partial                  }{\mathalpha}{partial differential}%
\UnicodeMathSymbol{"02203}{\exists                   }{\mathord}{at least one exists}%
\UnicodeMathSymbol{"02204}{\nexists                  }{\mathord}{negated exists}%
\UnicodeMathSymbol{"02205}{\varnothing               }{\mathord}{circle, slash}%
\UnicodeMathSymbol{"02206}{\increment                }{\mathord}{laplacian (delta; nabla\string^2)}%
\UnicodeMathSymbol{"02207}{\nabla                    }{\mathalpha}{nabla, del, hamilton operator}%
\UnicodeMathSymbol{"02208}{\in                       }{\mathrel}{set membership, variant}%
\UnicodeMathSymbol{"02209}{\notin                    }{\mathrel}{negated set membership}%
\UnicodeMathSymbol{"0220A}{\smallin                  }{\mathrel}{set membership (small set membership)}%
\UnicodeMathSymbol{"0220B}{\ni                       }{\mathrel}{contains, variant}%
\UnicodeMathSymbol{"0220C}{\nni                      }{\mathrel}{negated contains, variant}%
\UnicodeMathSymbol{"0220D}{\smallni                  }{\mathrel}{/ni /owns r: contains (small contains as member)}%
\UnicodeMathSymbol{"0220E}{\QED                      }{\mathord}{end of proof}%
\UnicodeMathSymbol{"0220F}{\prod                     }{\mathop}{product operator}%
\UnicodeMathSymbol{"02210}{\coprod                   }{\mathop}{coproduct operator}%
\UnicodeMathSymbol{"02211}{\sum                      }{\mathop}{summation operator}%
\UnicodeMathSymbol{"02212}{\minus                    }{\mathbin}{minus sign}%
\UnicodeMathSymbol{"02213}{\mp                       }{\mathbin}{minus-or-plus sign}%
\UnicodeMathSymbol{"02214}{\dotplus                  }{\mathbin}{plus sign, dot above}%
\UnicodeMathSymbol{"02215}{\divslash                 }{\mathbin}{division slash}%
\UnicodeMathSymbol{"02216}{\smallsetminus            }{\mathbin}{small set minus (cf. reverse solidus)}%
\UnicodeMathSymbol{"02217}{\ast                      }{\mathbin}{centered asterisk}%
\UnicodeMathSymbol{"02218}{\vysmwhtcircle            }{\mathbin}{composite function (small circle)}%
\UnicodeMathSymbol{"02219}{\vysmblkcircle            }{\mathbin}{bullet operator}%
\UnicodeMathSymbol{"0221A}{\sqrt                     }{\mathopen}{radical}%
\UnicodeMathSymbol{"0221A}{\surd                     }{\mathord}{radical}%
\UnicodeMathSymbol{"0221B}{\cuberoot                 }{\mathopen}{cube root}%
\UnicodeMathSymbol{"0221C}{\fourthroot               }{\mathopen}{fourth root}%
\UnicodeMathSymbol{"0221D}{\propto                   }{\mathrel}{is proportional to}%
\UnicodeMathSymbol{"0221E}{\infty                    }{\mathord}{infinity}%
\UnicodeMathSymbol{"0221F}{\rightangle               }{\mathord}{right (90 degree) angle}%
\UnicodeMathSymbol{"02220}{\angle                    }{\mathord}{angle}%
\UnicodeMathSymbol{"02221}{\measuredangle            }{\mathord}{angle-measured}%
\UnicodeMathSymbol{"02222}{\sphericalangle           }{\mathord}{angle-spherical}%
\UnicodeMathSymbol{"02223}{\mid                      }{\mathrel}{/mid r:}%
\UnicodeMathSymbol{"02224}{\nmid                     }{\mathrel}{negated mid}%
\UnicodeMathSymbol{"02225}{\parallel                 }{\mathrel}{parallel}%
\UnicodeMathSymbol{"02226}{\nparallel                }{\mathrel}{not parallel}%
\UnicodeMathSymbol{"02227}{\wedge                    }{\mathbin}{/wedge /land b: logical and}%
\UnicodeMathSymbol{"02228}{\vee                      }{\mathbin}{/vee /lor b: logical or}%
\UnicodeMathSymbol{"02229}{\cap                      }{\mathbin}{intersection}%
\UnicodeMathSymbol{"0222A}{\cup                      }{\mathbin}{union or logical sum}%
\UnicodeMathSymbol{"0222B}{\int                      }{\mathop}{integral operator}%
\UnicodeMathSymbol{"0222C}{\iint                     }{\mathop}{double integral operator}%
\UnicodeMathSymbol{"0222D}{\iiint                    }{\mathop}{triple integral operator}%
\UnicodeMathSymbol{"0222E}{\oint                     }{\mathop}{contour integral operator}%
\UnicodeMathSymbol{"0222F}{\oiint                    }{\mathop}{double contour integral operator}%
\UnicodeMathSymbol{"02230}{\oiiint                   }{\mathop}{triple contour integral operator}%
\UnicodeMathSymbol{"02231}{\intclockwise             }{\mathop}{clockwise integral}%
\UnicodeMathSymbol{"02232}{\varointclockwise         }{\mathop}{contour integral, clockwise}%
\UnicodeMathSymbol{"02233}{\ointctrclockwise         }{\mathop}{contour integral, anticlockwise}%
\UnicodeMathSymbol{"02234}{\therefore                }{\mathord}{therefore}%
\UnicodeMathSymbol{"02235}{\because                  }{\mathord}{because}%
\UnicodeMathSymbol{"02236}{\mathratio                }{\mathrel}{ratio}%
\UnicodeMathSymbol{"02237}{\Colon                    }{\mathrel}{two colons}%
\UnicodeMathSymbol{"02238}{\dotminus                 }{\mathbin}{minus sign, dot above}%
\UnicodeMathSymbol{"02239}{\dashcolon                }{\mathrel}{excess (-:)}%
\UnicodeMathSymbol{"0223A}{\dotsminusdots            }{\mathrel}{minus with four dots, geometric properties}%
\UnicodeMathSymbol{"0223B}{\kernelcontraction        }{\mathrel}{homothetic}%
\UnicodeMathSymbol{"0223C}{\sim                      }{\mathrel}{similar}%
\UnicodeMathSymbol{"0223D}{\backsim                  }{\mathrel}{reverse similar}%
\UnicodeMathSymbol{"0223E}{\invlazys                 }{\mathbin}{most positive [inverted lazy s]}%
\UnicodeMathSymbol{"0223F}{\sinewave                 }{\mathord}{sine wave}%
\UnicodeMathSymbol{"02240}{\wr                       }{\mathbin}{wreath product}%
\UnicodeMathSymbol{"02241}{\nsim                     }{\mathrel}{not similar}%
\UnicodeMathSymbol{"02242}{\eqsim                    }{\mathrel}{equals, similar}%
\UnicodeMathSymbol{"02243}{\simeq                    }{\mathrel}{similar, equals}%
\UnicodeMathSymbol{"02244}{\nsime                    }{\mathrel}{not similar, equals}%
\UnicodeMathSymbol{"02243}{\sime                     }{\mathrel}{similar, equals (alias)}%
\UnicodeMathSymbol{"02244}{\nsimeq                   }{\mathrel}{not similar, equals (alias)}%
\UnicodeMathSymbol{"02245}{\cong                     }{\mathrel}{congruent with}%
\UnicodeMathSymbol{"02246}{\simneqq                  }{\mathrel}{similar, not equals [vert only for 9573 entity]}%
\UnicodeMathSymbol{"02247}{\ncong                    }{\mathrel}{not congruent with}%
\UnicodeMathSymbol{"02248}{\approx                   }{\mathrel}{approximate}%
\UnicodeMathSymbol{"02249}{\napprox                  }{\mathrel}{not approximate}%
\UnicodeMathSymbol{"0224A}{\approxeq                 }{\mathrel}{approximate, equals}%
\UnicodeMathSymbol{"0224B}{\approxident              }{\mathrel}{approximately identical to}%
\UnicodeMathSymbol{"0224C}{\backcong                 }{\mathrel}{all equal to}%
\UnicodeMathSymbol{"0224D}{\asymp                    }{\mathrel}{asymptotically equal to}%
\UnicodeMathSymbol{"0224E}{\Bumpeq                   }{\mathrel}{bumpy equals}%
\UnicodeMathSymbol{"0224F}{\bumpeq                   }{\mathrel}{bumpy equals, equals}%
\UnicodeMathSymbol{"02250}{\doteq                    }{\mathrel}{equals, single dot above}%
\UnicodeMathSymbol{"02251}{\Doteq                    }{\mathrel}{/doteqdot /doteq r: equals, even dots}%
\UnicodeMathSymbol{"02252}{\fallingdotseq            }{\mathrel}{equals, falling dots}%
\UnicodeMathSymbol{"02253}{\risingdotseq             }{\mathrel}{equals, rising dots}%
\UnicodeMathSymbol{"02254}{\coloneq                  }{\mathrel}{colon, equals}%
\UnicodeMathSymbol{"02255}{\eqcolon                  }{\mathrel}{equals, colon}%
\UnicodeMathSymbol{"02256}{\eqcirc                   }{\mathrel}{circle on equals sign}%
\UnicodeMathSymbol{"02257}{\circeq                   }{\mathrel}{circle, equals}%
\UnicodeMathSymbol{"02258}{\arceq                    }{\mathrel}{arc, equals; corresponds to}%
\UnicodeMathSymbol{"02259}{\wedgeq                   }{\mathrel}{corresponds to (wedge, equals)}%
\UnicodeMathSymbol{"0225A}{\veeeq                    }{\mathrel}{logical or, equals}%
\UnicodeMathSymbol{"0225B}{\stareq                   }{\mathrel}{star equals}%
\UnicodeMathSymbol{"0225C}{\triangleq                }{\mathrel}{triangle, equals}%
\UnicodeMathSymbol{"0225D}{\eqdef                    }{\mathrel}{equals by definition}%
\UnicodeMathSymbol{"0225E}{\measeq                   }{\mathrel}{measured by (m over equals)}%
\UnicodeMathSymbol{"0225F}{\questeq                  }{\mathrel}{equal with questionmark}%
\UnicodeMathSymbol{"02260}{\ne                       }{\mathrel}{/ne /neq r: not equal}%
\UnicodeMathSymbol{"02261}{\equiv                    }{\mathrel}{identical with}%
\UnicodeMathSymbol{"02262}{\nequiv                   }{\mathrel}{not identical with}%
\UnicodeMathSymbol{"02263}{\Equiv                    }{\mathrel}{strict equivalence (4 lines)}%
\UnicodeMathSymbol{"02264}{\leq                      }{\mathrel}{/leq /le r: less-than-or-equal}%
\UnicodeMathSymbol{"02265}{\geq                      }{\mathrel}{/geq /ge r: greater-than-or-equal}%
\UnicodeMathSymbol{"02266}{\leqq                     }{\mathrel}{less, double equals}%
\UnicodeMathSymbol{"02267}{\geqq                     }{\mathrel}{greater, double equals}%
\UnicodeMathSymbol{"02268}{\lneqq                    }{\mathrel}{less, not double equals}%
\UnicodeMathSymbol{"02269}{\gneqq                    }{\mathrel}{greater, not double equals}%
\UnicodeMathSymbol{"0226A}{\ll                       }{\mathrel}{much less than, type 2}%
\UnicodeMathSymbol{"0226B}{\gg                       }{\mathrel}{much greater than, type 2}%
\UnicodeMathSymbol{"0226C}{\between                  }{\mathrel}{between}%
\UnicodeMathSymbol{"0226D}{\nasymp                   }{\mathrel}{not asymptotically equal to}%
\UnicodeMathSymbol{"0226E}{\nless                    }{\mathrel}{not less-than}%
\UnicodeMathSymbol{"0226F}{\ngtr                     }{\mathrel}{not greater-than}%
\UnicodeMathSymbol{"02270}{\nleq                     }{\mathrel}{not less-than-or-equal}%
\UnicodeMathSymbol{"02271}{\ngeq                     }{\mathrel}{not greater-than-or-equal}%
\UnicodeMathSymbol{"02272}{\lesssim                  }{\mathrel}{less, similar}%
\UnicodeMathSymbol{"02273}{\gtrsim                   }{\mathrel}{greater, similar}%
\UnicodeMathSymbol{"02274}{\nlesssim                 }{\mathrel}{not less, similar}%
\UnicodeMathSymbol{"02275}{\ngtrsim                  }{\mathrel}{not greater, similar}%
\UnicodeMathSymbol{"02276}{\lessgtr                  }{\mathrel}{less, greater}%
\UnicodeMathSymbol{"02277}{\gtrless                  }{\mathrel}{greater, less}%
\UnicodeMathSymbol{"02278}{\nlessgtr                 }{\mathrel}{not less, greater}%
\UnicodeMathSymbol{"02279}{\ngtrless                 }{\mathrel}{not greater, less}%
\UnicodeMathSymbol{"0227A}{\prec                     }{\mathrel}{precedes}%
\UnicodeMathSymbol{"0227B}{\succ                     }{\mathrel}{succeeds}%
\UnicodeMathSymbol{"0227C}{\preccurlyeq              }{\mathrel}{precedes, curly equals}%
\UnicodeMathSymbol{"0227D}{\succcurlyeq              }{\mathrel}{succeeds, curly equals}%
\UnicodeMathSymbol{"0227E}{\precsim                  }{\mathrel}{precedes, similar}%
\UnicodeMathSymbol{"0227F}{\succsim                  }{\mathrel}{succeeds, similar}%
\UnicodeMathSymbol{"02280}{\nprec                    }{\mathrel}{not precedes}%
\UnicodeMathSymbol{"02281}{\nsucc                    }{\mathrel}{not succeeds}%
\UnicodeMathSymbol{"02282}{\subset                   }{\mathrel}{subset or is implied by}%
\UnicodeMathSymbol{"02283}{\supset                   }{\mathrel}{superset or implies}%
\UnicodeMathSymbol{"02284}{\nsubset                  }{\mathrel}{not subset, variant [slash negation]}%
\UnicodeMathSymbol{"02285}{\nsupset                  }{\mathrel}{not superset, variant [slash negation]}%
\UnicodeMathSymbol{"02286}{\subseteq                 }{\mathrel}{subset, equals}%
\UnicodeMathSymbol{"02287}{\supseteq                 }{\mathrel}{superset, equals}%
\UnicodeMathSymbol{"02288}{\nsubseteq                }{\mathrel}{not subset, equals}%
\UnicodeMathSymbol{"02289}{\nsupseteq                }{\mathrel}{not superset, equals}%
\UnicodeMathSymbol{"0228A}{\subsetneq                }{\mathrel}{subset, not equals}%
\UnicodeMathSymbol{"0228B}{\supsetneq                }{\mathrel}{superset, not equals}%
\UnicodeMathSymbol{"0228C}{\cupleftarrow             }{\mathbin}{multiset}%
\UnicodeMathSymbol{"0228D}{\cupdot                   }{\mathbin}{union, with dot}%
\UnicodeMathSymbol{"0228E}{\uplus                    }{\mathbin}{plus sign in union}%
\UnicodeMathSymbol{"0228F}{\sqsubset                 }{\mathrel}{square subset}%
\UnicodeMathSymbol{"02290}{\sqsupset                 }{\mathrel}{square superset}%
\UnicodeMathSymbol{"02291}{\sqsubseteq               }{\mathrel}{square subset, equals}%
\UnicodeMathSymbol{"02292}{\sqsupseteq               }{\mathrel}{square superset, equals}%
\UnicodeMathSymbol{"02293}{\sqcap                    }{\mathbin}{square intersection}%
\UnicodeMathSymbol{"02294}{\sqcup                    }{\mathbin}{square union}%
\UnicodeMathSymbol{"02295}{\oplus                    }{\mathbin}{plus sign in circle}%
\UnicodeMathSymbol{"02296}{\ominus                   }{\mathbin}{minus sign in circle}%
\UnicodeMathSymbol{"02297}{\otimes                   }{\mathbin}{multiply sign in circle}%
\UnicodeMathSymbol{"02298}{\oslash                   }{\mathbin}{solidus in circle}%
\UnicodeMathSymbol{"02299}{\odot                     }{\mathbin}{middle dot in circle}%
\UnicodeMathSymbol{"0229A}{\circledcirc              }{\mathbin}{small circle in circle}%
\UnicodeMathSymbol{"0229B}{\circledast               }{\mathbin}{asterisk in circle}%
\UnicodeMathSymbol{"0229C}{\circledequal             }{\mathbin}{equal in circle}%
\UnicodeMathSymbol{"0229D}{\circleddash              }{\mathbin}{hyphen in circle}%
\UnicodeMathSymbol{"0229E}{\boxplus                  }{\mathbin}{plus sign in box}%
\UnicodeMathSymbol{"0229F}{\boxminus                 }{\mathbin}{minus sign in box}%
\UnicodeMathSymbol{"022A0}{\boxtimes                 }{\mathbin}{multiply sign in box}%
\UnicodeMathSymbol{"022A1}{\boxdot                   }{\mathbin}{/dotsquare /boxdot b: small dot in box}%
\UnicodeMathSymbol{"022A2}{\vdash                    }{\mathrel}{vertical, dash}%
\UnicodeMathSymbol{"022A3}{\dashv                    }{\mathrel}{dash, vertical}%
\UnicodeMathSymbol{"022A4}{\top                      }{\mathord}{top}%
\UnicodeMathSymbol{"022A5}{\bot                      }{\mathord}{bottom}%
\UnicodeMathSymbol{"022A6}{\assert                   }{\mathrel}{assertion (vertical, short dash)}%
\UnicodeMathSymbol{"022A7}{\models                   }{\mathrel}{models (vertical, short double dash)}%
\UnicodeMathSymbol{"022A8}{\vDash                    }{\mathrel}{vertical, double dash}%
\UnicodeMathSymbol{"022A9}{\Vdash                    }{\mathrel}{double vertical, dash}%
\UnicodeMathSymbol{"022AA}{\Vvdash                   }{\mathrel}{triple vertical, dash}%
\UnicodeMathSymbol{"022AB}{\VDash                    }{\mathrel}{double vert, double dash}%
\UnicodeMathSymbol{"022AC}{\nvdash                   }{\mathrel}{not vertical, dash}%
\UnicodeMathSymbol{"022AD}{\nvDash                   }{\mathrel}{not vertical, double dash}%
\UnicodeMathSymbol{"022AE}{\nVdash                   }{\mathrel}{not double vertical, dash}%
\UnicodeMathSymbol{"022AF}{\nVDash                   }{\mathrel}{not double vert, double dash}%
\UnicodeMathSymbol{"022B0}{\prurel                   }{\mathrel}{element precedes under relation}%
\UnicodeMathSymbol{"022B1}{\scurel                   }{\mathrel}{succeeds under relation}%
\UnicodeMathSymbol{"022B2}{\vartriangleleft          }{\mathrel}{left triangle, open, variant}%
\UnicodeMathSymbol{"022B3}{\vartriangleright         }{\mathrel}{right triangle, open, variant}%
\UnicodeMathSymbol{"022B4}{\trianglelefteq           }{\mathrel}{left triangle, equals}%
\UnicodeMathSymbol{"022B5}{\trianglerighteq          }{\mathrel}{right triangle, equals}%
\UnicodeMathSymbol{"022B6}{\origof                   }{\mathrel}{original of}%
\UnicodeMathSymbol{"022B7}{\imageof                  }{\mathrel}{image of}%
\UnicodeMathSymbol{"022B8}{\multimap                 }{\mathrel}{/multimap a:}%
\UnicodeMathSymbol{"022B9}{\hermitmatrix             }{\mathord}{hermitian conjugate matrix}%
\UnicodeMathSymbol{"022BA}{\intercal                 }{\mathbin}{intercal}%
\UnicodeMathSymbol{"022BB}{\veebar                   }{\mathbin}{logical or, bar below (large vee); exclusive disjunction}%
\UnicodeMathSymbol{"022BC}{\barwedge                 }{\mathbin}{bar, wedge (large wedge)}%
\UnicodeMathSymbol{"022BD}{\barvee                   }{\mathbin}{bar, vee (large vee)}%
\UnicodeMathSymbol{"022BE}{\measuredrightangle       }{\mathord}{right angle-measured [with arc]}%
\UnicodeMathSymbol{"022BF}{\varlrtriangle            }{\mathord}{right triangle}%
\UnicodeMathSymbol{"022C0}{\bigwedge                 }{\mathop}{logical and operator}%
\UnicodeMathSymbol{"022C1}{\bigvee                   }{\mathop}{logical or operator}%
\UnicodeMathSymbol{"022C2}{\bigcap                   }{\mathop}{intersection operator}%
\UnicodeMathSymbol{"022C3}{\bigcup                   }{\mathop}{union operator}%
\UnicodeMathSymbol{"022C4}{\smwhtdiamond             }{\mathbin}{white diamond}%
\UnicodeMathSymbol{"022C5}{\cdot                     }{\mathbin}{small middle dot}%
\UnicodeMathSymbol{"022C6}{\star                     }{\mathbin}{small star, filled, low}%
\UnicodeMathSymbol{"022C7}{\divideontimes            }{\mathbin}{division on times}%
\UnicodeMathSymbol{"022C8}{\bowtie                   }{\mathrel}{bowtie}%
\UnicodeMathSymbol{"022C9}{\ltimes                   }{\mathbin}{times sign, left closed}%
\UnicodeMathSymbol{"022CA}{\rtimes                   }{\mathbin}{times sign, right closed}%
\UnicodeMathSymbol{"022CB}{\leftthreetimes           }{\mathbin}{left semidirect product}%
\UnicodeMathSymbol{"022CC}{\rightthreetimes          }{\mathbin}{right semidirect product}%
\UnicodeMathSymbol{"022CD}{\backsimeq                }{\mathrel}{reverse similar, equals}%
\UnicodeMathSymbol{"022CE}{\curlyvee                 }{\mathbin}{curly logical or}%
\UnicodeMathSymbol{"022CF}{\curlywedge               }{\mathbin}{curly logical and}%
\UnicodeMathSymbol{"022D0}{\Subset                   }{\mathrel}{double subset}%
\UnicodeMathSymbol{"022D1}{\Supset                   }{\mathrel}{double superset}%
\UnicodeMathSymbol{"022D2}{\Cap                      }{\mathbin}{/cap /doublecap b: double intersection}%
\UnicodeMathSymbol{"022D3}{\Cup                      }{\mathbin}{/cup /doublecup b: double union}%
\UnicodeMathSymbol{"022D4}{\pitchfork                }{\mathrel}{pitchfork}%
\UnicodeMathSymbol{"022D5}{\equalparallel            }{\mathrel}{parallel, equal; equal or parallel}%
\UnicodeMathSymbol{"022D6}{\lessdot                  }{\mathrel}{less than, with dot}%
\UnicodeMathSymbol{"022D7}{\gtrdot                   }{\mathrel}{greater than, with dot}%
\UnicodeMathSymbol{"022D8}{\lll                      }{\mathrel}{/ll /lll /llless r: triple less-than}%
\UnicodeMathSymbol{"022D9}{\ggg                      }{\mathrel}{/ggg /gg /gggtr r: triple greater-than}%
\UnicodeMathSymbol{"022DA}{\lesseqgtr                }{\mathrel}{less, equals, greater}%
\UnicodeMathSymbol{"022DB}{\gtreqless                }{\mathrel}{greater, equals, less}%
\UnicodeMathSymbol{"022DC}{\eqless                   }{\mathrel}{equal-or-less}%
\UnicodeMathSymbol{"022DD}{\eqgtr                    }{\mathrel}{equal-or-greater}%
\UnicodeMathSymbol{"022DE}{\curlyeqprec              }{\mathrel}{curly equals, precedes}%
\UnicodeMathSymbol{"022DF}{\curlyeqsucc              }{\mathrel}{curly equals, succeeds}%
\UnicodeMathSymbol{"022E0}{\npreccurlyeq             }{\mathrel}{not precedes, curly equals}%
\UnicodeMathSymbol{"022E1}{\nsucccurlyeq             }{\mathrel}{not succeeds, curly equals}%
\UnicodeMathSymbol{"022E2}{\nsqsubseteq              }{\mathrel}{not, square subset, equals}%
\UnicodeMathSymbol{"022E3}{\nsqsupseteq              }{\mathrel}{not, square superset, equals}%
\UnicodeMathSymbol{"022E4}{\sqsubsetneq              }{\mathrel}{square subset, not equals}%
\UnicodeMathSymbol{"022E5}{\sqsupsetneq              }{\mathrel}{square superset, not equals}%
\UnicodeMathSymbol{"022E6}{\lnsim                    }{\mathrel}{less, not similar}%
\UnicodeMathSymbol{"022E7}{\gnsim                    }{\mathrel}{greater, not similar}%
\UnicodeMathSymbol{"022E8}{\precnsim                 }{\mathrel}{precedes, not similar}%
\UnicodeMathSymbol{"022E9}{\succnsim                 }{\mathrel}{succeeds, not similar}%
\UnicodeMathSymbol{"022EA}{\nvartriangleleft         }{\mathrel}{not left triangle}%
\UnicodeMathSymbol{"022EB}{\nvartriangleright        }{\mathrel}{not right triangle}%
\UnicodeMathSymbol{"022EC}{\ntrianglelefteq          }{\mathrel}{not left triangle, equals}%
\UnicodeMathSymbol{"022ED}{\ntrianglerighteq         }{\mathrel}{not right triangle, equals}%
\UnicodeMathSymbol{"022EE}{\vdots                    }{\mathrel}{vertical ellipsis}%
\UnicodeMathSymbol{"022EF}{\unicodecdots             }{\mathord}{three dots, centered}%
\UnicodeMathSymbol{"022F0}{\adots                    }{\mathrel}{three dots, ascending}%
\UnicodeMathSymbol{"022F1}{\ddots                    }{\mathrel}{three dots, descending}%
\UnicodeMathSymbol{"022F2}{\disin                    }{\mathrel}{element of with long horizontal stroke}%
\UnicodeMathSymbol{"022F3}{\varisins                 }{\mathrel}{element of with vertical bar at end of horizontal stroke}%
\UnicodeMathSymbol{"022F4}{\isins                    }{\mathrel}{small element of with vertical bar at end of horizontal stroke}%
\UnicodeMathSymbol{"022F5}{\isindot                  }{\mathrel}{element of with dot above}%
\UnicodeMathSymbol{"022F6}{\varisinobar              }{\mathrel}{element of with overbar}%
\UnicodeMathSymbol{"022F7}{\isinobar                 }{\mathrel}{small element of with overbar}%
\UnicodeMathSymbol{"022F8}{\isinvb                   }{\mathrel}{element of with underbar}%
\UnicodeMathSymbol{"022F9}{\isinE                    }{\mathrel}{element of with two horizontal strokes}%
\UnicodeMathSymbol{"022FA}{\nisd                     }{\mathrel}{contains with long horizontal stroke}%
\UnicodeMathSymbol{"022FB}{\varnis                   }{\mathrel}{contains with vertical bar at end of horizontal stroke}%
\UnicodeMathSymbol{"022FC}{\nis                      }{\mathrel}{small contains with vertical bar at end of horizontal stroke}%
\UnicodeMathSymbol{"022FD}{\varniobar                }{\mathrel}{contains with overbar}%
\UnicodeMathSymbol{"022FE}{\niobar                   }{\mathrel}{small contains with overbar}%
\UnicodeMathSymbol{"022FF}{\bagmember                }{\mathrel}{z notation bag membership}%
\UnicodeMathSymbol{"02300}{\diameter                 }{\mathord}{diameter sign}%
\UnicodeMathSymbol{"02302}{\house                    }{\mathord}{house}%
\UnicodeMathSymbol{"02305}{\varbarwedge              }{\mathbin}{/barwedge b: logical and, bar above [projective (bar over small wedge)]}%
\UnicodeMathSymbol{"02306}{\vardoublebarwedge        }{\mathbin}{/doublebarwedge b: logical and, double bar above [perspective (double bar over small wedge)]}%
\UnicodeMathSymbol{"02308}{\lceil                    }{\mathopen}{left ceiling}%
\UnicodeMathSymbol{"02309}{\rceil                    }{\mathclose}{right ceiling}%
\UnicodeMathSymbol{"0230A}{\lfloor                   }{\mathopen}{left floor}%
\UnicodeMathSymbol{"0230B}{\rfloor                   }{\mathclose}{right floor}%
\UnicodeMathSymbol{"02310}{\invnot                   }{\mathord}{reverse not}%
\UnicodeMathSymbol{"02311}{\sqlozenge                }{\mathord}{square lozenge}%
\UnicodeMathSymbol{"02312}{\profline                 }{\mathord}{profile of a line}%
\UnicodeMathSymbol{"02313}{\profsurf                 }{\mathord}{profile of a surface}%
\UnicodeMathSymbol{"02317}{\viewdata                 }{\mathord}{viewdata square}%
\UnicodeMathSymbol{"02319}{\turnednot                }{\mathord}{turned not sign}%
\UnicodeMathSymbol{"0231C}{\ulcorner                 }{\mathopen}{upper left corner}%
\UnicodeMathSymbol{"0231D}{\urcorner                 }{\mathclose}{upper right corner}%
\UnicodeMathSymbol{"0231E}{\llcorner                 }{\mathopen}{lower left corner}%
\UnicodeMathSymbol{"0231F}{\lrcorner                 }{\mathclose}{lower right corner}%
\UnicodeMathSymbol{"02320}{\inttop                   }{\mathord}{top half integral}%
\UnicodeMathSymbol{"02321}{\intbottom                }{\mathord}{bottom half integral}%
\UnicodeMathSymbol{"02322}{\frown                    }{\mathrel}{down curve}%
\UnicodeMathSymbol{"02323}{\smile                    }{\mathrel}{up curve}%
\UnicodeMathSymbol{"0232C}{\varhexagonlrbonds        }{\mathord}{six carbon ring, corner down, double bonds lower right etc}%
\UnicodeMathSymbol{"02332}{\conictaper               }{\mathord}{conical taper }%
\UnicodeMathSymbol{"02336}{\topbot                   }{\mathord}{top and bottom}%
\UnicodeMathSymbol{"0233D}{\obar                     }{\mathbin}{circle with vertical bar}%
\UnicodeMathSymbol{"0233F}{\APLnotslash              }{\mathrel}{solidus, bar through (apl functional symbol slash bar)}%
\UnicodeMathSymbol{"02340}{\APLnotbackslash          }{\mathord}{apl functional symbol backslash bar}%
\UnicodeMathSymbol{"02353}{\APLboxupcaret            }{\mathord}{boxed up caret}%
\UnicodeMathSymbol{"02370}{\APLboxquestion           }{\mathord}{boxed question mark}%
\UnicodeMathSymbol{"0237C}{\rangledownzigzagarrow    }{\mathord}{right angle with downwards zigzag arrow}%
\UnicodeMathSymbol{"02394}{\hexagon                  }{\mathord}{horizontal benzene ring [hexagon flat open]}%
\UnicodeMathSymbol{"0239B}{\lparenuend               }{\mathord}{left parenthesis upper hook}%
\UnicodeMathSymbol{"0239C}{\lparenextender           }{\mathord}{left parenthesis extension}%
\UnicodeMathSymbol{"0239D}{\lparenlend               }{\mathord}{left parenthesis lower hook}%
\UnicodeMathSymbol{"0239E}{\rparenuend               }{\mathord}{right parenthesis upper hook}%
\UnicodeMathSymbol{"0239F}{\rparenextender           }{\mathord}{right parenthesis extension}%
\UnicodeMathSymbol{"023A0}{\rparenlend               }{\mathord}{right parenthesis lower hook}%
\UnicodeMathSymbol{"023A1}{\lbrackuend               }{\mathord}{left square bracket upper corner}%
\UnicodeMathSymbol{"023A2}{\lbrackextender           }{\mathord}{left square bracket extension}%
\UnicodeMathSymbol{"023A3}{\lbracklend               }{\mathord}{left square bracket lower corner}%
\UnicodeMathSymbol{"023A4}{\rbrackuend               }{\mathord}{right square bracket upper corner}%
\UnicodeMathSymbol{"023A5}{\rbrackextender           }{\mathord}{right square bracket extension}%
\UnicodeMathSymbol{"023A6}{\rbracklend               }{\mathord}{right square bracket lower corner}%
\UnicodeMathSymbol{"023A7}{\lbraceuend               }{\mathord}{left curly bracket upper hook}%
\UnicodeMathSymbol{"023A8}{\lbracemid                }{\mathord}{left curly bracket middle piece}%
\UnicodeMathSymbol{"023A9}{\lbracelend               }{\mathord}{left curly bracket lower hook}%
\UnicodeMathSymbol{"023AA}{\vbraceextender           }{\mathord}{curly bracket extension}%
\UnicodeMathSymbol{"023AB}{\rbraceuend               }{\mathord}{right curly bracket upper hook}%
\UnicodeMathSymbol{"023AC}{\rbracemid                }{\mathord}{right curly bracket middle piece}%
\UnicodeMathSymbol{"023AD}{\rbracelend               }{\mathord}{right curly bracket lower hook}%
\UnicodeMathSymbol{"023AE}{\intextender              }{\mathord}{integral extension}%
\UnicodeMathSymbol{"023AF}{\harrowextender           }{\mathord}{horizontal line extension (used to extend arrows)}%
\UnicodeMathSymbol{"023B0}{\lmoustache               }{\mathopen}{upper left or lower right curly bracket section}%
\UnicodeMathSymbol{"023B1}{\rmoustache               }{\mathclose}{upper right or lower left curly bracket section}%
\UnicodeMathSymbol{"023B2}{\sumtop                   }{\mathord}{summation top}%
\UnicodeMathSymbol{"023B3}{\sumbottom                }{\mathord}{summation bottom}%
\UnicodeMathSymbol{"023B4}{\overbracket              }{\mathover}{top square bracket}%
\UnicodeMathSymbol{"023B5}{\underbracket             }{\mathunder}{bottom square bracket}%
\UnicodeMathSymbol{"023B6}{\bbrktbrk                 }{\mathord}{bottom square bracket over top square bracket}%
\UnicodeMathSymbol{"023B7}{\sqrtbottom               }{\mathord}{radical symbol bottom}%
\UnicodeMathSymbol{"023B8}{\lvboxline                }{\mathord}{left vertical box line}%
\UnicodeMathSymbol{"023B9}{\rvboxline                }{\mathord}{right vertical box line}%
\UnicodeMathSymbol{"023CE}{\varcarriagereturn        }{\mathord}{return symbol}%
\UnicodeMathSymbol{"023DC}{\overparen                }{\mathover}{top parenthesis (mathematical use)}%
\UnicodeMathSymbol{"023DD}{\underparen               }{\mathunder}{bottom parenthesis (mathematical use)}%
\UnicodeMathSymbol{"023DE}{\overbrace                }{\mathover}{top curly bracket (mathematical use)}%
\UnicodeMathSymbol{"023DF}{\underbrace               }{\mathunder}{bottom curly bracket (mathematical use)}%
\UnicodeMathSymbol{"023E0}{\obrbrak                  }{\mathord}{top tortoise shell bracket (mathematical use)}%
\UnicodeMathSymbol{"023E1}{\ubrbrak                  }{\mathord}{bottom tortoise shell bracket (mathematical use)}%
\UnicodeMathSymbol{"023E2}{\trapezium                }{\mathord}{white trapezium}%
\UnicodeMathSymbol{"023E3}{\benzenr                  }{\mathord}{benzene ring with circle}%
\UnicodeMathSymbol{"023E4}{\strns                    }{\mathord}{straightness}%
\UnicodeMathSymbol{"023E5}{\fltns                    }{\mathord}{flatness}%
\UnicodeMathSymbol{"023E6}{\accurrent                }{\mathord}{ac current}%
\UnicodeMathSymbol{"023E7}{\elinters                 }{\mathord}{electrical intersection}%
\UnicodeMathSymbol{"02422}{\blanksymbol              }{\mathord}{blank symbol}%
\UnicodeMathSymbol{"02423}{\mathvisiblespace         }{\mathord}{open box}%
\UnicodeMathSymbol{"02506}{\bdtriplevdash            }{\mathord}{doubly broken vert}%
\UnicodeMathSymbol{"02580}{\blockuphalf              }{\mathord}{upper half block}%
\UnicodeMathSymbol{"02584}{\blocklowhalf             }{\mathord}{lower half block}%
\UnicodeMathSymbol{"02588}{\blockfull                }{\mathord}{full block}%
\UnicodeMathSymbol{"0258C}{\blocklefthalf            }{\mathord}{left half block}%
\UnicodeMathSymbol{"02590}{\blockrighthalf           }{\mathord}{right half block}%
\UnicodeMathSymbol{"02591}{\blockqtrshaded           }{\mathord}{25\% shaded block}%
\UnicodeMathSymbol{"02592}{\blockhalfshaded          }{\mathord}{50\% shaded block}%
\UnicodeMathSymbol{"02593}{\blockthreeqtrshaded      }{\mathord}{75\% shaded block}%
\UnicodeMathSymbol{"025A0}{\mdlgblksquare            }{\mathord}{square, filled}%
\UnicodeMathSymbol{"025A1}{\mdlgwhtsquare            }{\mathord}{square, open}%
\UnicodeMathSymbol{"025A2}{\squoval                  }{\mathord}{white square with rounded corners}%
\UnicodeMathSymbol{"025A3}{\blackinwhitesquare       }{\mathord}{white square containing black small square}%
\UnicodeMathSymbol{"025A4}{\squarehfill              }{\mathord}{square, horizontal rule filled}%
\UnicodeMathSymbol{"025A5}{\squarevfill              }{\mathord}{square, vertical rule filled}%
\UnicodeMathSymbol{"025A6}{\squarehvfill             }{\mathord}{square with orthogonal crosshatch fill}%
\UnicodeMathSymbol{"025A7}{\squarenwsefill           }{\mathord}{square, nw-to-se rule filled}%
\UnicodeMathSymbol{"025A8}{\squareneswfill           }{\mathord}{square, ne-to-sw rule filled}%
\UnicodeMathSymbol{"025A9}{\squarecrossfill          }{\mathord}{square with diagonal crosshatch fill}%
\UnicodeMathSymbol{"025AA}{\smblksquare              }{\mathord}{/blacksquare - sq bullet, filled}%
\UnicodeMathSymbol{"025AB}{\smwhtsquare              }{\mathord}{white small square}%
\UnicodeMathSymbol{"025AC}{\hrectangleblack          }{\mathord}{black rectangle}%
\UnicodeMathSymbol{"025AD}{\hrectangle               }{\mathord}{horizontal rectangle, open}%
\UnicodeMathSymbol{"025AE}{\vrectangleblack          }{\mathord}{black vertical rectangle}%
\UnicodeMathSymbol{"025AF}{\vrectangle               }{\mathord}{rectangle, white (vertical)}%
\UnicodeMathSymbol{"025B0}{\parallelogramblack       }{\mathord}{black parallelogram}%
\UnicodeMathSymbol{"025B1}{\parallelogram            }{\mathord}{parallelogram, open}%
\UnicodeMathSymbol{"025B2}{\bigblacktriangleup       }{\mathord}{   0x25b2 6 6d      black up-pointing triangle}%
\UnicodeMathSymbol{"025B3}{\bigtriangleup            }{\mathbin}{big up triangle, open}%
\UnicodeMathSymbol{"025B4}{\blacktriangle            }{\mathord}{up triangle, filled}%
\UnicodeMathSymbol{"025B5}{\vartriangle              }{\mathrel}{/triangle - up triangle, open}%
\UnicodeMathSymbol{"025B6}{\blacktriangleright       }{\mathord}{(large) right triangle, filled}%
\UnicodeMathSymbol{"025B7}{\triangleright            }{\mathbin}{(large) right triangle, open; z notation range restriction}%
\UnicodeMathSymbol{"025B8}{\smallblacktriangleright  }{\mathord}{right triangle, filled}%
\UnicodeMathSymbol{"025B9}{\smalltriangleright       }{\mathord}{right triangle, open}%
\UnicodeMathSymbol{"025BA}{\blackpointerright        }{\mathord}{black right-pointing pointer}%
\UnicodeMathSymbol{"025BB}{\whitepointerright        }{\mathord}{white right-pointing pointer}%
\UnicodeMathSymbol{"025BC}{\bigblacktriangledown     }{\mathord}{big down triangle, filled}%
\UnicodeMathSymbol{"025BD}{\bigtriangledown          }{\mathord}{big down triangle, open}%
\UnicodeMathSymbol{"025BE}{\blacktriangledown        }{\mathord}{down triangle, filled}%
\UnicodeMathSymbol{"025BF}{\triangledown             }{\mathord}{down triangle, open}%
\UnicodeMathSymbol{"025C0}{\blacktriangleleft        }{\mathord}{(large) left triangle, filled}%
\UnicodeMathSymbol{"025C1}{\triangleleft             }{\mathbin}{(large) left triangle, open; z notation domain restriction}%
\UnicodeMathSymbol{"025C2}{\smallblacktriangleleft   }{\mathord}{left triangle, filled}%
\UnicodeMathSymbol{"025C3}{\smalltriangleleft        }{\mathord}{left triangle, open}%
\UnicodeMathSymbol{"025C4}{\blackpointerleft         }{\mathord}{black left-pointing pointer}%
\UnicodeMathSymbol{"025C5}{\whitepointerleft         }{\mathord}{white left-pointing pointer}%
\UnicodeMathSymbol{"025C6}{\mdlgblkdiamond           }{\mathord}{black diamond}%
\UnicodeMathSymbol{"025C7}{\mdlgwhtdiamond           }{\mathord}{white diamond; diamond, open}%
\UnicodeMathSymbol{"025C8}{\blackinwhitediamond      }{\mathord}{white diamond containing black small diamond}%
\UnicodeMathSymbol{"025C9}{\fisheye                  }{\mathord}{fisheye}%
\UnicodeMathSymbol{"025CA}{\mdlgwhtlozenge           }{\mathord}{lozenge or total mark}%
\UnicodeMathSymbol{"025CB}{\mdlgwhtcircle            }{\mathbin}{medium large circle}%
\UnicodeMathSymbol{"025CC}{\dottedcircle             }{\mathord}{dotted circle}%
\UnicodeMathSymbol{"025CD}{\circlevertfill           }{\mathord}{circle with vertical fill}%
\UnicodeMathSymbol{"025CE}{\bullseye                 }{\mathord}{bullseye}%
\UnicodeMathSymbol{"025CF}{\mdlgblkcircle            }{\mathord}{circle, filled}%
\UnicodeMathSymbol{"025D0}{\circlelefthalfblack      }{\mathord}{circle, filled left half [harvey ball]}%
\UnicodeMathSymbol{"025D1}{\circlerighthalfblack     }{\mathord}{circle, filled right half}%
\UnicodeMathSymbol{"025D2}{\circlebottomhalfblack    }{\mathord}{circle, filled bottom half}%
\UnicodeMathSymbol{"025D3}{\circletophalfblack       }{\mathord}{circle, filled top half}%
\UnicodeMathSymbol{"025D4}{\circleurquadblack        }{\mathord}{circle with upper right quadrant black}%
\UnicodeMathSymbol{"025D5}{\blackcircleulquadwhite   }{\mathord}{circle with all but upper left quadrant black}%
\UnicodeMathSymbol{"025D6}{\blacklefthalfcircle      }{\mathord}{left half black circle}%
\UnicodeMathSymbol{"025D7}{\blackrighthalfcircle     }{\mathord}{right half black circle}%
\UnicodeMathSymbol{"025D8}{\inversebullet            }{\mathord}{inverse bullet }%
\UnicodeMathSymbol{"025D9}{\inversewhitecircle       }{\mathord}{inverse white circle}%
\UnicodeMathSymbol{"025DA}{\invwhiteupperhalfcircle  }{\mathord}{upper half inverse white circle}%
\UnicodeMathSymbol{"025DB}{\invwhitelowerhalfcircle  }{\mathord}{lower half inverse white circle}%
\UnicodeMathSymbol{"025DC}{\ularc                    }{\mathord}{upper left quadrant circular arc}%
\UnicodeMathSymbol{"025DD}{\urarc                    }{\mathord}{upper right quadrant circular arc}%
\UnicodeMathSymbol{"025DE}{\lrarc                    }{\mathord}{lower right quadrant circular arc}%
\UnicodeMathSymbol{"025DF}{\llarc                    }{\mathord}{lower left quadrant circular arc}%
\UnicodeMathSymbol{"025E0}{\topsemicircle            }{\mathord}{upper half circle}%
\UnicodeMathSymbol{"025E1}{\botsemicircle            }{\mathord}{lower half circle}%
\UnicodeMathSymbol{"025E2}{\lrblacktriangle          }{\mathord}{lower right triangle, filled}%
\UnicodeMathSymbol{"025E3}{\llblacktriangle          }{\mathord}{lower left triangle, filled}%
\UnicodeMathSymbol{"025E4}{\ulblacktriangle          }{\mathord}{upper left triangle, filled}%
\UnicodeMathSymbol{"025E5}{\urblacktriangle          }{\mathord}{upper right triangle, filled}%
\UnicodeMathSymbol{"025E6}{\smwhtcircle              }{\mathord}{white bullet}%
\UnicodeMathSymbol{"025E7}{\squareleftblack          }{\mathord}{square, filled left half}%
\UnicodeMathSymbol{"025E8}{\squarerightblack         }{\mathord}{square, filled right half}%
\UnicodeMathSymbol{"025E9}{\squareulblack            }{\mathord}{square, filled top left corner}%
\UnicodeMathSymbol{"025EA}{\squarelrblack            }{\mathord}{square, filled bottom right corner}%
\UnicodeMathSymbol{"025EB}{\boxbar                   }{\mathbin}{vertical bar in box}%
\UnicodeMathSymbol{"025EC}{\trianglecdot             }{\mathord}{triangle with centered dot}%
\UnicodeMathSymbol{"025ED}{\triangleleftblack        }{\mathord}{up-pointing triangle with left half black}%
\UnicodeMathSymbol{"025EE}{\trianglerightblack       }{\mathord}{up-pointing triangle with right half black}%
\UnicodeMathSymbol{"025EF}{\lgwhtcircle              }{\mathord}{large circle}%
\UnicodeMathSymbol{"025F0}{\squareulquad             }{\mathord}{white square with upper left quadrant}%
\UnicodeMathSymbol{"025F1}{\squarellquad             }{\mathord}{white square with lower left quadrant}%
\UnicodeMathSymbol{"025F2}{\squarelrquad             }{\mathord}{white square with lower right quadrant}%
\UnicodeMathSymbol{"025F3}{\squareurquad             }{\mathord}{white square with upper right quadrant}%
\UnicodeMathSymbol{"025F4}{\circleulquad             }{\mathord}{white circle with upper left quadrant}%
\UnicodeMathSymbol{"025F5}{\circlellquad             }{\mathord}{white circle with lower left quadrant}%
\UnicodeMathSymbol{"025F6}{\circlelrquad             }{\mathord}{white circle with lower right quadrant}%
\UnicodeMathSymbol{"025F7}{\circleurquad             }{\mathord}{white circle with upper right quadrant}%
\UnicodeMathSymbol{"025F8}{\ultriangle               }{\mathord}{upper left triangle}%
\UnicodeMathSymbol{"025F9}{\urtriangle               }{\mathord}{upper right triangle}%
\UnicodeMathSymbol{"025FA}{\lltriangle               }{\mathord}{lower left triangle}%
\UnicodeMathSymbol{"025FB}{\mdwhtsquare              }{\mathord}{white medium square}%
\UnicodeMathSymbol{"025FC}{\mdblksquare              }{\mathord}{black medium square}%
\UnicodeMathSymbol{"025FD}{\mdsmwhtsquare            }{\mathord}{white medium small square}%
\UnicodeMathSymbol{"025FE}{\mdsmblksquare            }{\mathord}{black medium small square}%
\UnicodeMathSymbol{"025FF}{\lrtriangle               }{\mathord}{lower right triangle}%
\UnicodeMathSymbol{"02605}{\bigstar                  }{\mathord}{star, filled}%
\UnicodeMathSymbol{"02606}{\bigwhitestar             }{\mathord}{star, open}%
\UnicodeMathSymbol{"02609}{\astrosun                 }{\mathord}{sun}%
\UnicodeMathSymbol{"02621}{\danger                   }{\mathord}{dangerous bend (caution sign)}%
\UnicodeMathSymbol{"0263B}{\blacksmiley              }{\mathord}{black smiling face}%
\UnicodeMathSymbol{"0263C}{\sun                      }{\mathord}{white sun with rays}%
\UnicodeMathSymbol{"0263D}{\rightmoon                }{\mathord}{first quarter moon}%
\UnicodeMathSymbol{"0263E}{\leftmoon                 }{\mathord}{last quarter moon}%
\UnicodeMathSymbol{"02640}{\female                   }{\mathord}{venus, female}%
\UnicodeMathSymbol{"02642}{\male                     }{\mathord}{mars, male}%
\UnicodeMathSymbol{"02660}{\spadesuit                }{\mathord}{spades suit symbol}%
\UnicodeMathSymbol{"02661}{\heartsuit                }{\mathord}{heart suit symbol}%
\UnicodeMathSymbol{"02662}{\diamondsuit              }{\mathord}{diamond suit symbol}%
\UnicodeMathSymbol{"02663}{\clubsuit                 }{\mathord}{club suit symbol}%
\UnicodeMathSymbol{"02664}{\varspadesuit             }{\mathord}{spade, white (card suit)}%
\UnicodeMathSymbol{"02665}{\varheartsuit             }{\mathord}{filled heart (card suit)}%
\UnicodeMathSymbol{"02666}{\vardiamondsuit           }{\mathord}{filled diamond (card suit)}%
\UnicodeMathSymbol{"02667}{\varclubsuit              }{\mathord}{club, white (card suit)}%
\UnicodeMathSymbol{"02669}{\quarternote              }{\mathord}{music note (sung text sign)}%
\UnicodeMathSymbol{"0266A}{\eighthnote               }{\mathord}{eighth note}%
\UnicodeMathSymbol{"0266B}{\twonotes                 }{\mathord}{beamed eighth notes}%
\UnicodeMathSymbol{"0266D}{\flat                     }{\mathord}{musical flat}%
\UnicodeMathSymbol{"0266E}{\natural                  }{\mathord}{music natural}%
\UnicodeMathSymbol{"0266F}{\sharp                    }{\mathord}{musical sharp}%
\UnicodeMathSymbol{"0267E}{\acidfree                 }{\mathord}{permanent paper sign}%
\UnicodeMathSymbol{"02680}{\dicei                    }{\mathord}{die face-1}%
\UnicodeMathSymbol{"02681}{\diceii                   }{\mathord}{die face-2}%
\UnicodeMathSymbol{"02682}{\diceiii                  }{\mathord}{die face-3}%
\UnicodeMathSymbol{"02683}{\diceiv                   }{\mathord}{die face-4}%
\UnicodeMathSymbol{"02684}{\dicev                    }{\mathord}{die face-5}%
\UnicodeMathSymbol{"02685}{\dicevi                   }{\mathord}{die face-6}%
\UnicodeMathSymbol{"02686}{\circledrightdot          }{\mathord}{white circle with dot right}%
\UnicodeMathSymbol{"02687}{\circledtwodots           }{\mathord}{white circle with two dots}%
\UnicodeMathSymbol{"02688}{\blackcircledrightdot     }{\mathord}{black circle with white dot right}%
\UnicodeMathSymbol{"02689}{\blackcircledtwodots      }{\mathord}{black circle with two white dots}%
\UnicodeMathSymbol{"026A5}{\Hermaphrodite            }{\mathord}{male and female sign}%
\UnicodeMathSymbol{"026AA}{\mdwhtcircle              }{\mathord}{medium white circle}%
\UnicodeMathSymbol{"026AB}{\mdblkcircle              }{\mathord}{medium black circle}%
\UnicodeMathSymbol{"026AC}{\mdsmwhtcircle            }{\mathord}{medium small white circle}%
\UnicodeMathSymbol{"026B2}{\neuter                   }{\mathord}{neuter}%
\UnicodeMathSymbol{"02713}{\checkmark                }{\mathord}{tick, check mark}%
\UnicodeMathSymbol{"02720}{\maltese                  }{\mathord}{maltese cross}%
\UnicodeMathSymbol{"0272A}{\circledstar              }{\mathord}{circled white star}%
\UnicodeMathSymbol{"02736}{\varstar                  }{\mathord}{six pointed black star}%
\UnicodeMathSymbol{"0273D}{\dingasterisk             }{\mathord}{heavy teardrop-spoked asterisk}%
\UnicodeMathSymbol{"02772}{\lbrbrak                  }{\mathopen}{light left tortoise shell bracket ornament}%
\UnicodeMathSymbol{"02773}{\rbrbrak                  }{\mathclose}{light right tortoise shell bracket ornament}%
\UnicodeMathSymbol{"0279B}{\draftingarrow            }{\mathord}{right arrow with bold head (drafting)}%
\UnicodeMathSymbol{"027C0}{\threedangle              }{\mathord}{three dimensional angle}%
\UnicodeMathSymbol{"027C1}{\whiteinwhitetriangle     }{\mathord}{white triangle containing small white triangle}%
\UnicodeMathSymbol{"027C2}{\perp                     }{\mathrel}{perpendicular}%
\UnicodeMathSymbol{"027C3}{\subsetcirc               }{\mathord}{open subset}%
\UnicodeMathSymbol{"027C4}{\supsetcirc               }{\mathord}{open superset}%
\UnicodeMathSymbol{"027C5}{\lbag                     }{\mathopen}{left s-shaped bag delimiter}%
\UnicodeMathSymbol{"027C6}{\rbag                     }{\mathclose}{right s-shaped bag delimiter}%
\UnicodeMathSymbol{"027C7}{\veedot                   }{\mathbin}{or with dot inside}%
\UnicodeMathSymbol{"027C8}{\bsolhsub                 }{\mathrel}{reverse solidus preceding subset}%
\UnicodeMathSymbol{"027C9}{\suphsol                  }{\mathrel}{superset preceding solidus}%
\UnicodeMathSymbol{"027CC}{\longdivision             }{\mathopen}{long division}%
\UnicodeMathSymbol{"027D0}{\diamondcdot              }{\mathord}{white diamond with centred dot}%
\UnicodeMathSymbol{"027D1}{\wedgedot                 }{\mathbin}{and with dot}%
\UnicodeMathSymbol{"027D2}{\upin                     }{\mathrel}{element of opening upwards}%
\UnicodeMathSymbol{"027D3}{\pullback                 }{\mathrel}{lower right corner with dot}%
\UnicodeMathSymbol{"027D4}{\pushout                  }{\mathrel}{upper left corner with dot}%
\UnicodeMathSymbol{"027D5}{\leftouterjoin            }{\mathop}{left outer join}%
\UnicodeMathSymbol{"027D6}{\rightouterjoin           }{\mathop}{right outer join}%
\UnicodeMathSymbol{"027D7}{\fullouterjoin            }{\mathop}{full outer join}%
\UnicodeMathSymbol{"027D8}{\bigbot                   }{\mathop}{large up tack}%
\UnicodeMathSymbol{"027D9}{\bigtop                   }{\mathop}{large down tack}%
\UnicodeMathSymbol{"027DA}{\DashVDash                }{\mathrel}{left and right double turnstile}%
\UnicodeMathSymbol{"027DB}{\dashVdash                }{\mathrel}{left and right tack}%
\UnicodeMathSymbol{"027DC}{\multimapinv              }{\mathrel}{left multimap}%
\UnicodeMathSymbol{"027DD}{\vlongdash                }{\mathrel}{long left tack}%
\UnicodeMathSymbol{"027DE}{\longdashv                }{\mathrel}{long right tack}%
\UnicodeMathSymbol{"027DF}{\cirbot                   }{\mathrel}{up tack with circle above}%
\UnicodeMathSymbol{"027E0}{\lozengeminus             }{\mathbin}{lozenge divided by horizontal rule}%
\UnicodeMathSymbol{"027E1}{\concavediamond           }{\mathbin}{white concave-sided diamond}%
\UnicodeMathSymbol{"027E2}{\concavediamondtickleft   }{\mathbin}{white concave-sided diamond with leftwards tick}%
\UnicodeMathSymbol{"027E3}{\concavediamondtickright  }{\mathbin}{white concave-sided diamond with rightwards tick}%
\UnicodeMathSymbol{"027E4}{\whitesquaretickleft      }{\mathbin}{white square with leftwards tick}%
\UnicodeMathSymbol{"027E5}{\whitesquaretickright     }{\mathbin}{white square with rightwards tick}%
\UnicodeMathSymbol{"027E6}{\lBrack                   }{\mathopen}{mathematical left white square bracket}%
\UnicodeMathSymbol{"027E7}{\rBrack                   }{\mathclose}{mathematical right white square bracket}%
\UnicodeMathSymbol{"027E8}{\langle                   }{\mathopen}{mathematical left angle bracket}%
\UnicodeMathSymbol{"027E9}{\rangle                   }{\mathclose}{mathematical right angle bracket}%
\UnicodeMathSymbol{"027EA}{\lAngle                   }{\mathopen}{mathematical left double angle bracket}%
\UnicodeMathSymbol{"027EB}{\rAngle                   }{\mathclose}{mathematical right double angle bracket}%
\UnicodeMathSymbol{"027EC}{\Lbrbrak                  }{\mathopen}{mathematical left white tortoise shell bracket}%
\UnicodeMathSymbol{"027ED}{\Rbrbrak                  }{\mathclose}{mathematical right white tortoise shell bracket}%
\UnicodeMathSymbol{"027EE}{\lgroup                   }{\mathopen}{mathematical left flattened parenthesis}%
\UnicodeMathSymbol{"027EF}{\rgroup                   }{\mathclose}{mathematical right flattened parenthesis}%
\UnicodeMathSymbol{"027F0}{\UUparrow                 }{\mathrel}{upwards quadruple arrow}%
\UnicodeMathSymbol{"027F1}{\DDownarrow               }{\mathrel}{downwards quadruple arrow}%
\UnicodeMathSymbol{"027F2}{\acwgapcirclearrow        }{\mathrel}{anticlockwise gapped circle arrow}%
\UnicodeMathSymbol{"027F3}{\cwgapcirclearrow         }{\mathrel}{clockwise gapped circle arrow}%
\UnicodeMathSymbol{"027F4}{\rightarrowonoplus        }{\mathrel}{right arrow with circled plus}%
\UnicodeMathSymbol{"027F5}{\longleftarrow            }{\mathrel}{long leftwards arrow}%
\UnicodeMathSymbol{"027F6}{\longrightarrow           }{\mathrel}{long rightwards arrow}%
\UnicodeMathSymbol{"027F7}{\longleftrightarrow       }{\mathrel}{long left right arrow}%
\UnicodeMathSymbol{"027F8}{\Longleftarrow            }{\mathrel}{long leftwards double arrow}%
\UnicodeMathSymbol{"027F9}{\Longrightarrow           }{\mathrel}{long rightwards double arrow}%
\UnicodeMathSymbol{"027FA}{\Longleftrightarrow       }{\mathrel}{long left right double arrow}%
\UnicodeMathSymbol{"027FB}{\longmapsfrom             }{\mathrel}{long leftwards arrow from bar}%
\UnicodeMathSymbol{"027FC}{\longmapsto               }{\mathrel}{long rightwards arrow from bar}%
\UnicodeMathSymbol{"027FD}{\Longmapsfrom             }{\mathrel}{long leftwards double arrow from bar}%
\UnicodeMathSymbol{"027FE}{\Longmapsto               }{\mathrel}{long rightwards double arrow from bar}%
\UnicodeMathSymbol{"027FF}{\longrightsquigarrow      }{\mathrel}{long rightwards squiggle arrow}%
\UnicodeMathSymbol{"02900}{\nvtwoheadrightarrow      }{\mathrel}{rightwards two-headed arrow with vertical stroke}%
\UnicodeMathSymbol{"02901}{\nVtwoheadrightarrow      }{\mathrel}{rightwards two-headed arrow with double vertical stroke}%
\UnicodeMathSymbol{"02902}{\nvLeftarrow              }{\mathrel}{leftwards double arrow with vertical stroke}%
\UnicodeMathSymbol{"02903}{\nvRightarrow             }{\mathrel}{rightwards double arrow with vertical stroke}%
\UnicodeMathSymbol{"02904}{\nvLeftrightarrow         }{\mathrel}{left right double arrow with vertical stroke}%
\UnicodeMathSymbol{"02905}{\twoheadmapsto            }{\mathrel}{rightwards two-headed arrow from bar}%
\UnicodeMathSymbol{"02906}{\Mapsfrom                 }{\mathrel}{leftwards double arrow from bar}%
\UnicodeMathSymbol{"02907}{\Mapsto                   }{\mathrel}{rightwards double arrow from bar}%
\UnicodeMathSymbol{"02908}{\downarrowbarred          }{\mathrel}{downwards arrow with horizontal stroke}%
\UnicodeMathSymbol{"02909}{\uparrowbarred            }{\mathrel}{upwards arrow with horizontal stroke}%
\UnicodeMathSymbol{"0290A}{\Uuparrow                 }{\mathrel}{upwards triple arrow}%
\UnicodeMathSymbol{"0290B}{\Ddownarrow               }{\mathrel}{downwards triple arrow}%
\UnicodeMathSymbol{"0290C}{\leftbkarrow              }{\mathrel}{leftwards double dash arrow}%
\UnicodeMathSymbol{"0290D}{\rightbkarrow             }{\mathrel}{rightwards double dash arrow}%
\UnicodeMathSymbol{"0290E}{\leftdbkarrow             }{\mathrel}{leftwards triple dash arrow}%
\UnicodeMathSymbol{"0290F}{\dbkarrow                  }{\mathrel}{rightwards triple dash arrow}%
\UnicodeMathSymbol{"02910}{\drbkarrow                 }{\mathrel}{rightwards two-headed triple dash arrow}%
\UnicodeMathSymbol{"02911}{\rightdotarrow            }{\mathrel}{rightwards arrow with dotted stem}%
\UnicodeMathSymbol{"02912}{\baruparrow               }{\mathrel}{upwards arrow to bar}%
\UnicodeMathSymbol{"02913}{\downarrowbar             }{\mathrel}{downwards arrow to bar}%
\UnicodeMathSymbol{"02914}{\nvrightarrowtail         }{\mathrel}{rightwards arrow with tail with vertical stroke}%
\UnicodeMathSymbol{"02915}{\nVrightarrowtail         }{\mathrel}{rightwards arrow with tail with double vertical stroke}%
\UnicodeMathSymbol{"02916}{\twoheadrightarrowtail    }{\mathrel}{rightwards two-headed arrow with tail}%
\UnicodeMathSymbol{"02917}{\nvtwoheadrightarrowtail  }{\mathrel}{rightwards two-headed arrow with tail with vertical stroke}%
\UnicodeMathSymbol{"02918}{\nVtwoheadrightarrowtail  }{\mathrel}{rightwards two-headed arrow with tail with double vertical stroke}%
\UnicodeMathSymbol{"02919}{\lefttail                 }{\mathrel}{leftwards arrow-tail}%
\UnicodeMathSymbol{"0291A}{\righttail                }{\mathrel}{rightwards arrow-tail}%
\UnicodeMathSymbol{"0291B}{\leftdbltail              }{\mathrel}{leftwards double arrow-tail}%
\UnicodeMathSymbol{"0291C}{\rightdbltail             }{\mathrel}{rightwards double arrow-tail}%
\UnicodeMathSymbol{"0291D}{\diamondleftarrow         }{\mathrel}{leftwards arrow to black diamond}%
\UnicodeMathSymbol{"0291E}{\rightarrowdiamond        }{\mathrel}{rightwards arrow to black diamond}%
\UnicodeMathSymbol{"0291F}{\diamondleftarrowbar      }{\mathrel}{leftwards arrow from bar to black diamond}%
\UnicodeMathSymbol{"02920}{\barrightarrowdiamond     }{\mathrel}{rightwards arrow from bar to black diamond}%
\UnicodeMathSymbol{"02921}{\nwsearrow                }{\mathrel}{north west and south east arrow}%
\UnicodeMathSymbol{"02922}{\neswarrow                }{\mathrel}{north east and south west arrow}%
\UnicodeMathSymbol{"02923}{\hknwarrow                }{\mathrel}{north west arrow with hook}%
\UnicodeMathSymbol{"02924}{\hknearrow                }{\mathrel}{north east arrow with hook}%
\UnicodeMathSymbol{"02925}{\hksearrow                 }{\mathrel}{south east arrow with hook}%
\UnicodeMathSymbol{"02926}{\hkswarrow                 }{\mathrel}{south west arrow with hook}%
\UnicodeMathSymbol{"02927}{\tona                     }{\mathrel}{north west arrow and north east arrow}%
\UnicodeMathSymbol{"02928}{\toea                     }{\mathrel}{north east arrow and south east arrow}%
\UnicodeMathSymbol{"02929}{\tosa                     }{\mathrel}{south east arrow and south west arrow}%
\UnicodeMathSymbol{"0292A}{\towa                     }{\mathrel}{south west arrow and north west arrow}%
\UnicodeMathSymbol{"0292B}{\rdiagovfdiag             }{\mathord}{rising diagonal crossing falling diagonal}%
\UnicodeMathSymbol{"0292C}{\fdiagovrdiag             }{\mathord}{falling diagonal crossing rising diagonal}%
\UnicodeMathSymbol{"0292D}{\seovnearrow              }{\mathord}{south east arrow crossing north east arrow}%
\UnicodeMathSymbol{"0292E}{\neovsearrow              }{\mathord}{north east arrow crossing south east arrow}%
\UnicodeMathSymbol{"0292F}{\fdiagovnearrow           }{\mathord}{falling diagonal crossing north east arrow}%
\UnicodeMathSymbol{"02930}{\rdiagovsearrow           }{\mathord}{rising diagonal crossing south east arrow}%
\UnicodeMathSymbol{"02931}{\neovnwarrow              }{\mathord}{north east arrow crossing north west arrow}%
\UnicodeMathSymbol{"02932}{\nwovnearrow              }{\mathord}{north west arrow crossing north east arrow}%
\UnicodeMathSymbol{"02933}{\rightcurvedarrow         }{\mathrel}{wave arrow pointing directly right}%
\UnicodeMathSymbol{"02934}{\uprightcurvearrow        }{\mathord}{arrow pointing rightwards then curving upwards}%
\UnicodeMathSymbol{"02935}{\downrightcurvedarrow     }{\mathord}{arrow pointing rightwards then curving downwards}%
\UnicodeMathSymbol{"02936}{\leftdowncurvedarrow      }{\mathrel}{arrow pointing downwards then curving leftwards}%
\UnicodeMathSymbol{"02937}{\rightdowncurvedarrow     }{\mathrel}{arrow pointing downwards then curving rightwards}%
\UnicodeMathSymbol{"02938}{\cwrightarcarrow          }{\mathrel}{right-side arc clockwise arrow}%
\UnicodeMathSymbol{"02939}{\acwleftarcarrow          }{\mathrel}{left-side arc anticlockwise arrow}%
\UnicodeMathSymbol{"0293A}{\acwoverarcarrow          }{\mathrel}{top arc anticlockwise arrow}%
\UnicodeMathSymbol{"0293B}{\acwunderarcarrow         }{\mathrel}{bottom arc anticlockwise arrow}%
\UnicodeMathSymbol{"0293C}{\curvearrowrightminus     }{\mathrel}{top arc clockwise arrow with minus}%
\UnicodeMathSymbol{"0293D}{\curvearrowleftplus       }{\mathrel}{top arc anticlockwise arrow with plus}%
\UnicodeMathSymbol{"0293E}{\cwundercurvearrow        }{\mathrel}{lower right semicircular clockwise arrow}%
\UnicodeMathSymbol{"0293F}{\ccwundercurvearrow       }{\mathrel}{lower left semicircular anticlockwise arrow}%
\UnicodeMathSymbol{"02940}{\acwcirclearrow           }{\mathrel}{anticlockwise closed circle arrow}%
\UnicodeMathSymbol{"02941}{\cwcirclearrow            }{\mathrel}{clockwise closed circle arrow}%
\UnicodeMathSymbol{"02942}{\rightarrowshortleftarrow }{\mathrel}{rightwards arrow above short leftwards arrow}%
\UnicodeMathSymbol{"02943}{\leftarrowshortrightarrow }{\mathrel}{leftwards arrow above short rightwards arrow}%
\UnicodeMathSymbol{"02944}{\shortrightarrowleftarrow }{\mathrel}{short rightwards arrow above leftwards arrow}%
\UnicodeMathSymbol{"02945}{\rightarrowplus           }{\mathrel}{rightwards arrow with plus below}%
\UnicodeMathSymbol{"02946}{\leftarrowplus            }{\mathrel}{leftwards arrow with plus below}%
\UnicodeMathSymbol{"02947}{\rightarrowx              }{\mathrel}{rightwards arrow through x}%
\UnicodeMathSymbol{"02948}{\leftrightarrowcircle     }{\mathrel}{left right arrow through small circle}%
\UnicodeMathSymbol{"02949}{\twoheaduparrowcircle     }{\mathrel}{upwards two-headed arrow from small circle}%
\UnicodeMathSymbol{"0294A}{\leftrightharpoonupdown   }{\mathrel}{left barb up right barb down harpoon}%
\UnicodeMathSymbol{"0294B}{\leftrightharpoondownup   }{\mathrel}{left barb down right barb up harpoon}%
\UnicodeMathSymbol{"0294C}{\updownharpoonrightleft   }{\mathrel}{up barb right down barb left harpoon}%
\UnicodeMathSymbol{"0294D}{\updownharpoonleftright   }{\mathrel}{up barb left down barb right harpoon}%
\UnicodeMathSymbol{"0294E}{\leftrightharpoonupup     }{\mathrel}{left barb up right barb up harpoon}%
\UnicodeMathSymbol{"0294F}{\updownharpoonrightright  }{\mathrel}{up barb right down barb right harpoon}%
\UnicodeMathSymbol{"02950}{\leftrightharpoondowndown }{\mathrel}{left barb down right barb down harpoon}%
\UnicodeMathSymbol{"02951}{\updownharpoonleftleft    }{\mathrel}{up barb left down barb left harpoon}%
\UnicodeMathSymbol{"02952}{\barleftharpoonup         }{\mathrel}{leftwards harpoon with barb up to bar}%
\UnicodeMathSymbol{"02953}{\rightharpoonupbar        }{\mathrel}{rightwards harpoon with barb up to bar}%
\UnicodeMathSymbol{"02954}{\barupharpoonright        }{\mathrel}{upwards harpoon with barb right to bar}%
\UnicodeMathSymbol{"02955}{\downharpoonrightbar      }{\mathrel}{downwards harpoon with barb right to bar}%
\UnicodeMathSymbol{"02956}{\barleftharpoondown       }{\mathrel}{leftwards harpoon with barb down to bar}%
\UnicodeMathSymbol{"02957}{\rightharpoondownbar      }{\mathrel}{rightwards harpoon with barb down to bar}%
\UnicodeMathSymbol{"02958}{\barupharpoonleft         }{\mathrel}{upwards harpoon with barb left to bar}%
\UnicodeMathSymbol{"02959}{\downharpoonleftbar       }{\mathrel}{downwards harpoon with barb left to bar}%
\UnicodeMathSymbol{"0295A}{\leftharpoonupbar         }{\mathrel}{leftwards harpoon with barb up from bar}%
\UnicodeMathSymbol{"0295B}{\barrightharpoonup        }{\mathrel}{rightwards harpoon with barb up from bar}%
\UnicodeMathSymbol{"0295C}{\upharpoonrightbar        }{\mathrel}{upwards harpoon with barb right from bar}%
\UnicodeMathSymbol{"0295D}{\bardownharpoonright      }{\mathrel}{downwards harpoon with barb right from bar}%
\UnicodeMathSymbol{"0295E}{\leftharpoondownbar       }{\mathrel}{leftwards harpoon with barb down from bar}%
\UnicodeMathSymbol{"0295F}{\barrightharpoondown      }{\mathrel}{rightwards harpoon with barb down from bar}%
\UnicodeMathSymbol{"02960}{\upharpoonleftbar         }{\mathrel}{upwards harpoon with barb left from bar}%
\UnicodeMathSymbol{"02961}{\bardownharpoonleft       }{\mathrel}{downwards harpoon with barb left from bar}%
\UnicodeMathSymbol{"02962}{\leftharpoonsupdown       }{\mathrel}{leftwards harpoon with barb up above leftwards harpoon with barb down}%
\UnicodeMathSymbol{"02963}{\upharpoonsleftright      }{\mathrel}{upwards harpoon with barb left beside upwards harpoon with barb right}%
\UnicodeMathSymbol{"02964}{\rightharpoonsupdown      }{\mathrel}{rightwards harpoon with barb up above rightwards harpoon with barb down}%
\UnicodeMathSymbol{"02965}{\downharpoonsleftright    }{\mathrel}{downwards harpoon with barb left beside downwards harpoon with barb right}%
\UnicodeMathSymbol{"02966}{\leftrightharpoonsup      }{\mathrel}{leftwards harpoon with barb up above rightwards harpoon with barb up}%
\UnicodeMathSymbol{"02967}{\leftrightharpoonsdown    }{\mathrel}{leftwards harpoon with barb down above rightwards harpoon with barb down}%
\UnicodeMathSymbol{"02968}{\rightleftharpoonsup      }{\mathrel}{rightwards harpoon with barb up above leftwards harpoon with barb up}%
\UnicodeMathSymbol{"02969}{\rightleftharpoonsdown    }{\mathrel}{rightwards harpoon with barb down above leftwards harpoon with barb down}%
\UnicodeMathSymbol{"0296A}{\leftharpoonupdash        }{\mathrel}{leftwards harpoon with barb up above long dash}%
\UnicodeMathSymbol{"0296B}{\dashleftharpoondown      }{\mathrel}{leftwards harpoon with barb down below long dash}%
\UnicodeMathSymbol{"0296C}{\rightharpoonupdash       }{\mathrel}{rightwards harpoon with barb up above long dash}%
\UnicodeMathSymbol{"0296D}{\dashrightharpoondown     }{\mathrel}{rightwards harpoon with barb down below long dash}%
\UnicodeMathSymbol{"0296E}{\updownharpoonsleftright  }{\mathrel}{upwards harpoon with barb left beside downwards harpoon with barb right}%
\UnicodeMathSymbol{"0296F}{\downupharpoonsleftright  }{\mathrel}{downwards harpoon with barb left beside upwards harpoon with barb right}%
\UnicodeMathSymbol{"02970}{\rightimply               }{\mathrel}{right double arrow with rounded head}%
\UnicodeMathSymbol{"02971}{\equalrightarrow          }{\mathrel}{equals sign above rightwards arrow}%
\UnicodeMathSymbol{"02972}{\similarrightarrow        }{\mathrel}{tilde operator above rightwards arrow}%
\UnicodeMathSymbol{"02973}{\leftarrowsimilar         }{\mathrel}{leftwards arrow above tilde operator}%
\UnicodeMathSymbol{"02974}{\rightarrowsimilar        }{\mathrel}{rightwards arrow above tilde operator}%
\UnicodeMathSymbol{"02975}{\rightarrowapprox         }{\mathrel}{rightwards arrow above almost equal to}%
\UnicodeMathSymbol{"02976}{\ltlarr                   }{\mathrel}{less-than above leftwards arrow}%
\UnicodeMathSymbol{"02977}{\leftarrowless            }{\mathrel}{leftwards arrow through less-than}%
\UnicodeMathSymbol{"02978}{\gtrarr                   }{\mathrel}{greater-than above rightwards arrow}%
\UnicodeMathSymbol{"02979}{\subrarr                  }{\mathrel}{subset above rightwards arrow}%
\UnicodeMathSymbol{"0297A}{\leftarrowsubset          }{\mathrel}{leftwards arrow through subset}%
\UnicodeMathSymbol{"0297B}{\suplarr                  }{\mathrel}{superset above leftwards arrow}%
\UnicodeMathSymbol{"0297C}{\leftfishtail             }{\mathrel}{left fish tail}%
\UnicodeMathSymbol{"0297D}{\rightfishtail            }{\mathrel}{right fish tail}%
\UnicodeMathSymbol{"0297E}{\upfishtail               }{\mathrel}{up fish tail}%
\UnicodeMathSymbol{"0297F}{\downfishtail             }{\mathrel}{down fish tail}%
\UnicodeMathSymbol{"02980}{\Vvert                    }{\mathfence}{triple vertical bar delimiter}%
\UnicodeMathSymbol{"02981}{\mdsmblkcircle            }{\mathord}{z notation spot}%
\UnicodeMathSymbol{"02982}{\typecolon                }{\mathrel}{z notation type colon}%
\UnicodeMathSymbol{"02983}{\lBrace                   }{\mathopen}{left white curly bracket}%
\UnicodeMathSymbol{"02984}{\rBrace                   }{\mathclose}{right white curly bracket}%
\UnicodeMathSymbol{"02985}{\lParen                   }{\mathopen}{left white parenthesis}%
\UnicodeMathSymbol{"02986}{\rParen                   }{\mathclose}{right white parenthesis}%
\UnicodeMathSymbol{"02987}{\llparenthesis            }{\mathopen}{z notation left image bracket}%
\UnicodeMathSymbol{"02988}{\rrparenthesis            }{\mathclose}{z notation right image bracket}%
\UnicodeMathSymbol{"02989}{\llangle                  }{\mathopen}{z notation left binding bracket}%
\UnicodeMathSymbol{"0298A}{\rrangle                  }{\mathclose}{z notation right binding bracket}%
\UnicodeMathSymbol{"0298B}{\lbrackubar               }{\mathopen}{left square bracket with underbar}%
\UnicodeMathSymbol{"0298C}{\rbrackubar               }{\mathclose}{right square bracket with underbar}%
\UnicodeMathSymbol{"0298D}{\lbrackultick             }{\mathopen}{left square bracket with tick in top corner}%
\UnicodeMathSymbol{"0298E}{\rbracklrtick             }{\mathclose}{right square bracket with tick in bottom corner}%
\UnicodeMathSymbol{"0298F}{\lbracklltick             }{\mathopen}{left square bracket with tick in bottom corner}%
\UnicodeMathSymbol{"02990}{\rbrackurtick             }{\mathclose}{right square bracket with tick in top corner}%
\UnicodeMathSymbol{"02991}{\langledot                }{\mathopen}{left angle bracket with dot}%
\UnicodeMathSymbol{"02992}{\rangledot                }{\mathclose}{right angle bracket with dot}%
\UnicodeMathSymbol{"02993}{\lparenless               }{\mathopen}{left arc less-than bracket}%
\UnicodeMathSymbol{"02994}{\rparengtr                }{\mathclose}{right arc greater-than bracket}%
\UnicodeMathSymbol{"02995}{\Lparengtr                }{\mathopen}{double left arc greater-than bracket}%
\UnicodeMathSymbol{"02996}{\Rparenless               }{\mathclose}{double right arc less-than bracket}%
\UnicodeMathSymbol{"02997}{\lblkbrbrak               }{\mathopen}{left black tortoise shell bracket}%
\UnicodeMathSymbol{"02998}{\rblkbrbrak               }{\mathclose}{right black tortoise shell bracket}%
\UnicodeMathSymbol{"02999}{\fourvdots                }{\mathord}{dotted fence}%
\UnicodeMathSymbol{"0299A}{\vzigzag                  }{\mathord}{vertical zigzag line}%
\UnicodeMathSymbol{"0299B}{\measuredangleleft        }{\mathord}{measured angle opening left}%
\UnicodeMathSymbol{"0299C}{\rightanglesqr            }{\mathord}{right angle variant with square}%
\UnicodeMathSymbol{"0299D}{\rightanglemdot           }{\mathord}{measured right angle with dot}%
\UnicodeMathSymbol{"0299E}{\angles                   }{\mathord}{angle with s inside}%
\UnicodeMathSymbol{"0299F}{\angdnr                   }{\mathord}{acute angle}%
\UnicodeMathSymbol{"029A0}{\gtlpar                   }{\mathord}{spherical angle opening left}%
\UnicodeMathSymbol{"029A1}{\sphericalangleup         }{\mathord}{spherical angle opening up}%
\UnicodeMathSymbol{"029A2}{\turnangle                }{\mathord}{turned angle}%
\UnicodeMathSymbol{"029A3}{\revangle                 }{\mathord}{reversed angle}%
\UnicodeMathSymbol{"029A4}{\angleubar                }{\mathord}{angle with underbar}%
\UnicodeMathSymbol{"029A5}{\revangleubar             }{\mathord}{reversed angle with underbar}%
\UnicodeMathSymbol{"029A6}{\wideangledown            }{\mathord}{oblique angle opening up}%
\UnicodeMathSymbol{"029A7}{\wideangleup              }{\mathord}{oblique angle opening down}%
\UnicodeMathSymbol{"029A8}{\measanglerutone          }{\mathord}{measured angle with open arm ending in arrow pointing up and right}%
\UnicodeMathSymbol{"029A9}{\measanglelutonw          }{\mathord}{measured angle with open arm ending in arrow pointing up and left}%
\UnicodeMathSymbol{"029AA}{\measanglerdtose          }{\mathord}{measured angle with open arm ending in arrow pointing down and right}%
\UnicodeMathSymbol{"029AB}{\measangleldtosw          }{\mathord}{measured angle with open arm ending in arrow pointing down and left}%
\UnicodeMathSymbol{"029AC}{\measangleurtone          }{\mathord}{measured angle with open arm ending in arrow pointing right and up}%
\UnicodeMathSymbol{"029AD}{\measangleultonw          }{\mathord}{measured angle with open arm ending in arrow pointing left and up}%
\UnicodeMathSymbol{"029AE}{\measangledrtose          }{\mathord}{measured angle with open arm ending in arrow pointing right and down}%
\UnicodeMathSymbol{"029AF}{\measangledltosw          }{\mathord}{measured angle with open arm ending in arrow pointing left and down}%
\UnicodeMathSymbol{"029B0}{\revemptyset              }{\mathord}{reversed empty set}%
\UnicodeMathSymbol{"029B1}{\emptysetobar             }{\mathord}{empty set with overbar}%
\UnicodeMathSymbol{"029B2}{\emptysetocirc            }{\mathord}{empty set with small circle above}%
\UnicodeMathSymbol{"029B3}{\emptysetoarr             }{\mathord}{empty set with right arrow above}%
\UnicodeMathSymbol{"029B4}{\emptysetoarrl            }{\mathord}{empty set with left arrow above}%
\UnicodeMathSymbol{"029B5}{\circlehbar               }{\mathbin}{circle with horizontal bar}%
\UnicodeMathSymbol{"029B6}{\circledvert              }{\mathbin}{circled vertical bar}%
\UnicodeMathSymbol{"029B7}{\circledparallel          }{\mathbin}{circled parallel}%
\UnicodeMathSymbol{"029B8}{\obslash                  }{\mathbin}{circled reverse solidus}%
\UnicodeMathSymbol{"029B9}{\operp                    }{\mathbin}{circled perpendicular}%
\UnicodeMathSymbol{"029BA}{\obot                     }{\mathord}{circle divided by horizontal bar and top half divided by vertical bar}%
\UnicodeMathSymbol{"029BB}{\olcross                  }{\mathord}{circle with superimposed x}%
\UnicodeMathSymbol{"029BC}{\odotslashdot             }{\mathord}{circled anticlockwise-rotated division sign}%
\UnicodeMathSymbol{"029BD}{\uparrowoncircle          }{\mathord}{up arrow through circle}%
\UnicodeMathSymbol{"029BE}{\circledwhitebullet       }{\mathord}{circled white bullet}%
\UnicodeMathSymbol{"029BF}{\circledbullet            }{\mathord}{circled bullet}%
\UnicodeMathSymbol{"029C0}{\olessthan                }{\mathbin}{circled less-than}%
\UnicodeMathSymbol{"029C1}{\ogreaterthan             }{\mathbin}{circled greater-than}%
\UnicodeMathSymbol{"029C2}{\cirscir                  }{\mathord}{circle with small circle to the right}%
\UnicodeMathSymbol{"029C3}{\cirE                     }{\mathord}{circle with two horizontal strokes to the right}%
\UnicodeMathSymbol{"029C4}{\boxdiag                  }{\mathbin}{squared rising diagonal slash}%
\UnicodeMathSymbol{"029C5}{\boxbslash                }{\mathbin}{squared falling diagonal slash}%
\UnicodeMathSymbol{"029C6}{\boxast                   }{\mathbin}{squared asterisk}%
\UnicodeMathSymbol{"029C7}{\boxcircle                }{\mathbin}{squared small circle}%
\UnicodeMathSymbol{"029C8}{\boxbox                   }{\mathbin}{squared square}%
\UnicodeMathSymbol{"029C9}{\boxonbox                 }{\mathord}{two joined squares}%
\UnicodeMathSymbol{"029CA}{\triangleodot             }{\mathord}{triangle with dot above}%
\UnicodeMathSymbol{"029CB}{\triangleubar             }{\mathord}{triangle with underbar}%
\UnicodeMathSymbol{"029CC}{\triangles                }{\mathord}{s in triangle}%
\UnicodeMathSymbol{"029CD}{\triangleserifs           }{\mathbin}{triangle with serifs at bottom}%
\UnicodeMathSymbol{"029CE}{\rtriltri                 }{\mathrel}{right triangle above left triangle}%
\UnicodeMathSymbol{"029CF}{\ltrivb                   }{\mathrel}{left triangle beside vertical bar}%
\UnicodeMathSymbol{"029D0}{\vbrtri                   }{\mathrel}{vertical bar beside right triangle}%
\UnicodeMathSymbol{"029D1}{\lfbowtie                 }{\mathrel}{left black bowtie}%
\UnicodeMathSymbol{"029D2}{\rfbowtie                 }{\mathrel}{right black bowtie}%
\UnicodeMathSymbol{"029D3}{\fbowtie                  }{\mathrel}{black bowtie}%
\UnicodeMathSymbol{"029D4}{\lftimes                  }{\mathrel}{left black times}%
\UnicodeMathSymbol{"029D5}{\rftimes                  }{\mathrel}{right black times}%
\UnicodeMathSymbol{"029D6}{\hourglass                }{\mathbin}{white hourglass}%
\UnicodeMathSymbol{"029D7}{\blackhourglass           }{\mathbin}{black hourglass}%
\UnicodeMathSymbol{"029D8}{\lvzigzag                 }{\mathopen}{left wiggly fence}%
\UnicodeMathSymbol{"029D9}{\rvzigzag                 }{\mathclose}{right wiggly fence}%
\UnicodeMathSymbol{"029DA}{\Lvzigzag                 }{\mathopen}{left double wiggly fence}%
\UnicodeMathSymbol{"029DB}{\Rvzigzag                 }{\mathclose}{right double wiggly fence}%
\UnicodeMathSymbol{"029DC}{\iinfin                   }{\mathord}{incomplete infinity}%
\UnicodeMathSymbol{"029DD}{\tieinfty                 }{\mathord}{tie over infinity}%
\UnicodeMathSymbol{"029DE}{\nvinfty                  }{\mathord}{infinity negated with vertical bar}%
\UnicodeMathSymbol{"029DF}{\dualmap                  }{\mathrel}{double-ended multimap}%
\UnicodeMathSymbol{"029E0}{\laplac                   }{\mathord}{square with contoured outline}%
\UnicodeMathSymbol{"029E1}{\lrtriangleeq             }{\mathrel}{increases as}%
\UnicodeMathSymbol{"029E2}{\shuffle                  }{\mathbin}{shuffle product}%
\UnicodeMathSymbol{"029E3}{\eparsl                   }{\mathrel}{equals sign and slanted parallel}%
\UnicodeMathSymbol{"029E4}{\smeparsl                 }{\mathrel}{equals sign and slanted parallel with tilde above}%
\UnicodeMathSymbol{"029E5}{\eqvparsl                 }{\mathrel}{identical to and slanted parallel}%
\UnicodeMathSymbol{"029E6}{\gleichstark              }{\mathrel}{gleich stark}%
\UnicodeMathSymbol{"029E7}{\thermod                  }{\mathord}{thermodynamic}%
\UnicodeMathSymbol{"029E8}{\downtriangleleftblack    }{\mathord}{down-pointing triangle with left half black}%
\UnicodeMathSymbol{"029E9}{\downtrianglerightblack   }{\mathord}{down-pointing triangle with right half black}%
\UnicodeMathSymbol{"029EA}{\blackdiamonddownarrow    }{\mathord}{black diamond with down arrow}%
\UnicodeMathSymbol{"029EB}{\mdlgblklozenge           }{\mathbin}{black lozenge}%
\UnicodeMathSymbol{"029EC}{\circledownarrow          }{\mathord}{white circle with down arrow}%
\UnicodeMathSymbol{"029ED}{\blackcircledownarrow     }{\mathord}{black circle with down arrow}%
\UnicodeMathSymbol{"029EE}{\errbarsquare             }{\mathord}{error-barred white square}%
\UnicodeMathSymbol{"029EF}{\errbarblacksquare        }{\mathord}{error-barred black square}%
\UnicodeMathSymbol{"029F0}{\errbardiamond            }{\mathord}{error-barred white diamond}%
\UnicodeMathSymbol{"029F1}{\errbarblackdiamond       }{\mathord}{error-barred black diamond}%
\UnicodeMathSymbol{"029F2}{\errbarcircle             }{\mathord}{error-barred white circle}%
\UnicodeMathSymbol{"029F3}{\errbarblackcircle        }{\mathord}{error-barred black circle}%
\UnicodeMathSymbol{"029F4}{\ruledelayed              }{\mathrel}{rule-delayed}%
\UnicodeMathSymbol{"029F5}{\setminus                 }{\mathbin}{reverse solidus operator}%
\UnicodeMathSymbol{"029F6}{\dsol                     }{\mathbin}{solidus with overbar}%
\UnicodeMathSymbol{"029F7}{\rsolbar                  }{\mathbin}{reverse solidus with horizontal stroke}%
\UnicodeMathSymbol{"029F8}{\xsol                     }{\mathop}{big solidus}%
\UnicodeMathSymbol{"029F9}{\xbsol                    }{\mathop}{big reverse solidus}%
\UnicodeMathSymbol{"029FA}{\doubleplus               }{\mathbin}{double plus}%
\UnicodeMathSymbol{"029FB}{\tripleplus               }{\mathbin}{triple plus}%
\UnicodeMathSymbol{"029FC}{\lcurvyangle              }{\mathopen}{left pointing curved angle bracket}%
\UnicodeMathSymbol{"029FD}{\rcurvyangle              }{\mathclose}{right pointing curved angle bracket}%
\UnicodeMathSymbol{"029FE}{\tplus                    }{\mathbin}{tiny}%
\UnicodeMathSymbol{"029FF}{\tminus                   }{\mathbin}{miny}%
\UnicodeMathSymbol{"02A00}{\bigodot                  }{\mathop}{n-ary circled dot operator}%
\UnicodeMathSymbol{"02A01}{\bigoplus                 }{\mathop}{n-ary circled plus operator}%
\UnicodeMathSymbol{"02A02}{\bigotimes                }{\mathop}{n-ary circled times operator}%
\UnicodeMathSymbol{"02A03}{\bigcupdot                }{\mathop}{n-ary union operator with dot}%
\UnicodeMathSymbol{"02A04}{\biguplus                 }{\mathop}{n-ary union operator with plus}%
\UnicodeMathSymbol{"02A05}{\bigsqcap                 }{\mathop}{n-ary square intersection operator}%
\UnicodeMathSymbol{"02A06}{\bigsqcup                 }{\mathop}{n-ary square union operator}%
\UnicodeMathSymbol{"02A07}{\conjquant                }{\mathop}{two logical and operator}%
\UnicodeMathSymbol{"02A08}{\disjquant                }{\mathop}{two logical or operator}%
\UnicodeMathSymbol{"02A09}{\bigtimes                 }{\mathop}{n-ary times operator}%
\UnicodeMathSymbol{"02A0A}{\modtwosum                }{\mathop}{modulo two sum}%
\UnicodeMathSymbol{"02A0B}{\sumint                   }{\mathop}{summation with integral}%
\UnicodeMathSymbol{"02A0C}{\iiiint                   }{\mathop}{quadruple integral operator}%
\UnicodeMathSymbol{"02A0D}{\intbar                   }{\mathop}{finite part integral}%
\UnicodeMathSymbol{"02A0E}{\intBar                   }{\mathop}{integral with double stroke}%
\UnicodeMathSymbol{"02A0F}{\fint                     }{\mathop}{integral average with slash}%
\UnicodeMathSymbol{"02A10}{\cirfnint                 }{\mathop}{circulation function}%
\UnicodeMathSymbol{"02A11}{\awint                    }{\mathop}{anticlockwise integration}%
\UnicodeMathSymbol{"02A12}{\rppolint                 }{\mathop}{line integration with rectangular path around pole}%
\UnicodeMathSymbol{"02A13}{\scpolint                 }{\mathop}{line integration with semicircular path around pole}%
\UnicodeMathSymbol{"02A14}{\npolint                  }{\mathop}{line integration not including the pole}%
\UnicodeMathSymbol{"02A15}{\pointint                 }{\mathop}{integral around a point operator}%
\UnicodeMathSymbol{"02A16}{\sqint                    }{\mathop}{quaternion integral operator}%
\UnicodeMathSymbol{"02A17}{\intlarhk                 }{\mathop}{integral with leftwards arrow with hook}%
\UnicodeMathSymbol{"02A18}{\intx                     }{\mathop}{integral with times sign}%
\UnicodeMathSymbol{"02A19}{\intcap                   }{\mathop}{integral with intersection}%
\UnicodeMathSymbol{"02A1A}{\intcup                   }{\mathop}{integral with union}%
\UnicodeMathSymbol{"02A1B}{\upint                    }{\mathop}{integral with overbar}%
\UnicodeMathSymbol{"02A1C}{\lowint                   }{\mathop}{integral with underbar}%
\UnicodeMathSymbol{"02A1D}{\Join                     }{\mathop}{join}%
\UnicodeMathSymbol{"02A1E}{\bigtriangleleft          }{\mathop}{large left triangle operator}%
\UnicodeMathSymbol{"02A1F}{\zcmp                     }{\mathop}{z notation schema composition}%
\UnicodeMathSymbol{"02A20}{\zpipe                    }{\mathop}{z notation schema piping}%
\UnicodeMathSymbol{"02A21}{\zproject                 }{\mathop}{z notation schema projection}%
\UnicodeMathSymbol{"02A22}{\ringplus                 }{\mathbin}{plus sign with small circle above}%
\UnicodeMathSymbol{"02A23}{\plushat                  }{\mathbin}{plus sign with circumflex accent above}%
\UnicodeMathSymbol{"02A24}{\simplus                  }{\mathbin}{plus sign with tilde above}%
\UnicodeMathSymbol{"02A25}{\plusdot                  }{\mathbin}{plus sign with dot below}%
\UnicodeMathSymbol{"02A26}{\plussim                  }{\mathbin}{plus sign with tilde below}%
\UnicodeMathSymbol{"02A27}{\plussubtwo               }{\mathbin}{plus sign with subscript two}%
\UnicodeMathSymbol{"02A28}{\plustrif                 }{\mathbin}{plus sign with black triangle}%
\UnicodeMathSymbol{"02A29}{\commaminus               }{\mathbin}{minus sign with comma above}%
\UnicodeMathSymbol{"02A2A}{\minusdot                 }{\mathbin}{minus sign with dot below}%
\UnicodeMathSymbol{"02A2B}{\minusfdots               }{\mathbin}{minus sign with falling dots}%
\UnicodeMathSymbol{"02A2C}{\minusrdots               }{\mathbin}{minus sign with rising dots}%
\UnicodeMathSymbol{"02A2D}{\opluslhrim               }{\mathbin}{plus sign in left half circle}%
\UnicodeMathSymbol{"02A2E}{\oplusrhrim               }{\mathbin}{plus sign in right half circle}%
\UnicodeMathSymbol{"02A2F}{\vectimes                 }{\mathbin}{vector or cross product}%
\UnicodeMathSymbol{"02A30}{\dottimes                 }{\mathbin}{multiplication sign with dot above}%
\UnicodeMathSymbol{"02A31}{\timesbar                 }{\mathbin}{multiplication sign with underbar}%
\UnicodeMathSymbol{"02A32}{\btimes                   }{\mathbin}{semidirect product with bottom closed}%
\UnicodeMathSymbol{"02A33}{\smashtimes               }{\mathbin}{smash product}%
\UnicodeMathSymbol{"02A34}{\otimeslhrim              }{\mathbin}{multiplication sign in left half circle}%
\UnicodeMathSymbol{"02A35}{\otimesrhrim              }{\mathbin}{multiplication sign in right half circle}%
\UnicodeMathSymbol{"02A36}{\otimeshat                }{\mathbin}{circled multiplication sign with circumflex accent}%
\UnicodeMathSymbol{"02A37}{\Otimes                   }{\mathbin}{multiplication sign in double circle}%
\UnicodeMathSymbol{"02A38}{\odiv                     }{\mathbin}{circled division sign}%
\UnicodeMathSymbol{"02A39}{\triangleplus             }{\mathbin}{plus sign in triangle}%
\UnicodeMathSymbol{"02A3A}{\triangleminus            }{\mathbin}{minus sign in triangle}%
\UnicodeMathSymbol{"02A3B}{\triangletimes            }{\mathbin}{multiplication sign in triangle}%
\UnicodeMathSymbol{"02A3C}{\intprod                  }{\mathbin}{interior product}%
\UnicodeMathSymbol{"02A3D}{\intprodr                 }{\mathbin}{righthand interior product}%
\UnicodeMathSymbol{"02A3E}{\fcmp                     }{\mathbin}{z notation relational composition}%
\UnicodeMathSymbol{"02A3F}{\amalg                    }{\mathbin}{amalgamation or coproduct}%
\UnicodeMathSymbol{"02A40}{\capdot                   }{\mathbin}{intersection with dot}%
\UnicodeMathSymbol{"02A41}{\uminus                   }{\mathbin}{union with minus sign}%
\UnicodeMathSymbol{"02A42}{\barcup                   }{\mathbin}{union with overbar}%
\UnicodeMathSymbol{"02A43}{\barcap                   }{\mathbin}{intersection with overbar}%
\UnicodeMathSymbol{"02A44}{\capwedge                 }{\mathbin}{intersection with logical and}%
\UnicodeMathSymbol{"02A45}{\cupvee                   }{\mathbin}{union with logical or}%
\UnicodeMathSymbol{"02A46}{\cupovercap               }{\mathbin}{union above intersection}%
\UnicodeMathSymbol{"02A47}{\capovercup               }{\mathbin}{intersection above union}%
\UnicodeMathSymbol{"02A48}{\cupbarcap                }{\mathbin}{union above bar above intersection}%
\UnicodeMathSymbol{"02A49}{\capbarcup                }{\mathbin}{intersection above bar above union}%
\UnicodeMathSymbol{"02A4A}{\twocups                  }{\mathbin}{union beside and joined with union}%
\UnicodeMathSymbol{"02A4B}{\twocaps                  }{\mathbin}{intersection beside and joined with intersection}%
\UnicodeMathSymbol{"02A4C}{\closedvarcup             }{\mathbin}{closed union with serifs}%
\UnicodeMathSymbol{"02A4D}{\closedvarcap             }{\mathbin}{closed intersection with serifs}%
\UnicodeMathSymbol{"02A4E}{\Sqcap                    }{\mathbin}{double square intersection}%
\UnicodeMathSymbol{"02A4F}{\Sqcup                    }{\mathbin}{double square union}%
\UnicodeMathSymbol{"02A50}{\closedvarcupsmashprod    }{\mathbin}{closed union with serifs and smash product}%
\UnicodeMathSymbol{"02A51}{\wedgeodot                }{\mathbin}{logical and with dot above}%
\UnicodeMathSymbol{"02A52}{\veeodot                  }{\mathbin}{logical or with dot above}%
\UnicodeMathSymbol{"02A53}{\Wedge                    }{\mathbin}{double logical and}%
\UnicodeMathSymbol{"02A54}{\Vee                      }{\mathbin}{double logical or}%
\UnicodeMathSymbol{"02A55}{\wedgeonwedge             }{\mathbin}{two intersecting logical and}%
\UnicodeMathSymbol{"02A56}{\veeonvee                 }{\mathbin}{two intersecting logical or}%
\UnicodeMathSymbol{"02A57}{\bigslopedvee             }{\mathbin}{sloping large or}%
\UnicodeMathSymbol{"02A58}{\bigslopedwedge           }{\mathbin}{sloping large and}%
\UnicodeMathSymbol{"02A59}{\veeonwedge               }{\mathrel}{logical or overlapping logical and}%
\UnicodeMathSymbol{"02A5A}{\wedgemidvert             }{\mathbin}{logical and with middle stem}%
\UnicodeMathSymbol{"02A5B}{\veemidvert               }{\mathbin}{logical or with middle stem}%
\UnicodeMathSymbol{"02A5C}{\midbarwedge              }{\mathbin}{ogical and with horizontal dash}%
\UnicodeMathSymbol{"02A5D}{\midbarvee                }{\mathbin}{logical or with horizontal dash}%
\UnicodeMathSymbol{"02A5E}{\doublebarwedge           }{\mathbin}{logical and with double overbar}%
\UnicodeMathSymbol{"02A5F}{\wedgebar                 }{\mathbin}{logical and with underbar}%
\UnicodeMathSymbol{"02A60}{\wedgedoublebar           }{\mathbin}{logical and with double underbar}%
\UnicodeMathSymbol{"02A61}{\varveebar                }{\mathbin}{small vee with underbar}%
\UnicodeMathSymbol{"02A62}{\doublebarvee             }{\mathbin}{logical or with double overbar}%
\UnicodeMathSymbol{"02A63}{\veedoublebar             }{\mathbin}{logical or with double underbar}%
\UnicodeMathSymbol{"02A64}{\dsub                     }{\mathbin}{z notation domain antirestriction}%
\UnicodeMathSymbol{"02A65}{\rsub                     }{\mathbin}{z notation range antirestriction}%
\UnicodeMathSymbol{"02A66}{\eqdot                    }{\mathrel}{equals sign with dot below}%
\UnicodeMathSymbol{"02A67}{\dotequiv                 }{\mathrel}{identical with dot above}%
\UnicodeMathSymbol{"02A68}{\equivVert                }{\mathrel}{triple horizontal bar with double vertical stroke}%
\UnicodeMathSymbol{"02A69}{\equivVvert               }{\mathrel}{triple horizontal bar with triple vertical stroke}%
\UnicodeMathSymbol{"02A6A}{\dotsim                   }{\mathrel}{tilde operator with dot above}%
\UnicodeMathSymbol{"02A6B}{\simrdots                 }{\mathrel}{tilde operator with rising dots}%
\UnicodeMathSymbol{"02A6C}{\simminussim              }{\mathrel}{similar minus similar}%
\UnicodeMathSymbol{"02A6D}{\congdot                  }{\mathrel}{congruent with dot above}%
\UnicodeMathSymbol{"02A6E}{\asteq                    }{\mathrel}{equals with asterisk}%
\UnicodeMathSymbol{"02A6F}{\hatapprox                }{\mathrel}{almost equal to with circumflex accent}%
\UnicodeMathSymbol{"02A70}{\approxeqq                }{\mathrel}{approximately equal or equal to}%
\UnicodeMathSymbol{"02A71}{\eqqplus                  }{\mathbin}{equals sign above plus sign}%
\UnicodeMathSymbol{"02A72}{\pluseqq                  }{\mathbin}{plus sign above equals sign}%
\UnicodeMathSymbol{"02A73}{\eqqsim                   }{\mathrel}{equals sign above tilde operator}%
\UnicodeMathSymbol{"02A74}{\Coloneq                  }{\mathrel}{double colon equal}%
\UnicodeMathSymbol{"02A75}{\eqeq                     }{\mathrel}{two consecutive equals signs}%
\UnicodeMathSymbol{"02A76}{\eqeqeq                   }{\mathrel}{three consecutive equals signs}%
\UnicodeMathSymbol{"02A77}{\ddotseq                  }{\mathrel}{equals sign with two dots above and two dots below}%
\UnicodeMathSymbol{"02A78}{\equivDD                  }{\mathrel}{equivalent with four dots above}%
\UnicodeMathSymbol{"02A79}{\ltcir                    }{\mathrel}{less-than with circle inside}%
\UnicodeMathSymbol{"02A7A}{\gtcir                    }{\mathrel}{greater-than with circle inside}%
\UnicodeMathSymbol{"02A7B}{\ltquest                  }{\mathrel}{less-than with question mark above}%
\UnicodeMathSymbol{"02A7C}{\gtquest                  }{\mathrel}{greater-than with question mark above}%
\UnicodeMathSymbol{"02A7D}{\leqslant                 }{\mathrel}{less-than or slanted equal to}%
\UnicodeMathSymbol{"02A7E}{\geqslant                 }{\mathrel}{greater-than or slanted equal to}%
\UnicodeMathSymbol{"02A7F}{\lesdot                   }{\mathrel}{less-than or slanted equal to with dot inside}%
\UnicodeMathSymbol{"02A80}{\gesdot                   }{\mathrel}{greater-than or slanted equal to with dot inside}%
\UnicodeMathSymbol{"02A81}{\lesdoto                  }{\mathrel}{less-than or slanted equal to with dot above}%
\UnicodeMathSymbol{"02A82}{\gesdoto                  }{\mathrel}{greater-than or slanted equal to with dot above}%
\UnicodeMathSymbol{"02A83}{\lesdotor                 }{\mathrel}{less-than or slanted equal to with dot above right}%
\UnicodeMathSymbol{"02A84}{\gesdotol                 }{\mathrel}{greater-than or slanted equal to with dot above left}%
\UnicodeMathSymbol{"02A85}{\lessapprox               }{\mathrel}{less-than or approximate}%
\UnicodeMathSymbol{"02A86}{\gtrapprox                }{\mathrel}{greater-than or approximate}%
\UnicodeMathSymbol{"02A87}{\lneq                     }{\mathrel}{less-than and single-line not equal to}%
\UnicodeMathSymbol{"02A88}{\gneq                     }{\mathrel}{greater-than and single-line not equal to}%
\UnicodeMathSymbol{"02A89}{\lnapprox                 }{\mathrel}{less-than and not approximate}%
\UnicodeMathSymbol{"02A8A}{\gnapprox                 }{\mathrel}{greater-than and not approximate}%
\UnicodeMathSymbol{"02A8B}{\lesseqqgtr               }{\mathrel}{less-than above double-line equal above greater-than}%
\UnicodeMathSymbol{"02A8C}{\gtreqqless               }{\mathrel}{greater-than above double-line equal above less-than}%
\UnicodeMathSymbol{"02A8D}{\lsime                    }{\mathrel}{less-than above similar or equal}%
\UnicodeMathSymbol{"02A8E}{\gsime                    }{\mathrel}{greater-than above similar or equal}%
\UnicodeMathSymbol{"02A8F}{\lsimg                    }{\mathrel}{less-than above similar above greater-than}%
\UnicodeMathSymbol{"02A90}{\gsiml                    }{\mathrel}{greater-than above similar above less-than}%
\UnicodeMathSymbol{"02A91}{\lgE                      }{\mathrel}{less-than above greater-than above double-line equal}%
\UnicodeMathSymbol{"02A92}{\glE                      }{\mathrel}{greater-than above less-than above double-line equal}%
\UnicodeMathSymbol{"02A93}{\lesges                   }{\mathrel}{less-than above slanted equal above greater-than above slanted equal}%
\UnicodeMathSymbol{"02A94}{\gesles                   }{\mathrel}{greater-than above slanted equal above less-than above slanted equal}%
\UnicodeMathSymbol{"02A95}{\eqslantless              }{\mathrel}{slanted equal to or less-than}%
\UnicodeMathSymbol{"02A96}{\eqslantgtr               }{\mathrel}{slanted equal to or greater-than}%
\UnicodeMathSymbol{"02A97}{\elsdot                   }{\mathrel}{slanted equal to or less-than with dot inside}%
\UnicodeMathSymbol{"02A98}{\egsdot                   }{\mathrel}{slanted equal to or greater-than with dot inside}%
\UnicodeMathSymbol{"02A99}{\eqqless                  }{\mathrel}{double-line equal to or less-than}%
\UnicodeMathSymbol{"02A9A}{\eqqgtr                   }{\mathrel}{double-line equal to or greater-than}%
\UnicodeMathSymbol{"02A9B}{\eqqslantless             }{\mathrel}{double-line slanted equal to or less-than}%
\UnicodeMathSymbol{"02A9C}{\eqqslantgtr              }{\mathrel}{double-line slanted equal to or greater-than}%
\UnicodeMathSymbol{"02A9D}{\simless                  }{\mathrel}{similar or less-than}%
\UnicodeMathSymbol{"02A9E}{\simgtr                   }{\mathrel}{similar or greater-than}%
\UnicodeMathSymbol{"02A9F}{\simlE                    }{\mathrel}{similar above less-than above equals sign}%
\UnicodeMathSymbol{"02AA0}{\simgE                    }{\mathrel}{similar above greater-than above equals sign}%
\UnicodeMathSymbol{"02AA1}{\Lt                       }{\mathrel}{double nested less-than}%
\UnicodeMathSymbol{"02AA2}{\Gt                       }{\mathrel}{double nested greater-than}%
\UnicodeMathSymbol{"02AA3}{\partialmeetcontraction   }{\mathrel}{double less-than with underbar}%
\UnicodeMathSymbol{"02AA4}{\glj                      }{\mathrel}{greater-than overlapping less-than}%
\UnicodeMathSymbol{"02AA5}{\gla                      }{\mathrel}{greater-than beside less-than}%
\UnicodeMathSymbol{"02AA6}{\ltcc                     }{\mathrel}{less-than closed by curve}%
\UnicodeMathSymbol{"02AA7}{\gtcc                     }{\mathrel}{greater-than closed by curve}%
\UnicodeMathSymbol{"02AA8}{\lescc                    }{\mathrel}{less-than closed by curve above slanted equal}%
\UnicodeMathSymbol{"02AA9}{\gescc                    }{\mathrel}{greater-than closed by curve above slanted equal}%
\UnicodeMathSymbol{"02AAA}{\smt                      }{\mathrel}{smaller than}%
\UnicodeMathSymbol{"02AAB}{\lat                      }{\mathrel}{larger than}%
\UnicodeMathSymbol{"02AAC}{\smte                     }{\mathrel}{smaller than or equal to}%
\UnicodeMathSymbol{"02AAD}{\late                     }{\mathrel}{larger than or equal to}%
\UnicodeMathSymbol{"02AAE}{\bumpeqq                  }{\mathrel}{equals sign with bumpy above}%
\UnicodeMathSymbol{"02AAF}{\preceq                   }{\mathrel}{precedes above single-line equals sign}%
\UnicodeMathSymbol{"02AB0}{\succeq                   }{\mathrel}{succeeds above single-line equals sign}%
\UnicodeMathSymbol{"02AB1}{\precneq                  }{\mathrel}{precedes above single-line not equal to}%
\UnicodeMathSymbol{"02AB2}{\succneq                  }{\mathrel}{succeeds above single-line not equal to}%
\UnicodeMathSymbol{"02AB3}{\preceqq                  }{\mathrel}{precedes above equals sign}%
\UnicodeMathSymbol{"02AB4}{\succeqq                  }{\mathrel}{succeeds above equals sign}%
\UnicodeMathSymbol{"02AB5}{\precneqq                 }{\mathrel}{precedes above not equal to}%
\UnicodeMathSymbol{"02AB6}{\succneqq                 }{\mathrel}{succeeds above not equal to}%
\UnicodeMathSymbol{"02AB7}{\precapprox               }{\mathrel}{precedes above almost equal to}%
\UnicodeMathSymbol{"02AB8}{\succapprox               }{\mathrel}{succeeds above almost equal to}%
\UnicodeMathSymbol{"02AB9}{\precnapprox              }{\mathrel}{precedes above not almost equal to}%
\UnicodeMathSymbol{"02ABA}{\succnapprox              }{\mathrel}{succeeds above not almost equal to}%
\UnicodeMathSymbol{"02ABB}{\Prec                     }{\mathrel}{double precedes}%
\UnicodeMathSymbol{"02ABC}{\Succ                     }{\mathrel}{double succeeds}%
\UnicodeMathSymbol{"02ABD}{\subsetdot                }{\mathrel}{subset with dot}%
\UnicodeMathSymbol{"02ABE}{\supsetdot                }{\mathrel}{superset with dot}%
\UnicodeMathSymbol{"02ABF}{\subsetplus               }{\mathrel}{subset with plus sign below}%
\UnicodeMathSymbol{"02AC0}{\supsetplus               }{\mathrel}{superset with plus sign below}%
\UnicodeMathSymbol{"02AC1}{\submult                  }{\mathrel}{subset with multiplication sign below}%
\UnicodeMathSymbol{"02AC2}{\supmult                  }{\mathrel}{superset with multiplication sign below}%
\UnicodeMathSymbol{"02AC3}{\subedot                  }{\mathrel}{subset of or equal to with dot above}%
\UnicodeMathSymbol{"02AC4}{\supedot                  }{\mathrel}{superset of or equal to with dot above}%
\UnicodeMathSymbol{"02AC5}{\subseteqq                }{\mathrel}{subset of above equals sign}%
\UnicodeMathSymbol{"02AC6}{\supseteqq                }{\mathrel}{superset of above equals sign}%
\UnicodeMathSymbol{"02AC7}{\subsim                   }{\mathrel}{subset of above tilde operator}%
\UnicodeMathSymbol{"02AC8}{\supsim                   }{\mathrel}{superset of above tilde operator}%
\UnicodeMathSymbol{"02AC9}{\subsetapprox             }{\mathrel}{subset of above almost equal to}%
\UnicodeMathSymbol{"02ACA}{\supsetapprox             }{\mathrel}{superset of above almost equal to}%
\UnicodeMathSymbol{"02ACB}{\subsetneqq               }{\mathrel}{subset of above not equal to}%
\UnicodeMathSymbol{"02ACC}{\supsetneqq               }{\mathrel}{superset of above not equal to}%
\UnicodeMathSymbol{"02ACD}{\lsqhook                  }{\mathrel}{square left open box operator}%
\UnicodeMathSymbol{"02ACE}{\rsqhook                  }{\mathrel}{square right open box operator}%
\UnicodeMathSymbol{"02ACF}{\csub                     }{\mathrel}{closed subset}%
\UnicodeMathSymbol{"02AD0}{\csup                     }{\mathrel}{closed superset}%
\UnicodeMathSymbol{"02AD1}{\csube                    }{\mathrel}{closed subset or equal to}%
\UnicodeMathSymbol{"02AD2}{\csupe                    }{\mathrel}{closed superset or equal to}%
\UnicodeMathSymbol{"02AD3}{\subsup                   }{\mathrel}{subset above superset}%
\UnicodeMathSymbol{"02AD4}{\supsub                   }{\mathrel}{superset above subset}%
\UnicodeMathSymbol{"02AD5}{\subsub                   }{\mathrel}{subset above subset}%
\UnicodeMathSymbol{"02AD6}{\supsup                   }{\mathrel}{superset above superset}%
\UnicodeMathSymbol{"02AD7}{\suphsub                  }{\mathrel}{superset beside subset}%
\UnicodeMathSymbol{"02AD8}{\supdsub                  }{\mathrel}{superset beside and joined by dash with subset}%
\UnicodeMathSymbol{"02AD9}{\forkv                    }{\mathrel}{element of opening downwards}%
\UnicodeMathSymbol{"02ADA}{\topfork                  }{\mathrel}{pitchfork with tee top}%
\UnicodeMathSymbol{"02ADB}{\mlcp                     }{\mathrel}{transversal intersection}%
\UnicodeMathSymbol{"02ADC}{\forks                    }{\mathrel}{forking}%
\UnicodeMathSymbol{"02ADD}{\forksnot                 }{\mathrel}{nonforking}%
\UnicodeMathSymbol{"02ADE}{\shortlefttack            }{\mathrel}{short left tack}%
\UnicodeMathSymbol{"02ADF}{\shortdowntack            }{\mathrel}{short down tack}%
\UnicodeMathSymbol{"02AE0}{\shortuptack              }{\mathrel}{short up tack}%
\UnicodeMathSymbol{"02AE1}{\perps                    }{\mathord}{perpendicular with s}%
\UnicodeMathSymbol{"02AE2}{\vDdash                   }{\mathrel}{vertical bar triple right turnstile}%
\UnicodeMathSymbol{"02AE3}{\dashV                    }{\mathrel}{double vertical bar left turnstile}%
\UnicodeMathSymbol{"02AE4}{\Dashv                    }{\mathrel}{vertical bar double left turnstile}%
\UnicodeMathSymbol{"02AE5}{\DashV                    }{\mathrel}{double vertical bar double left turnstile}%
\UnicodeMathSymbol{"02AE6}{\varVdash                 }{\mathrel}{long dash from left member of double vertical}%
\UnicodeMathSymbol{"02AE7}{\Barv                     }{\mathrel}{short down tack with overbar}%
\UnicodeMathSymbol{"02AE8}{\vBar                     }{\mathrel}{short up tack with underbar}%
\UnicodeMathSymbol{"02AE9}{\vBarv                    }{\mathrel}{short up tack above short down tack}%
\UnicodeMathSymbol{"02AEA}{\barV                     }{\mathrel}{double down tack}%
\UnicodeMathSymbol{"02AEB}{\Vbar                     }{\mathrel}{double up tack}%
\UnicodeMathSymbol{"02AEC}{\Not                      }{\mathrel}{double stroke not sign}%
\UnicodeMathSymbol{"02AED}{\bNot                     }{\mathrel}{reversed double stroke not sign}%
\UnicodeMathSymbol{"02AEE}{\revnmid                  }{\mathrel}{does not divide with reversed negation slash}%
\UnicodeMathSymbol{"02AEF}{\cirmid                   }{\mathrel}{vertical line with circle above}%
\UnicodeMathSymbol{"02AF0}{\midcir                   }{\mathrel}{vertical line with circle below}%
\UnicodeMathSymbol{"02AF1}{\topcir                   }{\mathord}{down tack with circle below}%
\UnicodeMathSymbol{"02AF2}{\nhpar                    }{\mathrel}{parallel with horizontal stroke}%
\UnicodeMathSymbol{"02AF3}{\parsim                   }{\mathrel}{parallel with tilde operator}%
\UnicodeMathSymbol{"02AF4}{\interleave               }{\mathbin}{triple vertical bar binary relation}%
\UnicodeMathSymbol{"02AF5}{\nhVvert                  }{\mathbin}{triple vertical bar with horizontal stroke}%
\UnicodeMathSymbol{"02AF6}{\threedotcolon            }{\mathbin}{triple colon operator}%
\UnicodeMathSymbol{"02AF7}{\lllnest                  }{\mathrel}{stacked very much less-than}%
\UnicodeMathSymbol{"02AF8}{\gggnest                  }{\mathrel}{stacked very much greater-than}%
\UnicodeMathSymbol{"02AF9}{\leqqslant                }{\mathrel}{double-line slanted less-than or equal to}%
\UnicodeMathSymbol{"02AFA}{\geqqslant                }{\mathrel}{double-line slanted greater-than or equal to}%
\UnicodeMathSymbol{"02AFB}{\trslash                  }{\mathbin}{triple solidus binary relation}%
\UnicodeMathSymbol{"02AFC}{\biginterleave            }{\mathop}{large triple vertical bar operator}%
\UnicodeMathSymbol{"02AFD}{\sslash                   }{\mathbin}{double solidus operator}%
\UnicodeMathSymbol{"02AFE}{\talloblong               }{\mathbin}{white vertical bar}%
\UnicodeMathSymbol{"02AFF}{\bigtalloblong            }{\mathop}{n-ary white vertical bar}%
\UnicodeMathSymbol{"02B12}{\squaretopblack           }{\mathord}{square with top half black}%
\UnicodeMathSymbol{"02B13}{\squarebotblack           }{\mathord}{square with bottom half black}%
\UnicodeMathSymbol{"02B14}{\squareurblack            }{\mathord}{square with upper right diagonal half black}%
\UnicodeMathSymbol{"02B15}{\squarellblack            }{\mathord}{square with lower left diagonal half black}%
\UnicodeMathSymbol{"02B16}{\diamondleftblack         }{\mathord}{diamond with left half black}%
\UnicodeMathSymbol{"02B17}{\diamondrightblack        }{\mathord}{diamond with right half black}%
\UnicodeMathSymbol{"02B18}{\diamondtopblack          }{\mathord}{diamond with top half black}%
\UnicodeMathSymbol{"02B19}{\diamondbotblack          }{\mathord}{diamond with bottom half black}%
\UnicodeMathSymbol{"02B1A}{\dottedsquare             }{\mathord}{dotted square}%
\UnicodeMathSymbol{"02B1B}{\lgblksquare              }{\mathord}{black large square}%
\UnicodeMathSymbol{"02B1C}{\lgwhtsquare              }{\mathord}{white large square}%
\UnicodeMathSymbol{"02B1D}{\vysmblksquare            }{\mathord}{black very small square}%
\UnicodeMathSymbol{"02B1E}{\vysmwhtsquare            }{\mathord}{white very small square}%
\UnicodeMathSymbol{"02B1F}{\pentagonblack            }{\mathord}{black pentagon}%
\UnicodeMathSymbol{"02B20}{\pentagon                 }{\mathord}{white pentagon}%
\UnicodeMathSymbol{"02B21}{\varhexagon               }{\mathord}{white hexagon}%
\UnicodeMathSymbol{"02B22}{\varhexagonblack          }{\mathord}{black hexagon}%
\UnicodeMathSymbol{"02B23}{\hexagonblack             }{\mathord}{horizontal black hexagon}%
\UnicodeMathSymbol{"02B24}{\lgblkcircle              }{\mathord}{black large circle}%
\UnicodeMathSymbol{"02B25}{\mdblkdiamond             }{\mathord}{black medium diamond}%
\UnicodeMathSymbol{"02B26}{\mdwhtdiamond             }{\mathord}{white medium diamond}%
\UnicodeMathSymbol{"02B27}{\mdblklozenge             }{\mathord}{black medium lozenge}%
\UnicodeMathSymbol{"02B28}{\mdwhtlozenge             }{\mathord}{white medium lozenge}%
\UnicodeMathSymbol{"02B29}{\smblkdiamond             }{\mathord}{black small diamond}%
\UnicodeMathSymbol{"02B2A}{\smblklozenge             }{\mathord}{black small lozenge}%
\UnicodeMathSymbol{"02B2B}{\smwhtlozenge             }{\mathord}{white small lozenge}%
\UnicodeMathSymbol{"02B2C}{\blkhorzoval              }{\mathord}{black horizontal ellipse}%
\UnicodeMathSymbol{"02B2D}{\whthorzoval              }{\mathord}{white horizontal ellipse}%
\UnicodeMathSymbol{"02B2E}{\blkvertoval              }{\mathord}{black vertical ellipse}%
\UnicodeMathSymbol{"02B2F}{\whtvertoval              }{\mathord}{white vertical ellipse}%
\UnicodeMathSymbol{"02B30}{\circleonleftarrow        }{\mathrel}{left arrow with small circle}%
\UnicodeMathSymbol{"02B31}{\leftthreearrows          }{\mathrel}{three leftwards arrows}%
\UnicodeMathSymbol{"02B32}{\leftarrowonoplus         }{\mathrel}{left arrow with circled plus}%
\UnicodeMathSymbol{"02B33}{\longleftsquigarrow       }{\mathrel}{long leftwards squiggle arrow}%
\UnicodeMathSymbol{"02B34}{\nvtwoheadleftarrow       }{\mathrel}{leftwards two-headed arrow with vertical stroke}%
\UnicodeMathSymbol{"02B35}{\nVtwoheadleftarrow       }{\mathrel}{leftwards two-headed arrow with double vertical stroke}%
\UnicodeMathSymbol{"02B36}{\twoheadmapsfrom          }{\mathrel}{leftwards two-headed arrow from bar}%
\UnicodeMathSymbol{"02B37}{\twoheadleftdbkarrow      }{\mathrel}{leftwards two-headed triple-dash arrow}%
\UnicodeMathSymbol{"02B38}{\leftdotarrow             }{\mathrel}{leftwards arrow with dotted stem}%
\UnicodeMathSymbol{"02B39}{\nvleftarrowtail          }{\mathrel}{leftwards arrow with tail with vertical stroke}%
\UnicodeMathSymbol{"02B3A}{\nVleftarrowtail          }{\mathrel}{leftwards arrow with tail with double vertical stroke}%
\UnicodeMathSymbol{"02B3B}{\twoheadleftarrowtail     }{\mathrel}{leftwards two-headed arrow with tail}%
\UnicodeMathSymbol{"02B3C}{\nvtwoheadleftarrowtail   }{\mathrel}{leftwards two-headed arrow with tail with vertical stroke}%
\UnicodeMathSymbol{"02B3D}{\nVtwoheadleftarrowtail   }{\mathrel}{leftwards two-headed arrow with tail with double vertical stroke}%
\UnicodeMathSymbol{"02B3E}{\leftarrowx               }{\mathrel}{leftwards arrow through x}%
\UnicodeMathSymbol{"02B3F}{\leftcurvedarrow          }{\mathrel}{wave arrow pointing directly left}%
\UnicodeMathSymbol{"02B40}{\equalleftarrow           }{\mathrel}{equals sign above leftwards arrow}%
\UnicodeMathSymbol{"02B41}{\bsimilarleftarrow        }{\mathrel}{reverse tilde operator above leftwards arrow}%
\UnicodeMathSymbol{"02B42}{\leftarrowbackapprox      }{\mathrel}{leftwards arrow above reverse almost equal to}%
\UnicodeMathSymbol{"02B43}{\rightarrowgtr            }{\mathrel}{rightwards arrow through greater-than}%
\UnicodeMathSymbol{"02B44}{\rightarrowsupset         }{\mathrel}{rightwards arrow through subset}%
\UnicodeMathSymbol{"02B45}{\LLeftarrow               }{\mathrel}{leftwards quadruple arrow}%
\UnicodeMathSymbol{"02B46}{\RRightarrow              }{\mathrel}{rightwards quadruple arrow}%
\UnicodeMathSymbol{"02B47}{\bsimilarrightarrow       }{\mathrel}{reverse tilde operator above rightwards arrow}%
\UnicodeMathSymbol{"02B48}{\rightarrowbackapprox     }{\mathrel}{rightwards arrow above reverse almost equal to}%
\UnicodeMathSymbol{"02B49}{\similarleftarrow         }{\mathrel}{tilde operator above leftwards arrow}%
\UnicodeMathSymbol{"02B4A}{\leftarrowapprox          }{\mathrel}{leftwards arrow above almost equal to}%
\UnicodeMathSymbol{"02B4B}{\leftarrowbsimilar        }{\mathrel}{leftwards arrow above reverse tilde operator}%
\UnicodeMathSymbol{"02B4C}{\rightarrowbsimilar       }{\mathrel}{righttwards arrow above reverse tilde operator}%
\UnicodeMathSymbol{"02B50}{\medwhitestar             }{\mathord}{white medium star}%
\UnicodeMathSymbol{"02B51}{\medblackstar             }{\mathord}{black medium star}%
\UnicodeMathSymbol{"02B52}{\smwhitestar              }{\mathord}{white small star}%
\UnicodeMathSymbol{"02B53}{\rightpentagonblack       }{\mathord}{black right-pointing pentagon}%
\UnicodeMathSymbol{"02B54}{\rightpentagon            }{\mathord}{white right-pointing pentagon}%
\UnicodeMathSymbol{"03012}{\postalmark               }{\mathord}{postal mark}%
\UnicodeMathSymbol{"03030}{\hzigzag                  }{\mathord}{zigzag}%
\UnicodeMathSymbol{"1D400}{\mbfA                     }{\mathalpha}{mathematical bold capital a}%
\UnicodeMathSymbol{"1D401}{\mbfB                     }{\mathalpha}{mathematical bold capital b}%
\UnicodeMathSymbol{"1D402}{\mbfC                     }{\mathalpha}{mathematical bold capital c}%
\UnicodeMathSymbol{"1D403}{\mbfD                     }{\mathalpha}{mathematical bold capital d}%
\UnicodeMathSymbol{"1D404}{\mbfE                     }{\mathalpha}{mathematical bold capital e}%
\UnicodeMathSymbol{"1D405}{\mbfF                     }{\mathalpha}{mathematical bold capital f}%
\UnicodeMathSymbol{"1D406}{\mbfG                     }{\mathalpha}{mathematical bold capital g}%
\UnicodeMathSymbol{"1D407}{\mbfH                     }{\mathalpha}{mathematical bold capital h}%
\UnicodeMathSymbol{"1D408}{\mbfI                     }{\mathalpha}{mathematical bold capital i}%
\UnicodeMathSymbol{"1D409}{\mbfJ                     }{\mathalpha}{mathematical bold capital j}%
\UnicodeMathSymbol{"1D40A}{\mbfK                     }{\mathalpha}{mathematical bold capital k}%
\UnicodeMathSymbol{"1D40B}{\mbfL                     }{\mathalpha}{mathematical bold capital l}%
\UnicodeMathSymbol{"1D40C}{\mbfM                     }{\mathalpha}{mathematical bold capital m}%
\UnicodeMathSymbol{"1D40D}{\mbfN                     }{\mathalpha}{mathematical bold capital n}%
\UnicodeMathSymbol{"1D40E}{\mbfO                     }{\mathalpha}{mathematical bold capital o}%
\UnicodeMathSymbol{"1D40F}{\mbfP                     }{\mathalpha}{mathematical bold capital p}%
\UnicodeMathSymbol{"1D410}{\mbfQ                     }{\mathalpha}{mathematical bold capital q}%
\UnicodeMathSymbol{"1D411}{\mbfR                     }{\mathalpha}{mathematical bold capital r}%
\UnicodeMathSymbol{"1D412}{\mbfS                     }{\mathalpha}{mathematical bold capital s}%
\UnicodeMathSymbol{"1D413}{\mbfT                     }{\mathalpha}{mathematical bold capital t}%
\UnicodeMathSymbol{"1D414}{\mbfU                     }{\mathalpha}{mathematical bold capital u}%
\UnicodeMathSymbol{"1D415}{\mbfV                     }{\mathalpha}{mathematical bold capital v}%
\UnicodeMathSymbol{"1D416}{\mbfW                     }{\mathalpha}{mathematical bold capital w}%
\UnicodeMathSymbol{"1D417}{\mbfX                     }{\mathalpha}{mathematical bold capital x}%
\UnicodeMathSymbol{"1D418}{\mbfY                     }{\mathalpha}{mathematical bold capital y}%
\UnicodeMathSymbol{"1D419}{\mbfZ                     }{\mathalpha}{mathematical bold capital z}%
\UnicodeMathSymbol{"1D41A}{\mbfa                     }{\mathalpha}{mathematical bold small a}%
\UnicodeMathSymbol{"1D41B}{\mbfb                     }{\mathalpha}{mathematical bold small b}%
\UnicodeMathSymbol{"1D41C}{\mbfc                     }{\mathalpha}{mathematical bold small c}%
\UnicodeMathSymbol{"1D41D}{\mbfd                     }{\mathalpha}{mathematical bold small d}%
\UnicodeMathSymbol{"1D41E}{\mbfe                     }{\mathalpha}{mathematical bold small e}%
\UnicodeMathSymbol{"1D41F}{\mbff                     }{\mathalpha}{mathematical bold small f}%
\UnicodeMathSymbol{"1D420}{\mbfg                     }{\mathalpha}{mathematical bold small g}%
\UnicodeMathSymbol{"1D421}{\mbfh                     }{\mathalpha}{mathematical bold small h}%
\UnicodeMathSymbol{"1D422}{\mbfi                     }{\mathalpha}{mathematical bold small i}%
\UnicodeMathSymbol{"1D423}{\mbfj                     }{\mathalpha}{mathematical bold small j}%
\UnicodeMathSymbol{"1D424}{\mbfk                     }{\mathalpha}{mathematical bold small k}%
\UnicodeMathSymbol{"1D425}{\mbfl                     }{\mathalpha}{mathematical bold small l}%
\UnicodeMathSymbol{"1D426}{\mbfm                     }{\mathalpha}{mathematical bold small m}%
\UnicodeMathSymbol{"1D427}{\mbfn                     }{\mathalpha}{mathematical bold small n}%
\UnicodeMathSymbol{"1D428}{\mbfo                     }{\mathalpha}{mathematical bold small o}%
\UnicodeMathSymbol{"1D429}{\mbfp                     }{\mathalpha}{mathematical bold small p}%
\UnicodeMathSymbol{"1D42A}{\mbfq                     }{\mathalpha}{mathematical bold small q}%
\UnicodeMathSymbol{"1D42B}{\mbfr                     }{\mathalpha}{mathematical bold small r}%
\UnicodeMathSymbol{"1D42C}{\mbfs                     }{\mathalpha}{mathematical bold small s}%
\UnicodeMathSymbol{"1D42D}{\mbft                     }{\mathalpha}{mathematical bold small t}%
\UnicodeMathSymbol{"1D42E}{\mbfu                     }{\mathalpha}{mathematical bold small u}%
\UnicodeMathSymbol{"1D42F}{\mbfv                     }{\mathalpha}{mathematical bold small v}%
\UnicodeMathSymbol{"1D430}{\mbfw                     }{\mathalpha}{mathematical bold small w}%
\UnicodeMathSymbol{"1D431}{\mbfx                     }{\mathalpha}{mathematical bold small x}%
\UnicodeMathSymbol{"1D432}{\mbfy                     }{\mathalpha}{mathematical bold small y}%
\UnicodeMathSymbol{"1D433}{\mbfz                     }{\mathalpha}{mathematical bold small z}%
\UnicodeMathSymbol{"1D434}{\mitA                     }{\mathalpha}{mathematical italic capital a}%
\UnicodeMathSymbol{"1D435}{\mitB                     }{\mathalpha}{mathematical italic capital b}%
\UnicodeMathSymbol{"1D436}{\mitC                     }{\mathalpha}{mathematical italic capital c}%
\UnicodeMathSymbol{"1D437}{\mitD                     }{\mathalpha}{mathematical italic capital d}%
\UnicodeMathSymbol{"1D438}{\mitE                     }{\mathalpha}{mathematical italic capital e}%
\UnicodeMathSymbol{"1D439}{\mitF                     }{\mathalpha}{mathematical italic capital f}%
\UnicodeMathSymbol{"1D43A}{\mitG                     }{\mathalpha}{mathematical italic capital g}%
\UnicodeMathSymbol{"1D43B}{\mitH                     }{\mathalpha}{mathematical italic capital h}%
\UnicodeMathSymbol{"1D43C}{\mitI                     }{\mathalpha}{mathematical italic capital i}%
\UnicodeMathSymbol{"1D43D}{\mitJ                     }{\mathalpha}{mathematical italic capital j}%
\UnicodeMathSymbol{"1D43E}{\mitK                     }{\mathalpha}{mathematical italic capital k}%
\UnicodeMathSymbol{"1D43F}{\mitL                     }{\mathalpha}{mathematical italic capital l}%
\UnicodeMathSymbol{"1D440}{\mitM                     }{\mathalpha}{mathematical italic capital m}%
\UnicodeMathSymbol{"1D441}{\mitN                     }{\mathalpha}{mathematical italic capital n}%
\UnicodeMathSymbol{"1D442}{\mitO                     }{\mathalpha}{mathematical italic capital o}%
\UnicodeMathSymbol{"1D443}{\mitP                     }{\mathalpha}{mathematical italic capital p}%
\UnicodeMathSymbol{"1D444}{\mitQ                     }{\mathalpha}{mathematical italic capital q}%
\UnicodeMathSymbol{"1D445}{\mitR                     }{\mathalpha}{mathematical italic capital r}%
\UnicodeMathSymbol{"1D446}{\mitS                     }{\mathalpha}{mathematical italic capital s}%
\UnicodeMathSymbol{"1D447}{\mitT                     }{\mathalpha}{mathematical italic capital t}%
\UnicodeMathSymbol{"1D448}{\mitU                     }{\mathalpha}{mathematical italic capital u}%
\UnicodeMathSymbol{"1D449}{\mitV                     }{\mathalpha}{mathematical italic capital v}%
\UnicodeMathSymbol{"1D44A}{\mitW                     }{\mathalpha}{mathematical italic capital w}%
\UnicodeMathSymbol{"1D44B}{\mitX                     }{\mathalpha}{mathematical italic capital x}%
\UnicodeMathSymbol{"1D44C}{\mitY                     }{\mathalpha}{mathematical italic capital y}%
\UnicodeMathSymbol{"1D44D}{\mitZ                     }{\mathalpha}{mathematical italic capital z}%
\UnicodeMathSymbol{"1D44E}{\mita                     }{\mathalpha}{mathematical italic small a}%
\UnicodeMathSymbol{"1D44F}{\mitb                     }{\mathalpha}{mathematical italic small b}%
\UnicodeMathSymbol{"1D450}{\mitc                     }{\mathalpha}{mathematical italic small c}%
\UnicodeMathSymbol{"1D451}{\mitd                     }{\mathalpha}{mathematical italic small d}%
\UnicodeMathSymbol{"1D452}{\mite                     }{\mathalpha}{mathematical italic small e}%
\UnicodeMathSymbol{"1D453}{\mitf                     }{\mathalpha}{mathematical italic small f}%
\UnicodeMathSymbol{"1D454}{\mitg                     }{\mathalpha}{mathematical italic small g}%
\UnicodeMathSymbol{"1D456}{\miti                     }{\mathalpha}{mathematical italic small i}%
\UnicodeMathSymbol{"1D457}{\mitj                     }{\mathalpha}{mathematical italic small j}%
\UnicodeMathSymbol{"1D458}{\mitk                     }{\mathalpha}{mathematical italic small k}%
\UnicodeMathSymbol{"1D459}{\mitl                     }{\mathalpha}{mathematical italic small l}%
\UnicodeMathSymbol{"1D45A}{\mitm                     }{\mathalpha}{mathematical italic small m}%
\UnicodeMathSymbol{"1D45B}{\mitn                     }{\mathalpha}{mathematical italic small n}%
\UnicodeMathSymbol{"1D45C}{\mito                     }{\mathalpha}{mathematical italic small o}%
\UnicodeMathSymbol{"1D45D}{\mitp                     }{\mathalpha}{mathematical italic small p}%
\UnicodeMathSymbol{"1D45E}{\mitq                     }{\mathalpha}{mathematical italic small q}%
\UnicodeMathSymbol{"1D45F}{\mitr                     }{\mathalpha}{mathematical italic small r}%
\UnicodeMathSymbol{"1D460}{\mits                     }{\mathalpha}{mathematical italic small s}%
\UnicodeMathSymbol{"1D461}{\mitt                     }{\mathalpha}{mathematical italic small t}%
\UnicodeMathSymbol{"1D462}{\mitu                     }{\mathalpha}{mathematical italic small u}%
\UnicodeMathSymbol{"1D463}{\mitv                     }{\mathalpha}{mathematical italic small v}%
\UnicodeMathSymbol{"1D464}{\mitw                     }{\mathalpha}{mathematical italic small w}%
\UnicodeMathSymbol{"1D465}{\mitx                     }{\mathalpha}{mathematical italic small x}%
\UnicodeMathSymbol{"1D466}{\mity                     }{\mathalpha}{mathematical italic small y}%
\UnicodeMathSymbol{"1D467}{\mitz                     }{\mathalpha}{mathematical italic small z}%
\UnicodeMathSymbol{"1D468}{\mbfitA                   }{\mathalpha}{mathematical bold italic capital a}%
\UnicodeMathSymbol{"1D469}{\mbfitB                   }{\mathalpha}{mathematical bold italic capital b}%
\UnicodeMathSymbol{"1D46A}{\mbfitC                   }{\mathalpha}{mathematical bold italic capital c}%
\UnicodeMathSymbol{"1D46B}{\mbfitD                   }{\mathalpha}{mathematical bold italic capital d}%
\UnicodeMathSymbol{"1D46C}{\mbfitE                   }{\mathalpha}{mathematical bold italic capital e}%
\UnicodeMathSymbol{"1D46D}{\mbfitF                   }{\mathalpha}{mathematical bold italic capital f}%
\UnicodeMathSymbol{"1D46E}{\mbfitG                   }{\mathalpha}{mathematical bold italic capital g}%
\UnicodeMathSymbol{"1D46F}{\mbfitH                   }{\mathalpha}{mathematical bold italic capital h}%
\UnicodeMathSymbol{"1D470}{\mbfitI                   }{\mathalpha}{mathematical bold italic capital i}%
\UnicodeMathSymbol{"1D471}{\mbfitJ                   }{\mathalpha}{mathematical bold italic capital j}%
\UnicodeMathSymbol{"1D472}{\mbfitK                   }{\mathalpha}{mathematical bold italic capital k}%
\UnicodeMathSymbol{"1D473}{\mbfitL                   }{\mathalpha}{mathematical bold italic capital l}%
\UnicodeMathSymbol{"1D474}{\mbfitM                   }{\mathalpha}{mathematical bold italic capital m}%
\UnicodeMathSymbol{"1D475}{\mbfitN                   }{\mathalpha}{mathematical bold italic capital n}%
\UnicodeMathSymbol{"1D476}{\mbfitO                   }{\mathalpha}{mathematical bold italic capital o}%
\UnicodeMathSymbol{"1D477}{\mbfitP                   }{\mathalpha}{mathematical bold italic capital p}%
\UnicodeMathSymbol{"1D478}{\mbfitQ                   }{\mathalpha}{mathematical bold italic capital q}%
\UnicodeMathSymbol{"1D479}{\mbfitR                   }{\mathalpha}{mathematical bold italic capital r}%
\UnicodeMathSymbol{"1D47A}{\mbfitS                   }{\mathalpha}{mathematical bold italic capital s}%
\UnicodeMathSymbol{"1D47B}{\mbfitT                   }{\mathalpha}{mathematical bold italic capital t}%
\UnicodeMathSymbol{"1D47C}{\mbfitU                   }{\mathalpha}{mathematical bold italic capital u}%
\UnicodeMathSymbol{"1D47D}{\mbfitV                   }{\mathalpha}{mathematical bold italic capital v}%
\UnicodeMathSymbol{"1D47E}{\mbfitW                   }{\mathalpha}{mathematical bold italic capital w}%
\UnicodeMathSymbol{"1D47F}{\mbfitX                   }{\mathalpha}{mathematical bold italic capital x}%
\UnicodeMathSymbol{"1D480}{\mbfitY                   }{\mathalpha}{mathematical bold italic capital y}%
\UnicodeMathSymbol{"1D481}{\mbfitZ                   }{\mathalpha}{mathematical bold italic capital z}%
\UnicodeMathSymbol{"1D482}{\mbfita                   }{\mathalpha}{mathematical bold italic small a}%
\UnicodeMathSymbol{"1D483}{\mbfitb                   }{\mathalpha}{mathematical bold italic small b}%
\UnicodeMathSymbol{"1D484}{\mbfitc                   }{\mathalpha}{mathematical bold italic small c}%
\UnicodeMathSymbol{"1D485}{\mbfitd                   }{\mathalpha}{mathematical bold italic small d}%
\UnicodeMathSymbol{"1D486}{\mbfite                   }{\mathalpha}{mathematical bold italic small e}%
\UnicodeMathSymbol{"1D487}{\mbfitf                   }{\mathalpha}{mathematical bold italic small f}%
\UnicodeMathSymbol{"1D488}{\mbfitg                   }{\mathalpha}{mathematical bold italic small g}%
\UnicodeMathSymbol{"1D489}{\mbfith                   }{\mathalpha}{mathematical bold italic small h}%
\UnicodeMathSymbol{"1D48A}{\mbfiti                   }{\mathalpha}{mathematical bold italic small i}%
\UnicodeMathSymbol{"1D48B}{\mbfitj                   }{\mathalpha}{mathematical bold italic small j}%
\UnicodeMathSymbol{"1D48C}{\mbfitk                   }{\mathalpha}{mathematical bold italic small k}%
\UnicodeMathSymbol{"1D48D}{\mbfitl                   }{\mathalpha}{mathematical bold italic small l}%
\UnicodeMathSymbol{"1D48E}{\mbfitm                   }{\mathalpha}{mathematical bold italic small m}%
\UnicodeMathSymbol{"1D48F}{\mbfitn                   }{\mathalpha}{mathematical bold italic small n}%
\UnicodeMathSymbol{"1D490}{\mbfito                   }{\mathalpha}{mathematical bold italic small o}%
\UnicodeMathSymbol{"1D491}{\mbfitp                   }{\mathalpha}{mathematical bold italic small p}%
\UnicodeMathSymbol{"1D492}{\mbfitq                   }{\mathalpha}{mathematical bold italic small q}%
\UnicodeMathSymbol{"1D493}{\mbfitr                   }{\mathalpha}{mathematical bold italic small r}%
\UnicodeMathSymbol{"1D494}{\mbfits                   }{\mathalpha}{mathematical bold italic small s}%
\UnicodeMathSymbol{"1D495}{\mbfitt                   }{\mathalpha}{mathematical bold italic small t}%
\UnicodeMathSymbol{"1D496}{\mbfitu                   }{\mathalpha}{mathematical bold italic small u}%
\UnicodeMathSymbol{"1D497}{\mbfitv                   }{\mathalpha}{mathematical bold italic small v}%
\UnicodeMathSymbol{"1D498}{\mbfitw                   }{\mathalpha}{mathematical bold italic small w}%
\UnicodeMathSymbol{"1D499}{\mbfitx                   }{\mathalpha}{mathematical bold italic small x}%
\UnicodeMathSymbol{"1D49A}{\mbfity                   }{\mathalpha}{mathematical bold italic small y}%
\UnicodeMathSymbol{"1D49B}{\mbfitz                   }{\mathalpha}{mathematical bold italic small z}%
\UnicodeMathSymbol{"1D49C}{\mscrA                    }{\mathalpha}{mathematical script capital a}%
\UnicodeMathSymbol{"1D49E}{\mscrC                    }{\mathalpha}{mathematical script capital c}%
\UnicodeMathSymbol{"1D49F}{\mscrD                    }{\mathalpha}{mathematical script capital d}%
\UnicodeMathSymbol{"1D4A2}{\mscrG                    }{\mathalpha}{mathematical script capital g}%
\UnicodeMathSymbol{"1D4A5}{\mscrJ                    }{\mathalpha}{mathematical script capital j}%
\UnicodeMathSymbol{"1D4A6}{\mscrK                    }{\mathalpha}{mathematical script capital k}%
\UnicodeMathSymbol{"1D4A9}{\mscrN                    }{\mathalpha}{mathematical script capital n}%
\UnicodeMathSymbol{"1D4AA}{\mscrO                    }{\mathalpha}{mathematical script capital o}%
\UnicodeMathSymbol{"1D4AB}{\mscrP                    }{\mathalpha}{mathematical script capital p}%
\UnicodeMathSymbol{"1D4AC}{\mscrQ                    }{\mathalpha}{mathematical script capital q}%
\UnicodeMathSymbol{"1D4AE}{\mscrS                    }{\mathalpha}{mathematical script capital s}%
\UnicodeMathSymbol{"1D4AF}{\mscrT                    }{\mathalpha}{mathematical script capital t}%
\UnicodeMathSymbol{"1D4B0}{\mscrU                    }{\mathalpha}{mathematical script capital u}%
\UnicodeMathSymbol{"1D4B1}{\mscrV                    }{\mathalpha}{mathematical script capital v}%
\UnicodeMathSymbol{"1D4B2}{\mscrW                    }{\mathalpha}{mathematical script capital w}%
\UnicodeMathSymbol{"1D4B3}{\mscrX                    }{\mathalpha}{mathematical script capital x}%
\UnicodeMathSymbol{"1D4B4}{\mscrY                    }{\mathalpha}{mathematical script capital y}%
\UnicodeMathSymbol{"1D4B5}{\mscrZ                    }{\mathalpha}{mathematical script capital z}%
\UnicodeMathSymbol{"1D4B6}{\mscra                    }{\mathalpha}{mathematical script small a}%
\UnicodeMathSymbol{"1D4B7}{\mscrb                    }{\mathalpha}{mathematical script small b}%
\UnicodeMathSymbol{"1D4B8}{\mscrc                    }{\mathalpha}{mathematical script small c}%
\UnicodeMathSymbol{"1D4B9}{\mscrd                    }{\mathalpha}{mathematical script small d}%
\UnicodeMathSymbol{"1D4BB}{\mscrf                    }{\mathalpha}{mathematical script small f}%
\UnicodeMathSymbol{"1D4BD}{\mscrh                    }{\mathalpha}{mathematical script small h}%
\UnicodeMathSymbol{"1D4BE}{\mscri                    }{\mathalpha}{mathematical script small i}%
\UnicodeMathSymbol{"1D4BF}{\mscrj                    }{\mathalpha}{mathematical script small j}%
\UnicodeMathSymbol{"1D4C0}{\mscrk                    }{\mathalpha}{mathematical script small k}%
\UnicodeMathSymbol{"1D4C1}{\mscrl                    }{\mathalpha}{mathematical script small l}%
\UnicodeMathSymbol{"1D4C2}{\mscrm                    }{\mathalpha}{mathematical script small m}%
\UnicodeMathSymbol{"1D4C3}{\mscrn                    }{\mathalpha}{mathematical script small n}%
\UnicodeMathSymbol{"1D4C5}{\mscrp                    }{\mathalpha}{mathematical script small p}%
\UnicodeMathSymbol{"1D4C6}{\mscrq                    }{\mathalpha}{mathematical script small q}%
\UnicodeMathSymbol{"1D4C7}{\mscrr                    }{\mathalpha}{mathematical script small r}%
\UnicodeMathSymbol{"1D4C8}{\mscrs                    }{\mathalpha}{mathematical script small s}%
\UnicodeMathSymbol{"1D4C9}{\mscrt                    }{\mathalpha}{mathematical script small t}%
\UnicodeMathSymbol{"1D4CA}{\mscru                    }{\mathalpha}{mathematical script small u}%
\UnicodeMathSymbol{"1D4CB}{\mscrv                    }{\mathalpha}{mathematical script small v}%
\UnicodeMathSymbol{"1D4CC}{\mscrw                    }{\mathalpha}{mathematical script small w}%
\UnicodeMathSymbol{"1D4CD}{\mscrx                    }{\mathalpha}{mathematical script small x}%
\UnicodeMathSymbol{"1D4CE}{\mscry                    }{\mathalpha}{mathematical script small y}%
\UnicodeMathSymbol{"1D4CF}{\mscrz                    }{\mathalpha}{mathematical script small z}%
\UnicodeMathSymbol{"1D4D0}{\mbfscrA                  }{\mathalpha}{mathematical bold script capital a}%
\UnicodeMathSymbol{"1D4D1}{\mbfscrB                  }{\mathalpha}{mathematical bold script capital b}%
\UnicodeMathSymbol{"1D4D2}{\mbfscrC                  }{\mathalpha}{mathematical bold script capital c}%
\UnicodeMathSymbol{"1D4D3}{\mbfscrD                  }{\mathalpha}{mathematical bold script capital d}%
\UnicodeMathSymbol{"1D4D4}{\mbfscrE                  }{\mathalpha}{mathematical bold script capital e}%
\UnicodeMathSymbol{"1D4D5}{\mbfscrF                  }{\mathalpha}{mathematical bold script capital f}%
\UnicodeMathSymbol{"1D4D6}{\mbfscrG                  }{\mathalpha}{mathematical bold script capital g}%
\UnicodeMathSymbol{"1D4D7}{\mbfscrH                  }{\mathalpha}{mathematical bold script capital h}%
\UnicodeMathSymbol{"1D4D8}{\mbfscrI                  }{\mathalpha}{mathematical bold script capital i}%
\UnicodeMathSymbol{"1D4D9}{\mbfscrJ                  }{\mathalpha}{mathematical bold script capital j}%
\UnicodeMathSymbol{"1D4DA}{\mbfscrK                  }{\mathalpha}{mathematical bold script capital k}%
\UnicodeMathSymbol{"1D4DB}{\mbfscrL                  }{\mathalpha}{mathematical bold script capital l}%
\UnicodeMathSymbol{"1D4DC}{\mbfscrM                  }{\mathalpha}{mathematical bold script capital m}%
\UnicodeMathSymbol{"1D4DD}{\mbfscrN                  }{\mathalpha}{mathematical bold script capital n}%
\UnicodeMathSymbol{"1D4DE}{\mbfscrO                  }{\mathalpha}{mathematical bold script capital o}%
\UnicodeMathSymbol{"1D4DF}{\mbfscrP                  }{\mathalpha}{mathematical bold script capital p}%
\UnicodeMathSymbol{"1D4E0}{\mbfscrQ                  }{\mathalpha}{mathematical bold script capital q}%
\UnicodeMathSymbol{"1D4E1}{\mbfscrR                  }{\mathalpha}{mathematical bold script capital r}%
\UnicodeMathSymbol{"1D4E2}{\mbfscrS                  }{\mathalpha}{mathematical bold script capital s}%
\UnicodeMathSymbol{"1D4E3}{\mbfscrT                  }{\mathalpha}{mathematical bold script capital t}%
\UnicodeMathSymbol{"1D4E4}{\mbfscrU                  }{\mathalpha}{mathematical bold script capital u}%
\UnicodeMathSymbol{"1D4E5}{\mbfscrV                  }{\mathalpha}{mathematical bold script capital v}%
\UnicodeMathSymbol{"1D4E6}{\mbfscrW                  }{\mathalpha}{mathematical bold script capital w}%
\UnicodeMathSymbol{"1D4E7}{\mbfscrX                  }{\mathalpha}{mathematical bold script capital x}%
\UnicodeMathSymbol{"1D4E8}{\mbfscrY                  }{\mathalpha}{mathematical bold script capital y}%
\UnicodeMathSymbol{"1D4E9}{\mbfscrZ                  }{\mathalpha}{mathematical bold script capital z}%
\UnicodeMathSymbol{"1D4EA}{\mbfscra                  }{\mathalpha}{mathematical bold script small a}%
\UnicodeMathSymbol{"1D4EB}{\mbfscrb                  }{\mathalpha}{mathematical bold script small b}%
\UnicodeMathSymbol{"1D4EC}{\mbfscrc                  }{\mathalpha}{mathematical bold script small c}%
\UnicodeMathSymbol{"1D4ED}{\mbfscrd                  }{\mathalpha}{mathematical bold script small d}%
\UnicodeMathSymbol{"1D4EE}{\mbfscre                  }{\mathalpha}{mathematical bold script small e}%
\UnicodeMathSymbol{"1D4EF}{\mbfscrf                  }{\mathalpha}{mathematical bold script small f}%
\UnicodeMathSymbol{"1D4F0}{\mbfscrg                  }{\mathalpha}{mathematical bold script small g}%
\UnicodeMathSymbol{"1D4F1}{\mbfscrh                  }{\mathalpha}{mathematical bold script small h}%
\UnicodeMathSymbol{"1D4F2}{\mbfscri                  }{\mathalpha}{mathematical bold script small i}%
\UnicodeMathSymbol{"1D4F3}{\mbfscrj                  }{\mathalpha}{mathematical bold script small j}%
\UnicodeMathSymbol{"1D4F4}{\mbfscrk                  }{\mathalpha}{mathematical bold script small k}%
\UnicodeMathSymbol{"1D4F5}{\mbfscrl                  }{\mathalpha}{mathematical bold script small l}%
\UnicodeMathSymbol{"1D4F6}{\mbfscrm                  }{\mathalpha}{mathematical bold script small m}%
\UnicodeMathSymbol{"1D4F7}{\mbfscrn                  }{\mathalpha}{mathematical bold script small n}%
\UnicodeMathSymbol{"1D4F8}{\mbfscro                  }{\mathalpha}{mathematical bold script small o}%
\UnicodeMathSymbol{"1D4F9}{\mbfscrp                  }{\mathalpha}{mathematical bold script small p}%
\UnicodeMathSymbol{"1D4FA}{\mbfscrq                  }{\mathalpha}{mathematical bold script small q}%
\UnicodeMathSymbol{"1D4FB}{\mbfscrr                  }{\mathalpha}{mathematical bold script small r}%
\UnicodeMathSymbol{"1D4FC}{\mbfscrs                  }{\mathalpha}{mathematical bold script small s}%
\UnicodeMathSymbol{"1D4FD}{\mbfscrt                  }{\mathalpha}{mathematical bold script small t}%
\UnicodeMathSymbol{"1D4FE}{\mbfscru                  }{\mathalpha}{mathematical bold script small u}%
\UnicodeMathSymbol{"1D4FF}{\mbfscrv                  }{\mathalpha}{mathematical bold script small v}%
\UnicodeMathSymbol{"1D500}{\mbfscrw                  }{\mathalpha}{mathematical bold script small w}%
\UnicodeMathSymbol{"1D501}{\mbfscrx                  }{\mathalpha}{mathematical bold script small x}%
\UnicodeMathSymbol{"1D502}{\mbfscry                  }{\mathalpha}{mathematical bold script small y}%
\UnicodeMathSymbol{"1D503}{\mbfscrz                  }{\mathalpha}{mathematical bold script small z}%
\UnicodeMathSymbol{"1D504}{\mfrakA                   }{\mathalpha}{mathematical fraktur capital a}%
\UnicodeMathSymbol{"1D505}{\mfrakB                   }{\mathalpha}{mathematical fraktur capital b}%
\UnicodeMathSymbol{"1D507}{\mfrakD                   }{\mathalpha}{mathematical fraktur capital d}%
\UnicodeMathSymbol{"1D508}{\mfrakE                   }{\mathalpha}{mathematical fraktur capital e}%
\UnicodeMathSymbol{"1D509}{\mfrakF                   }{\mathalpha}{mathematical fraktur capital f}%
\UnicodeMathSymbol{"1D50A}{\mfrakG                   }{\mathalpha}{mathematical fraktur capital g}%
\UnicodeMathSymbol{"1D50D}{\mfrakJ                   }{\mathalpha}{mathematical fraktur capital j}%
\UnicodeMathSymbol{"1D50E}{\mfrakK                   }{\mathalpha}{mathematical fraktur capital k}%
\UnicodeMathSymbol{"1D50F}{\mfrakL                   }{\mathalpha}{mathematical fraktur capital l}%
\UnicodeMathSymbol{"1D510}{\mfrakM                   }{\mathalpha}{mathematical fraktur capital m}%
\UnicodeMathSymbol{"1D511}{\mfrakN                   }{\mathalpha}{mathematical fraktur capital n}%
\UnicodeMathSymbol{"1D512}{\mfrakO                   }{\mathalpha}{mathematical fraktur capital o}%
\UnicodeMathSymbol{"1D513}{\mfrakP                   }{\mathalpha}{mathematical fraktur capital p}%
\UnicodeMathSymbol{"1D514}{\mfrakQ                   }{\mathalpha}{mathematical fraktur capital q}%
\UnicodeMathSymbol{"1D516}{\mfrakS                   }{\mathalpha}{mathematical fraktur capital s}%
\UnicodeMathSymbol{"1D517}{\mfrakT                   }{\mathalpha}{mathematical fraktur capital t}%
\UnicodeMathSymbol{"1D518}{\mfrakU                   }{\mathalpha}{mathematical fraktur capital u}%
\UnicodeMathSymbol{"1D519}{\mfrakV                   }{\mathalpha}{mathematical fraktur capital v}%
\UnicodeMathSymbol{"1D51A}{\mfrakW                   }{\mathalpha}{mathematical fraktur capital w}%
\UnicodeMathSymbol{"1D51B}{\mfrakX                   }{\mathalpha}{mathematical fraktur capital x}%
\UnicodeMathSymbol{"1D51C}{\mfrakY                   }{\mathalpha}{mathematical fraktur capital y}%
\UnicodeMathSymbol{"1D51E}{\mfraka                   }{\mathalpha}{mathematical fraktur small a}%
\UnicodeMathSymbol{"1D51F}{\mfrakb                   }{\mathalpha}{mathematical fraktur small b}%
\UnicodeMathSymbol{"1D520}{\mfrakc                   }{\mathalpha}{mathematical fraktur small c}%
\UnicodeMathSymbol{"1D521}{\mfrakd                   }{\mathalpha}{mathematical fraktur small d}%
\UnicodeMathSymbol{"1D522}{\mfrake                   }{\mathalpha}{mathematical fraktur small e}%
\UnicodeMathSymbol{"1D523}{\mfrakf                   }{\mathalpha}{mathematical fraktur small f}%
\UnicodeMathSymbol{"1D524}{\mfrakg                   }{\mathalpha}{mathematical fraktur small g}%
\UnicodeMathSymbol{"1D525}{\mfrakh                   }{\mathalpha}{mathematical fraktur small h}%
\UnicodeMathSymbol{"1D526}{\mfraki                   }{\mathalpha}{mathematical fraktur small i}%
\UnicodeMathSymbol{"1D527}{\mfrakj                   }{\mathalpha}{mathematical fraktur small j}%
\UnicodeMathSymbol{"1D528}{\mfrakk                   }{\mathalpha}{mathematical fraktur small k}%
\UnicodeMathSymbol{"1D529}{\mfrakl                   }{\mathalpha}{mathematical fraktur small l}%
\UnicodeMathSymbol{"1D52A}{\mfrakm                   }{\mathalpha}{mathematical fraktur small m}%
\UnicodeMathSymbol{"1D52B}{\mfrakn                   }{\mathalpha}{mathematical fraktur small n}%
\UnicodeMathSymbol{"1D52C}{\mfrako                   }{\mathalpha}{mathematical fraktur small o}%
\UnicodeMathSymbol{"1D52D}{\mfrakp                   }{\mathalpha}{mathematical fraktur small p}%
\UnicodeMathSymbol{"1D52E}{\mfrakq                   }{\mathalpha}{mathematical fraktur small q}%
\UnicodeMathSymbol{"1D52F}{\mfrakr                   }{\mathalpha}{mathematical fraktur small r}%
\UnicodeMathSymbol{"1D530}{\mfraks                   }{\mathalpha}{mathematical fraktur small s}%
\UnicodeMathSymbol{"1D531}{\mfrakt                   }{\mathalpha}{mathematical fraktur small t}%
\UnicodeMathSymbol{"1D532}{\mfraku                   }{\mathalpha}{mathematical fraktur small u}%
\UnicodeMathSymbol{"1D533}{\mfrakv                   }{\mathalpha}{mathematical fraktur small v}%
\UnicodeMathSymbol{"1D534}{\mfrakw                   }{\mathalpha}{mathematical fraktur small w}%
\UnicodeMathSymbol{"1D535}{\mfrakx                   }{\mathalpha}{mathematical fraktur small x}%
\UnicodeMathSymbol{"1D536}{\mfraky                   }{\mathalpha}{mathematical fraktur small y}%
\UnicodeMathSymbol{"1D537}{\mfrakz                   }{\mathalpha}{mathematical fraktur small z}%
\UnicodeMathSymbol{"1D538}{\BbbA                     }{\mathalpha}{mathematical double-struck capital a}%
\UnicodeMathSymbol{"1D539}{\BbbB                     }{\mathalpha}{mathematical double-struck capital b}%
\UnicodeMathSymbol{"1D53B}{\BbbD                     }{\mathalpha}{mathematical double-struck capital d}%
\UnicodeMathSymbol{"1D53C}{\BbbE                     }{\mathalpha}{mathematical double-struck capital e}%
\UnicodeMathSymbol{"1D53D}{\BbbF                     }{\mathalpha}{mathematical double-struck capital f}%
\UnicodeMathSymbol{"1D53E}{\BbbG                     }{\mathalpha}{mathematical double-struck capital g}%
\UnicodeMathSymbol{"1D540}{\BbbI                     }{\mathalpha}{mathematical double-struck capital i}%
\UnicodeMathSymbol{"1D541}{\BbbJ                     }{\mathalpha}{mathematical double-struck capital j}%
\UnicodeMathSymbol{"1D542}{\BbbK                     }{\mathalpha}{mathematical double-struck capital k}%
\UnicodeMathSymbol{"1D543}{\BbbL                     }{\mathalpha}{mathematical double-struck capital l}%
\UnicodeMathSymbol{"1D544}{\BbbM                     }{\mathalpha}{mathematical double-struck capital m}%
\UnicodeMathSymbol{"1D546}{\BbbO                     }{\mathalpha}{mathematical double-struck capital o}%
\UnicodeMathSymbol{"1D54A}{\BbbS                     }{\mathalpha}{mathematical double-struck capital s}%
\UnicodeMathSymbol{"1D54B}{\BbbT                     }{\mathalpha}{mathematical double-struck capital t}%
\UnicodeMathSymbol{"1D54C}{\BbbU                     }{\mathalpha}{mathematical double-struck capital u}%
\UnicodeMathSymbol{"1D54D}{\BbbV                     }{\mathalpha}{mathematical double-struck capital v}%
\UnicodeMathSymbol{"1D54E}{\BbbW                     }{\mathalpha}{mathematical double-struck capital w}%
\UnicodeMathSymbol{"1D54F}{\BbbX                     }{\mathalpha}{mathematical double-struck capital x}%
\UnicodeMathSymbol{"1D550}{\BbbY                     }{\mathalpha}{mathematical double-struck capital y}%
\UnicodeMathSymbol{"1D552}{\Bbba                     }{\mathalpha}{mathematical double-struck small a}%
\UnicodeMathSymbol{"1D553}{\Bbbb                     }{\mathalpha}{mathematical double-struck small b}%
\UnicodeMathSymbol{"1D554}{\Bbbc                     }{\mathalpha}{mathematical double-struck small c}%
\UnicodeMathSymbol{"1D555}{\Bbbd                     }{\mathalpha}{mathematical double-struck small d}%
\UnicodeMathSymbol{"1D556}{\Bbbe                     }{\mathalpha}{mathematical double-struck small e}%
\UnicodeMathSymbol{"1D557}{\Bbbf                     }{\mathalpha}{mathematical double-struck small f}%
\UnicodeMathSymbol{"1D558}{\Bbbg                     }{\mathalpha}{mathematical double-struck small g}%
\UnicodeMathSymbol{"1D559}{\Bbbh                     }{\mathalpha}{mathematical double-struck small h}%
\UnicodeMathSymbol{"1D55A}{\Bbbi                     }{\mathalpha}{mathematical double-struck small i}%
\UnicodeMathSymbol{"1D55B}{\Bbbj                     }{\mathalpha}{mathematical double-struck small j}%
\UnicodeMathSymbol{"1D55C}{\Bbbk                     }{\mathalpha}{mathematical double-struck small k}%
\UnicodeMathSymbol{"1D55D}{\Bbbl                     }{\mathalpha}{mathematical double-struck small l}%
\UnicodeMathSymbol{"1D55E}{\Bbbm                     }{\mathalpha}{mathematical double-struck small m}%
\UnicodeMathSymbol{"1D55F}{\Bbbn                     }{\mathalpha}{mathematical double-struck small n}%
\UnicodeMathSymbol{"1D560}{\Bbbo                     }{\mathalpha}{mathematical double-struck small o}%
\UnicodeMathSymbol{"1D561}{\Bbbp                     }{\mathalpha}{mathematical double-struck small p}%
\UnicodeMathSymbol{"1D562}{\Bbbq                     }{\mathalpha}{mathematical double-struck small q}%
\UnicodeMathSymbol{"1D563}{\Bbbr                     }{\mathalpha}{mathematical double-struck small r}%
\UnicodeMathSymbol{"1D564}{\Bbbs                     }{\mathalpha}{mathematical double-struck small s}%
\UnicodeMathSymbol{"1D565}{\Bbbt                     }{\mathalpha}{mathematical double-struck small t}%
\UnicodeMathSymbol{"1D566}{\Bbbu                     }{\mathalpha}{mathematical double-struck small u}%
\UnicodeMathSymbol{"1D567}{\Bbbv                     }{\mathalpha}{mathematical double-struck small v}%
\UnicodeMathSymbol{"1D568}{\Bbbw                     }{\mathalpha}{mathematical double-struck small w}%
\UnicodeMathSymbol{"1D569}{\Bbbx                     }{\mathalpha}{mathematical double-struck small x}%
\UnicodeMathSymbol{"1D56A}{\Bbby                     }{\mathalpha}{mathematical double-struck small y}%
\UnicodeMathSymbol{"1D56B}{\Bbbz                     }{\mathalpha}{mathematical double-struck small z}%
\UnicodeMathSymbol{"1D56C}{\mbffrakA                 }{\mathalpha}{mathematical bold fraktur capital a}%
\UnicodeMathSymbol{"1D56D}{\mbffrakB                 }{\mathalpha}{mathematical bold fraktur capital b}%
\UnicodeMathSymbol{"1D56E}{\mbffrakC                 }{\mathalpha}{mathematical bold fraktur capital c}%
\UnicodeMathSymbol{"1D56F}{\mbffrakD                 }{\mathalpha}{mathematical bold fraktur capital d}%
\UnicodeMathSymbol{"1D570}{\mbffrakE                 }{\mathalpha}{mathematical bold fraktur capital e}%
\UnicodeMathSymbol{"1D571}{\mbffrakF                 }{\mathalpha}{mathematical bold fraktur capital f}%
\UnicodeMathSymbol{"1D572}{\mbffrakG                 }{\mathalpha}{mathematical bold fraktur capital g}%
\UnicodeMathSymbol{"1D573}{\mbffrakH                 }{\mathalpha}{mathematical bold fraktur capital h}%
\UnicodeMathSymbol{"1D574}{\mbffrakI                 }{\mathalpha}{mathematical bold fraktur capital i}%
\UnicodeMathSymbol{"1D575}{\mbffrakJ                 }{\mathalpha}{mathematical bold fraktur capital j}%
\UnicodeMathSymbol{"1D576}{\mbffrakK                 }{\mathalpha}{mathematical bold fraktur capital k}%
\UnicodeMathSymbol{"1D577}{\mbffrakL                 }{\mathalpha}{mathematical bold fraktur capital l}%
\UnicodeMathSymbol{"1D578}{\mbffrakM                 }{\mathalpha}{mathematical bold fraktur capital m}%
\UnicodeMathSymbol{"1D579}{\mbffrakN                 }{\mathalpha}{mathematical bold fraktur capital n}%
\UnicodeMathSymbol{"1D57A}{\mbffrakO                 }{\mathalpha}{mathematical bold fraktur capital o}%
\UnicodeMathSymbol{"1D57B}{\mbffrakP                 }{\mathalpha}{mathematical bold fraktur capital p}%
\UnicodeMathSymbol{"1D57C}{\mbffrakQ                 }{\mathalpha}{mathematical bold fraktur capital q}%
\UnicodeMathSymbol{"1D57D}{\mbffrakR                 }{\mathalpha}{mathematical bold fraktur capital r}%
\UnicodeMathSymbol{"1D57E}{\mbffrakS                 }{\mathalpha}{mathematical bold fraktur capital s}%
\UnicodeMathSymbol{"1D57F}{\mbffrakT                 }{\mathalpha}{mathematical bold fraktur capital t}%
\UnicodeMathSymbol{"1D580}{\mbffrakU                 }{\mathalpha}{mathematical bold fraktur capital u}%
\UnicodeMathSymbol{"1D581}{\mbffrakV                 }{\mathalpha}{mathematical bold fraktur capital v}%
\UnicodeMathSymbol{"1D582}{\mbffrakW                 }{\mathalpha}{mathematical bold fraktur capital w}%
\UnicodeMathSymbol{"1D583}{\mbffrakX                 }{\mathalpha}{mathematical bold fraktur capital x}%
\UnicodeMathSymbol{"1D584}{\mbffrakY                 }{\mathalpha}{mathematical bold fraktur capital y}%
\UnicodeMathSymbol{"1D585}{\mbffrakZ                 }{\mathalpha}{mathematical bold fraktur capital z}%
\UnicodeMathSymbol{"1D586}{\mbffraka                 }{\mathalpha}{mathematical bold fraktur small a}%
\UnicodeMathSymbol{"1D587}{\mbffrakb                 }{\mathalpha}{mathematical bold fraktur small b}%
\UnicodeMathSymbol{"1D588}{\mbffrakc                 }{\mathalpha}{mathematical bold fraktur small c}%
\UnicodeMathSymbol{"1D589}{\mbffrakd                 }{\mathalpha}{mathematical bold fraktur small d}%
\UnicodeMathSymbol{"1D58A}{\mbffrake                 }{\mathalpha}{mathematical bold fraktur small e}%
\UnicodeMathSymbol{"1D58B}{\mbffrakf                 }{\mathalpha}{mathematical bold fraktur small f}%
\UnicodeMathSymbol{"1D58C}{\mbffrakg                 }{\mathalpha}{mathematical bold fraktur small g}%
\UnicodeMathSymbol{"1D58D}{\mbffrakh                 }{\mathalpha}{mathematical bold fraktur small h}%
\UnicodeMathSymbol{"1D58E}{\mbffraki                 }{\mathalpha}{mathematical bold fraktur small i}%
\UnicodeMathSymbol{"1D58F}{\mbffrakj                 }{\mathalpha}{mathematical bold fraktur small j}%
\UnicodeMathSymbol{"1D590}{\mbffrakk                 }{\mathalpha}{mathematical bold fraktur small k}%
\UnicodeMathSymbol{"1D591}{\mbffrakl                 }{\mathalpha}{mathematical bold fraktur small l}%
\UnicodeMathSymbol{"1D592}{\mbffrakm                 }{\mathalpha}{mathematical bold fraktur small m}%
\UnicodeMathSymbol{"1D593}{\mbffrakn                 }{\mathalpha}{mathematical bold fraktur small n}%
\UnicodeMathSymbol{"1D594}{\mbffrako                 }{\mathalpha}{mathematical bold fraktur small o}%
\UnicodeMathSymbol{"1D595}{\mbffrakp                 }{\mathalpha}{mathematical bold fraktur small p}%
\UnicodeMathSymbol{"1D596}{\mbffrakq                 }{\mathalpha}{mathematical bold fraktur small q}%
\UnicodeMathSymbol{"1D597}{\mbffrakr                 }{\mathalpha}{mathematical bold fraktur small r}%
\UnicodeMathSymbol{"1D598}{\mbffraks                 }{\mathalpha}{mathematical bold fraktur small s}%
\UnicodeMathSymbol{"1D599}{\mbffrakt                 }{\mathalpha}{mathematical bold fraktur small t}%
\UnicodeMathSymbol{"1D59A}{\mbffraku                 }{\mathalpha}{mathematical bold fraktur small u}%
\UnicodeMathSymbol{"1D59B}{\mbffrakv                 }{\mathalpha}{mathematical bold fraktur small v}%
\UnicodeMathSymbol{"1D59C}{\mbffrakw                 }{\mathalpha}{mathematical bold fraktur small w}%
\UnicodeMathSymbol{"1D59D}{\mbffrakx                 }{\mathalpha}{mathematical bold fraktur small x}%
\UnicodeMathSymbol{"1D59E}{\mbffraky                 }{\mathalpha}{mathematical bold fraktur small y}%
\UnicodeMathSymbol{"1D59F}{\mbffrakz                 }{\mathalpha}{mathematical bold fraktur small z}%
\UnicodeMathSymbol{"1D5A0}{\msansA                   }{\mathalpha}{mathematical sans-serif capital a}%
\UnicodeMathSymbol{"1D5A1}{\msansB                   }{\mathalpha}{mathematical sans-serif capital b}%
\UnicodeMathSymbol{"1D5A2}{\msansC                   }{\mathalpha}{mathematical sans-serif capital c}%
\UnicodeMathSymbol{"1D5A3}{\msansD                   }{\mathalpha}{mathematical sans-serif capital d}%
\UnicodeMathSymbol{"1D5A4}{\msansE                   }{\mathalpha}{mathematical sans-serif capital e}%
\UnicodeMathSymbol{"1D5A5}{\msansF                   }{\mathalpha}{mathematical sans-serif capital f}%
\UnicodeMathSymbol{"1D5A6}{\msansG                   }{\mathalpha}{mathematical sans-serif capital g}%
\UnicodeMathSymbol{"1D5A7}{\msansH                   }{\mathalpha}{mathematical sans-serif capital h}%
\UnicodeMathSymbol{"1D5A8}{\msansI                   }{\mathalpha}{mathematical sans-serif capital i}%
\UnicodeMathSymbol{"1D5A9}{\msansJ                   }{\mathalpha}{mathematical sans-serif capital j}%
\UnicodeMathSymbol{"1D5AA}{\msansK                   }{\mathalpha}{mathematical sans-serif capital k}%
\UnicodeMathSymbol{"1D5AB}{\msansL                   }{\mathalpha}{mathematical sans-serif capital l}%
\UnicodeMathSymbol{"1D5AC}{\msansM                   }{\mathalpha}{mathematical sans-serif capital m}%
\UnicodeMathSymbol{"1D5AD}{\msansN                   }{\mathalpha}{mathematical sans-serif capital n}%
\UnicodeMathSymbol{"1D5AE}{\msansO                   }{\mathalpha}{mathematical sans-serif capital o}%
\UnicodeMathSymbol{"1D5AF}{\msansP                   }{\mathalpha}{mathematical sans-serif capital p}%
\UnicodeMathSymbol{"1D5B0}{\msansQ                   }{\mathalpha}{mathematical sans-serif capital q}%
\UnicodeMathSymbol{"1D5B1}{\msansR                   }{\mathalpha}{mathematical sans-serif capital r}%
\UnicodeMathSymbol{"1D5B2}{\msansS                   }{\mathalpha}{mathematical sans-serif capital s}%
\UnicodeMathSymbol{"1D5B3}{\msansT                   }{\mathalpha}{mathematical sans-serif capital t}%
\UnicodeMathSymbol{"1D5B4}{\msansU                   }{\mathalpha}{mathematical sans-serif capital u}%
\UnicodeMathSymbol{"1D5B5}{\msansV                   }{\mathalpha}{mathematical sans-serif capital v}%
\UnicodeMathSymbol{"1D5B6}{\msansW                   }{\mathalpha}{mathematical sans-serif capital w}%
\UnicodeMathSymbol{"1D5B7}{\msansX                   }{\mathalpha}{mathematical sans-serif capital x}%
\UnicodeMathSymbol{"1D5B8}{\msansY                   }{\mathalpha}{mathematical sans-serif capital y}%
\UnicodeMathSymbol{"1D5B9}{\msansZ                   }{\mathalpha}{mathematical sans-serif capital z}%
\UnicodeMathSymbol{"1D5BA}{\msansa                   }{\mathalpha}{mathematical sans-serif small a}%
\UnicodeMathSymbol{"1D5BB}{\msansb                   }{\mathalpha}{mathematical sans-serif small b}%
\UnicodeMathSymbol{"1D5BC}{\msansc                   }{\mathalpha}{mathematical sans-serif small c}%
\UnicodeMathSymbol{"1D5BD}{\msansd                   }{\mathalpha}{mathematical sans-serif small d}%
\UnicodeMathSymbol{"1D5BE}{\msanse                   }{\mathalpha}{mathematical sans-serif small e}%
\UnicodeMathSymbol{"1D5BF}{\msansf                   }{\mathalpha}{mathematical sans-serif small f}%
\UnicodeMathSymbol{"1D5C0}{\msansg                   }{\mathalpha}{mathematical sans-serif small g}%
\UnicodeMathSymbol{"1D5C1}{\msansh                   }{\mathalpha}{mathematical sans-serif small h}%
\UnicodeMathSymbol{"1D5C2}{\msansi                   }{\mathalpha}{mathematical sans-serif small i}%
\UnicodeMathSymbol{"1D5C3}{\msansj                   }{\mathalpha}{mathematical sans-serif small j}%
\UnicodeMathSymbol{"1D5C4}{\msansk                   }{\mathalpha}{mathematical sans-serif small k}%
\UnicodeMathSymbol{"1D5C5}{\msansl                   }{\mathalpha}{mathematical sans-serif small l}%
\UnicodeMathSymbol{"1D5C6}{\msansm                   }{\mathalpha}{mathematical sans-serif small m}%
\UnicodeMathSymbol{"1D5C7}{\msansn                   }{\mathalpha}{mathematical sans-serif small n}%
\UnicodeMathSymbol{"1D5C8}{\msanso                   }{\mathalpha}{mathematical sans-serif small o}%
\UnicodeMathSymbol{"1D5C9}{\msansp                   }{\mathalpha}{mathematical sans-serif small p}%
\UnicodeMathSymbol{"1D5CA}{\msansq                   }{\mathalpha}{mathematical sans-serif small q}%
\UnicodeMathSymbol{"1D5CB}{\msansr                   }{\mathalpha}{mathematical sans-serif small r}%
\UnicodeMathSymbol{"1D5CC}{\msanss                   }{\mathalpha}{mathematical sans-serif small s}%
\UnicodeMathSymbol{"1D5CD}{\msanst                   }{\mathalpha}{mathematical sans-serif small t}%
\UnicodeMathSymbol{"1D5CE}{\msansu                   }{\mathalpha}{mathematical sans-serif small u}%
\UnicodeMathSymbol{"1D5CF}{\msansv                   }{\mathalpha}{mathematical sans-serif small v}%
\UnicodeMathSymbol{"1D5D0}{\msansw                   }{\mathalpha}{mathematical sans-serif small w}%
\UnicodeMathSymbol{"1D5D1}{\msansx                   }{\mathalpha}{mathematical sans-serif small x}%
\UnicodeMathSymbol{"1D5D2}{\msansy                   }{\mathalpha}{mathematical sans-serif small y}%
\UnicodeMathSymbol{"1D5D3}{\msansz                   }{\mathalpha}{mathematical sans-serif small z}%
\UnicodeMathSymbol{"1D5D4}{\mbfsansA                 }{\mathalpha}{mathematical sans-serif bold capital a}%
\UnicodeMathSymbol{"1D5D5}{\mbfsansB                 }{\mathalpha}{mathematical sans-serif bold capital b}%
\UnicodeMathSymbol{"1D5D6}{\mbfsansC                 }{\mathalpha}{mathematical sans-serif bold capital c}%
\UnicodeMathSymbol{"1D5D7}{\mbfsansD                 }{\mathalpha}{mathematical sans-serif bold capital d}%
\UnicodeMathSymbol{"1D5D8}{\mbfsansE                 }{\mathalpha}{mathematical sans-serif bold capital e}%
\UnicodeMathSymbol{"1D5D9}{\mbfsansF                 }{\mathalpha}{mathematical sans-serif bold capital f}%
\UnicodeMathSymbol{"1D5DA}{\mbfsansG                 }{\mathalpha}{mathematical sans-serif bold capital g}%
\UnicodeMathSymbol{"1D5DB}{\mbfsansH                 }{\mathalpha}{mathematical sans-serif bold capital h}%
\UnicodeMathSymbol{"1D5DC}{\mbfsansI                 }{\mathalpha}{mathematical sans-serif bold capital i}%
\UnicodeMathSymbol{"1D5DD}{\mbfsansJ                 }{\mathalpha}{mathematical sans-serif bold capital j}%
\UnicodeMathSymbol{"1D5DE}{\mbfsansK                 }{\mathalpha}{mathematical sans-serif bold capital k}%
\UnicodeMathSymbol{"1D5DF}{\mbfsansL                 }{\mathalpha}{mathematical sans-serif bold capital l}%
\UnicodeMathSymbol{"1D5E0}{\mbfsansM                 }{\mathalpha}{mathematical sans-serif bold capital m}%
\UnicodeMathSymbol{"1D5E1}{\mbfsansN                 }{\mathalpha}{mathematical sans-serif bold capital n}%
\UnicodeMathSymbol{"1D5E2}{\mbfsansO                 }{\mathalpha}{mathematical sans-serif bold capital o}%
\UnicodeMathSymbol{"1D5E3}{\mbfsansP                 }{\mathalpha}{mathematical sans-serif bold capital p}%
\UnicodeMathSymbol{"1D5E4}{\mbfsansQ                 }{\mathalpha}{mathematical sans-serif bold capital q}%
\UnicodeMathSymbol{"1D5E5}{\mbfsansR                 }{\mathalpha}{mathematical sans-serif bold capital r}%
\UnicodeMathSymbol{"1D5E6}{\mbfsansS                 }{\mathalpha}{mathematical sans-serif bold capital s}%
\UnicodeMathSymbol{"1D5E7}{\mbfsansT                 }{\mathalpha}{mathematical sans-serif bold capital t}%
\UnicodeMathSymbol{"1D5E8}{\mbfsansU                 }{\mathalpha}{mathematical sans-serif bold capital u}%
\UnicodeMathSymbol{"1D5E9}{\mbfsansV                 }{\mathalpha}{mathematical sans-serif bold capital v}%
\UnicodeMathSymbol{"1D5EA}{\mbfsansW                 }{\mathalpha}{mathematical sans-serif bold capital w}%
\UnicodeMathSymbol{"1D5EB}{\mbfsansX                 }{\mathalpha}{mathematical sans-serif bold capital x}%
\UnicodeMathSymbol{"1D5EC}{\mbfsansY                 }{\mathalpha}{mathematical sans-serif bold capital y}%
\UnicodeMathSymbol{"1D5ED}{\mbfsansZ                 }{\mathalpha}{mathematical sans-serif bold capital z}%
\UnicodeMathSymbol{"1D5EE}{\mbfsansa                 }{\mathalpha}{mathematical sans-serif bold small a}%
\UnicodeMathSymbol{"1D5EF}{\mbfsansb                 }{\mathalpha}{mathematical sans-serif bold small b}%
\UnicodeMathSymbol{"1D5F0}{\mbfsansc                 }{\mathalpha}{mathematical sans-serif bold small c}%
\UnicodeMathSymbol{"1D5F1}{\mbfsansd                 }{\mathalpha}{mathematical sans-serif bold small d}%
\UnicodeMathSymbol{"1D5F2}{\mbfsanse                 }{\mathalpha}{mathematical sans-serif bold small e}%
\UnicodeMathSymbol{"1D5F3}{\mbfsansf                 }{\mathalpha}{mathematical sans-serif bold small f}%
\UnicodeMathSymbol{"1D5F4}{\mbfsansg                 }{\mathalpha}{mathematical sans-serif bold small g}%
\UnicodeMathSymbol{"1D5F5}{\mbfsansh                 }{\mathalpha}{mathematical sans-serif bold small h}%
\UnicodeMathSymbol{"1D5F6}{\mbfsansi                 }{\mathalpha}{mathematical sans-serif bold small i}%
\UnicodeMathSymbol{"1D5F7}{\mbfsansj                 }{\mathalpha}{mathematical sans-serif bold small j}%
\UnicodeMathSymbol{"1D5F8}{\mbfsansk                 }{\mathalpha}{mathematical sans-serif bold small k}%
\UnicodeMathSymbol{"1D5F9}{\mbfsansl                 }{\mathalpha}{mathematical sans-serif bold small l}%
\UnicodeMathSymbol{"1D5FA}{\mbfsansm                 }{\mathalpha}{mathematical sans-serif bold small m}%
\UnicodeMathSymbol{"1D5FB}{\mbfsansn                 }{\mathalpha}{mathematical sans-serif bold small n}%
\UnicodeMathSymbol{"1D5FC}{\mbfsanso                 }{\mathalpha}{mathematical sans-serif bold small o}%
\UnicodeMathSymbol{"1D5FD}{\mbfsansp                 }{\mathalpha}{mathematical sans-serif bold small p}%
\UnicodeMathSymbol{"1D5FE}{\mbfsansq                 }{\mathalpha}{mathematical sans-serif bold small q}%
\UnicodeMathSymbol{"1D5FF}{\mbfsansr                 }{\mathalpha}{mathematical sans-serif bold small r}%
\UnicodeMathSymbol{"1D600}{\mbfsanss                 }{\mathalpha}{mathematical sans-serif bold small s}%
\UnicodeMathSymbol{"1D601}{\mbfsanst                 }{\mathalpha}{mathematical sans-serif bold small t}%
\UnicodeMathSymbol{"1D602}{\mbfsansu                 }{\mathalpha}{mathematical sans-serif bold small u}%
\UnicodeMathSymbol{"1D603}{\mbfsansv                 }{\mathalpha}{mathematical sans-serif bold small v}%
\UnicodeMathSymbol{"1D604}{\mbfsansw                 }{\mathalpha}{mathematical sans-serif bold small w}%
\UnicodeMathSymbol{"1D605}{\mbfsansx                 }{\mathalpha}{mathematical sans-serif bold small x}%
\UnicodeMathSymbol{"1D606}{\mbfsansy                 }{\mathalpha}{mathematical sans-serif bold small y}%
\UnicodeMathSymbol{"1D607}{\mbfsansz                 }{\mathalpha}{mathematical sans-serif bold small z}%
\UnicodeMathSymbol{"1D608}{\mitsansA                 }{\mathalpha}{mathematical sans-serif italic capital a}%
\UnicodeMathSymbol{"1D609}{\mitsansB                 }{\mathalpha}{mathematical sans-serif italic capital b}%
\UnicodeMathSymbol{"1D60A}{\mitsansC                 }{\mathalpha}{mathematical sans-serif italic capital c}%
\UnicodeMathSymbol{"1D60B}{\mitsansD                 }{\mathalpha}{mathematical sans-serif italic capital d}%
\UnicodeMathSymbol{"1D60C}{\mitsansE                 }{\mathalpha}{mathematical sans-serif italic capital e}%
\UnicodeMathSymbol{"1D60D}{\mitsansF                 }{\mathalpha}{mathematical sans-serif italic capital f}%
\UnicodeMathSymbol{"1D60E}{\mitsansG                 }{\mathalpha}{mathematical sans-serif italic capital g}%
\UnicodeMathSymbol{"1D60F}{\mitsansH                 }{\mathalpha}{mathematical sans-serif italic capital h}%
\UnicodeMathSymbol{"1D610}{\mitsansI                 }{\mathalpha}{mathematical sans-serif italic capital i}%
\UnicodeMathSymbol{"1D611}{\mitsansJ                 }{\mathalpha}{mathematical sans-serif italic capital j}%
\UnicodeMathSymbol{"1D612}{\mitsansK                 }{\mathalpha}{mathematical sans-serif italic capital k}%
\UnicodeMathSymbol{"1D613}{\mitsansL                 }{\mathalpha}{mathematical sans-serif italic capital l}%
\UnicodeMathSymbol{"1D614}{\mitsansM                 }{\mathalpha}{mathematical sans-serif italic capital m}%
\UnicodeMathSymbol{"1D615}{\mitsansN                 }{\mathalpha}{mathematical sans-serif italic capital n}%
\UnicodeMathSymbol{"1D616}{\mitsansO                 }{\mathalpha}{mathematical sans-serif italic capital o}%
\UnicodeMathSymbol{"1D617}{\mitsansP                 }{\mathalpha}{mathematical sans-serif italic capital p}%
\UnicodeMathSymbol{"1D618}{\mitsansQ                 }{\mathalpha}{mathematical sans-serif italic capital q}%
\UnicodeMathSymbol{"1D619}{\mitsansR                 }{\mathalpha}{mathematical sans-serif italic capital r}%
\UnicodeMathSymbol{"1D61A}{\mitsansS                 }{\mathalpha}{mathematical sans-serif italic capital s}%
\UnicodeMathSymbol{"1D61B}{\mitsansT                 }{\mathalpha}{mathematical sans-serif italic capital t}%
\UnicodeMathSymbol{"1D61C}{\mitsansU                 }{\mathalpha}{mathematical sans-serif italic capital u}%
\UnicodeMathSymbol{"1D61D}{\mitsansV                 }{\mathalpha}{mathematical sans-serif italic capital v}%
\UnicodeMathSymbol{"1D61E}{\mitsansW                 }{\mathalpha}{mathematical sans-serif italic capital w}%
\UnicodeMathSymbol{"1D61F}{\mitsansX                 }{\mathalpha}{mathematical sans-serif italic capital x}%
\UnicodeMathSymbol{"1D620}{\mitsansY                 }{\mathalpha}{mathematical sans-serif italic capital y}%
\UnicodeMathSymbol{"1D621}{\mitsansZ                 }{\mathalpha}{mathematical sans-serif italic capital z}%
\UnicodeMathSymbol{"1D622}{\mitsansa                 }{\mathalpha}{mathematical sans-serif italic small a}%
\UnicodeMathSymbol{"1D623}{\mitsansb                 }{\mathalpha}{mathematical sans-serif italic small b}%
\UnicodeMathSymbol{"1D624}{\mitsansc                 }{\mathalpha}{mathematical sans-serif italic small c}%
\UnicodeMathSymbol{"1D625}{\mitsansd                 }{\mathalpha}{mathematical sans-serif italic small d}%
\UnicodeMathSymbol{"1D626}{\mitsanse                 }{\mathalpha}{mathematical sans-serif italic small e}%
\UnicodeMathSymbol{"1D627}{\mitsansf                 }{\mathalpha}{mathematical sans-serif italic small f}%
\UnicodeMathSymbol{"1D628}{\mitsansg                 }{\mathalpha}{mathematical sans-serif italic small g}%
\UnicodeMathSymbol{"1D629}{\mitsansh                 }{\mathalpha}{mathematical sans-serif italic small h}%
\UnicodeMathSymbol{"1D62A}{\mitsansi                 }{\mathalpha}{mathematical sans-serif italic small i}%
\UnicodeMathSymbol{"1D62B}{\mitsansj                 }{\mathalpha}{mathematical sans-serif italic small j}%
\UnicodeMathSymbol{"1D62C}{\mitsansk                 }{\mathalpha}{mathematical sans-serif italic small k}%
\UnicodeMathSymbol{"1D62D}{\mitsansl                 }{\mathalpha}{mathematical sans-serif italic small l}%
\UnicodeMathSymbol{"1D62E}{\mitsansm                 }{\mathalpha}{mathematical sans-serif italic small m}%
\UnicodeMathSymbol{"1D62F}{\mitsansn                 }{\mathalpha}{mathematical sans-serif italic small n}%
\UnicodeMathSymbol{"1D630}{\mitsanso                 }{\mathalpha}{mathematical sans-serif italic small o}%
\UnicodeMathSymbol{"1D631}{\mitsansp                 }{\mathalpha}{mathematical sans-serif italic small p}%
\UnicodeMathSymbol{"1D632}{\mitsansq                 }{\mathalpha}{mathematical sans-serif italic small q}%
\UnicodeMathSymbol{"1D633}{\mitsansr                 }{\mathalpha}{mathematical sans-serif italic small r}%
\UnicodeMathSymbol{"1D634}{\mitsanss                 }{\mathalpha}{mathematical sans-serif italic small s}%
\UnicodeMathSymbol{"1D635}{\mitsanst                 }{\mathalpha}{mathematical sans-serif italic small t}%
\UnicodeMathSymbol{"1D636}{\mitsansu                 }{\mathalpha}{mathematical sans-serif italic small u}%
\UnicodeMathSymbol{"1D637}{\mitsansv                 }{\mathalpha}{mathematical sans-serif italic small v}%
\UnicodeMathSymbol{"1D638}{\mitsansw                 }{\mathalpha}{mathematical sans-serif italic small w}%
\UnicodeMathSymbol{"1D639}{\mitsansx                 }{\mathalpha}{mathematical sans-serif italic small x}%
\UnicodeMathSymbol{"1D63A}{\mitsansy                 }{\mathalpha}{mathematical sans-serif italic small y}%
\UnicodeMathSymbol{"1D63B}{\mitsansz                 }{\mathalpha}{mathematical sans-serif italic small z}%
\UnicodeMathSymbol{"1D63C}{\mbfitsansA               }{\mathalpha}{mathematical sans-serif bold italic capital a}%
\UnicodeMathSymbol{"1D63D}{\mbfitsansB               }{\mathalpha}{mathematical sans-serif bold italic capital b}%
\UnicodeMathSymbol{"1D63E}{\mbfitsansC               }{\mathalpha}{mathematical sans-serif bold italic capital c}%
\UnicodeMathSymbol{"1D63F}{\mbfitsansD               }{\mathalpha}{mathematical sans-serif bold italic capital d}%
\UnicodeMathSymbol{"1D640}{\mbfitsansE               }{\mathalpha}{mathematical sans-serif bold italic capital e}%
\UnicodeMathSymbol{"1D641}{\mbfitsansF               }{\mathalpha}{mathematical sans-serif bold italic capital f}%
\UnicodeMathSymbol{"1D642}{\mbfitsansG               }{\mathalpha}{mathematical sans-serif bold italic capital g}%
\UnicodeMathSymbol{"1D643}{\mbfitsansH               }{\mathalpha}{mathematical sans-serif bold italic capital h}%
\UnicodeMathSymbol{"1D644}{\mbfitsansI               }{\mathalpha}{mathematical sans-serif bold italic capital i}%
\UnicodeMathSymbol{"1D645}{\mbfitsansJ               }{\mathalpha}{mathematical sans-serif bold italic capital j}%
\UnicodeMathSymbol{"1D646}{\mbfitsansK               }{\mathalpha}{mathematical sans-serif bold italic capital k}%
\UnicodeMathSymbol{"1D647}{\mbfitsansL               }{\mathalpha}{mathematical sans-serif bold italic capital l}%
\UnicodeMathSymbol{"1D648}{\mbfitsansM               }{\mathalpha}{mathematical sans-serif bold italic capital m}%
\UnicodeMathSymbol{"1D649}{\mbfitsansN               }{\mathalpha}{mathematical sans-serif bold italic capital n}%
\UnicodeMathSymbol{"1D64A}{\mbfitsansO               }{\mathalpha}{mathematical sans-serif bold italic capital o}%
\UnicodeMathSymbol{"1D64B}{\mbfitsansP               }{\mathalpha}{mathematical sans-serif bold italic capital p}%
\UnicodeMathSymbol{"1D64C}{\mbfitsansQ               }{\mathalpha}{mathematical sans-serif bold italic capital q}%
\UnicodeMathSymbol{"1D64D}{\mbfitsansR               }{\mathalpha}{mathematical sans-serif bold italic capital r}%
\UnicodeMathSymbol{"1D64E}{\mbfitsansS               }{\mathalpha}{mathematical sans-serif bold italic capital s}%
\UnicodeMathSymbol{"1D64F}{\mbfitsansT               }{\mathalpha}{mathematical sans-serif bold italic capital t}%
\UnicodeMathSymbol{"1D650}{\mbfitsansU               }{\mathalpha}{mathematical sans-serif bold italic capital u}%
\UnicodeMathSymbol{"1D651}{\mbfitsansV               }{\mathalpha}{mathematical sans-serif bold italic capital v}%
\UnicodeMathSymbol{"1D652}{\mbfitsansW               }{\mathalpha}{mathematical sans-serif bold italic capital w}%
\UnicodeMathSymbol{"1D653}{\mbfitsansX               }{\mathalpha}{mathematical sans-serif bold italic capital x}%
\UnicodeMathSymbol{"1D654}{\mbfitsansY               }{\mathalpha}{mathematical sans-serif bold italic capital y}%
\UnicodeMathSymbol{"1D655}{\mbfitsansZ               }{\mathalpha}{mathematical sans-serif bold italic capital z}%
\UnicodeMathSymbol{"1D656}{\mbfitsansa               }{\mathalpha}{mathematical sans-serif bold italic small a}%
\UnicodeMathSymbol{"1D657}{\mbfitsansb               }{\mathalpha}{mathematical sans-serif bold italic small b}%
\UnicodeMathSymbol{"1D658}{\mbfitsansc               }{\mathalpha}{mathematical sans-serif bold italic small c}%
\UnicodeMathSymbol{"1D659}{\mbfitsansd               }{\mathalpha}{mathematical sans-serif bold italic small d}%
\UnicodeMathSymbol{"1D65A}{\mbfitsanse               }{\mathalpha}{mathematical sans-serif bold italic small e}%
\UnicodeMathSymbol{"1D65B}{\mbfitsansf               }{\mathalpha}{mathematical sans-serif bold italic small f}%
\UnicodeMathSymbol{"1D65C}{\mbfitsansg               }{\mathalpha}{mathematical sans-serif bold italic small g}%
\UnicodeMathSymbol{"1D65D}{\mbfitsansh               }{\mathalpha}{mathematical sans-serif bold italic small h}%
\UnicodeMathSymbol{"1D65E}{\mbfitsansi               }{\mathalpha}{mathematical sans-serif bold italic small i}%
\UnicodeMathSymbol{"1D65F}{\mbfitsansj               }{\mathalpha}{mathematical sans-serif bold italic small j}%
\UnicodeMathSymbol{"1D660}{\mbfitsansk               }{\mathalpha}{mathematical sans-serif bold italic small k}%
\UnicodeMathSymbol{"1D661}{\mbfitsansl               }{\mathalpha}{mathematical sans-serif bold italic small l}%
\UnicodeMathSymbol{"1D662}{\mbfitsansm               }{\mathalpha}{mathematical sans-serif bold italic small m}%
\UnicodeMathSymbol{"1D663}{\mbfitsansn               }{\mathalpha}{mathematical sans-serif bold italic small n}%
\UnicodeMathSymbol{"1D664}{\mbfitsanso               }{\mathalpha}{mathematical sans-serif bold italic small o}%
\UnicodeMathSymbol{"1D665}{\mbfitsansp               }{\mathalpha}{mathematical sans-serif bold italic small p}%
\UnicodeMathSymbol{"1D666}{\mbfitsansq               }{\mathalpha}{mathematical sans-serif bold italic small q}%
\UnicodeMathSymbol{"1D667}{\mbfitsansr               }{\mathalpha}{mathematical sans-serif bold italic small r}%
\UnicodeMathSymbol{"1D668}{\mbfitsanss               }{\mathalpha}{mathematical sans-serif bold italic small s}%
\UnicodeMathSymbol{"1D669}{\mbfitsanst               }{\mathalpha}{mathematical sans-serif bold italic small t}%
\UnicodeMathSymbol{"1D66A}{\mbfitsansu               }{\mathalpha}{mathematical sans-serif bold italic small u}%
\UnicodeMathSymbol{"1D66B}{\mbfitsansv               }{\mathalpha}{mathematical sans-serif bold italic small v}%
\UnicodeMathSymbol{"1D66C}{\mbfitsansw               }{\mathalpha}{mathematical sans-serif bold italic small w}%
\UnicodeMathSymbol{"1D66D}{\mbfitsansx               }{\mathalpha}{mathematical sans-serif bold italic small x}%
\UnicodeMathSymbol{"1D66E}{\mbfitsansy               }{\mathalpha}{mathematical sans-serif bold italic small y}%
\UnicodeMathSymbol{"1D66F}{\mbfitsansz               }{\mathalpha}{mathematical sans-serif bold italic small z}%
\UnicodeMathSymbol{"1D670}{\mttA                     }{\mathalpha}{mathematical monospace capital a}%
\UnicodeMathSymbol{"1D671}{\mttB                     }{\mathalpha}{mathematical monospace capital b}%
\UnicodeMathSymbol{"1D672}{\mttC                     }{\mathalpha}{mathematical monospace capital c}%
\UnicodeMathSymbol{"1D673}{\mttD                     }{\mathalpha}{mathematical monospace capital d}%
\UnicodeMathSymbol{"1D674}{\mttE                     }{\mathalpha}{mathematical monospace capital e}%
\UnicodeMathSymbol{"1D675}{\mttF                     }{\mathalpha}{mathematical monospace capital f}%
\UnicodeMathSymbol{"1D676}{\mttG                     }{\mathalpha}{mathematical monospace capital g}%
\UnicodeMathSymbol{"1D677}{\mttH                     }{\mathalpha}{mathematical monospace capital h}%
\UnicodeMathSymbol{"1D678}{\mttI                     }{\mathalpha}{mathematical monospace capital i}%
\UnicodeMathSymbol{"1D679}{\mttJ                     }{\mathalpha}{mathematical monospace capital j}%
\UnicodeMathSymbol{"1D67A}{\mttK                     }{\mathalpha}{mathematical monospace capital k}%
\UnicodeMathSymbol{"1D67B}{\mttL                     }{\mathalpha}{mathematical monospace capital l}%
\UnicodeMathSymbol{"1D67C}{\mttM                     }{\mathalpha}{mathematical monospace capital m}%
\UnicodeMathSymbol{"1D67D}{\mttN                     }{\mathalpha}{mathematical monospace capital n}%
\UnicodeMathSymbol{"1D67E}{\mttO                     }{\mathalpha}{mathematical monospace capital o}%
\UnicodeMathSymbol{"1D67F}{\mttP                     }{\mathalpha}{mathematical monospace capital p}%
\UnicodeMathSymbol{"1D680}{\mttQ                     }{\mathalpha}{mathematical monospace capital q}%
\UnicodeMathSymbol{"1D681}{\mttR                     }{\mathalpha}{mathematical monospace capital r}%
\UnicodeMathSymbol{"1D682}{\mttS                     }{\mathalpha}{mathematical monospace capital s}%
\UnicodeMathSymbol{"1D683}{\mttT                     }{\mathalpha}{mathematical monospace capital t}%
\UnicodeMathSymbol{"1D684}{\mttU                     }{\mathalpha}{mathematical monospace capital u}%
\UnicodeMathSymbol{"1D685}{\mttV                     }{\mathalpha}{mathematical monospace capital v}%
\UnicodeMathSymbol{"1D686}{\mttW                     }{\mathalpha}{mathematical monospace capital w}%
\UnicodeMathSymbol{"1D687}{\mttX                     }{\mathalpha}{mathematical monospace capital x}%
\UnicodeMathSymbol{"1D688}{\mttY                     }{\mathalpha}{mathematical monospace capital y}%
\UnicodeMathSymbol{"1D689}{\mttZ                     }{\mathalpha}{mathematical monospace capital z}%
\UnicodeMathSymbol{"1D68A}{\mtta                     }{\mathalpha}{mathematical monospace small a}%
\UnicodeMathSymbol{"1D68B}{\mttb                     }{\mathalpha}{mathematical monospace small b}%
\UnicodeMathSymbol{"1D68C}{\mttc                     }{\mathalpha}{mathematical monospace small c}%
\UnicodeMathSymbol{"1D68D}{\mttd                     }{\mathalpha}{mathematical monospace small d}%
\UnicodeMathSymbol{"1D68E}{\mtte                     }{\mathalpha}{mathematical monospace small e}%
\UnicodeMathSymbol{"1D68F}{\mttf                     }{\mathalpha}{mathematical monospace small f}%
\UnicodeMathSymbol{"1D690}{\mttg                     }{\mathalpha}{mathematical monospace small g}%
\UnicodeMathSymbol{"1D691}{\mtth                     }{\mathalpha}{mathematical monospace small h}%
\UnicodeMathSymbol{"1D692}{\mtti                     }{\mathalpha}{mathematical monospace small i}%
\UnicodeMathSymbol{"1D693}{\mttj                     }{\mathalpha}{mathematical monospace small j}%
\UnicodeMathSymbol{"1D694}{\mttk                     }{\mathalpha}{mathematical monospace small k}%
\UnicodeMathSymbol{"1D695}{\mttl                     }{\mathalpha}{mathematical monospace small l}%
\UnicodeMathSymbol{"1D696}{\mttm                     }{\mathalpha}{mathematical monospace small m}%
\UnicodeMathSymbol{"1D697}{\mttn                     }{\mathalpha}{mathematical monospace small n}%
\UnicodeMathSymbol{"1D698}{\mtto                     }{\mathalpha}{mathematical monospace small o}%
\UnicodeMathSymbol{"1D699}{\mttp                     }{\mathalpha}{mathematical monospace small p}%
\UnicodeMathSymbol{"1D69A}{\mttq                     }{\mathalpha}{mathematical monospace small q}%
\UnicodeMathSymbol{"1D69B}{\mttr                     }{\mathalpha}{mathematical monospace small r}%
\UnicodeMathSymbol{"1D69C}{\mtts                     }{\mathalpha}{mathematical monospace small s}%
\UnicodeMathSymbol{"1D69D}{\mttt                     }{\mathalpha}{mathematical monospace small t}%
\UnicodeMathSymbol{"1D69E}{\mttu                     }{\mathalpha}{mathematical monospace small u}%
\UnicodeMathSymbol{"1D69F}{\mttv                     }{\mathalpha}{mathematical monospace small v}%
\UnicodeMathSymbol{"1D6A0}{\mttw                     }{\mathalpha}{mathematical monospace small w}%
\UnicodeMathSymbol{"1D6A1}{\mttx                     }{\mathalpha}{mathematical monospace small x}%
\UnicodeMathSymbol{"1D6A2}{\mtty                     }{\mathalpha}{mathematical monospace small y}%
\UnicodeMathSymbol{"1D6A3}{\mttz                     }{\mathalpha}{mathematical monospace small z}%
\UnicodeMathSymbol{"1D6A4}{\imath                    }{\mathalpha}{mathematical italic small dotless i}%
\UnicodeMathSymbol{"1D6A5}{\jmath                    }{\mathalpha}{mathematical italic small dotless j}%
\UnicodeMathSymbol{"1D6A8}{\mbfAlpha                 }{\mathalpha}{mathematical bold capital alpha}%
\UnicodeMathSymbol{"1D6A9}{\mbfBeta                  }{\mathalpha}{mathematical bold capital beta}%
\UnicodeMathSymbol{"1D6AA}{\mbfGamma                 }{\mathalpha}{mathematical bold capital gamma}%
\UnicodeMathSymbol{"1D6AB}{\mbfDelta                 }{\mathalpha}{mathematical bold capital delta}%
\UnicodeMathSymbol{"1D6AC}{\mbfEpsilon               }{\mathalpha}{mathematical bold capital epsilon}%
\UnicodeMathSymbol{"1D6AD}{\mbfZeta                  }{\mathalpha}{mathematical bold capital zeta}%
\UnicodeMathSymbol{"1D6AE}{\mbfEta                   }{\mathalpha}{mathematical bold capital eta}%
\UnicodeMathSymbol{"1D6AF}{\mbfTheta                 }{\mathalpha}{mathematical bold capital theta}%
\UnicodeMathSymbol{"1D6B0}{\mbfIota                  }{\mathalpha}{mathematical bold capital iota}%
\UnicodeMathSymbol{"1D6B1}{\mbfKappa                 }{\mathalpha}{mathematical bold capital kappa}%
\UnicodeMathSymbol{"1D6B2}{\mbfLambda                }{\mathalpha}{mathematical bold capital lambda}%
\UnicodeMathSymbol{"1D6B3}{\mbfMu                    }{\mathalpha}{mathematical bold capital mu}%
\UnicodeMathSymbol{"1D6B4}{\mbfNu                    }{\mathalpha}{mathematical bold capital nu}%
\UnicodeMathSymbol{"1D6B5}{\mbfXi                    }{\mathalpha}{mathematical bold capital xi}%
\UnicodeMathSymbol{"1D6B6}{\mbfOmicron               }{\mathalpha}{mathematical bold capital omicron}%
\UnicodeMathSymbol{"1D6B7}{\mbfPi                    }{\mathalpha}{mathematical bold capital pi}%
\UnicodeMathSymbol{"1D6B8}{\mbfRho                   }{\mathalpha}{mathematical bold capital rho}%
\UnicodeMathSymbol{"1D6B9}{\mbfvarTheta              }{\mathalpha}{mathematical bold capital theta symbol}%
\UnicodeMathSymbol{"1D6BA}{\mbfSigma                 }{\mathalpha}{mathematical bold capital sigma}%
\UnicodeMathSymbol{"1D6BB}{\mbfTau                   }{\mathalpha}{mathematical bold capital tau}%
\UnicodeMathSymbol{"1D6BC}{\mbfUpsilon               }{\mathalpha}{mathematical bold capital upsilon}%
\UnicodeMathSymbol{"1D6BD}{\mbfPhi                   }{\mathalpha}{mathematical bold capital phi}%
\UnicodeMathSymbol{"1D6BE}{\mbfChi                   }{\mathalpha}{mathematical bold capital chi}%
\UnicodeMathSymbol{"1D6BF}{\mbfPsi                   }{\mathalpha}{mathematical bold capital psi}%
\UnicodeMathSymbol{"1D6C0}{\mbfOmega                 }{\mathalpha}{mathematical bold capital omega}%
\UnicodeMathSymbol{"1D6C1}{\mbfnabla                 }{\mathalpha}{mathematical bold nabla}%
\UnicodeMathSymbol{"1D6C2}{\mbfalpha                 }{\mathalpha}{mathematical bold small alpha}%
\UnicodeMathSymbol{"1D6C3}{\mbfbeta                  }{\mathalpha}{mathematical bold small beta}%
\UnicodeMathSymbol{"1D6C4}{\mbfgamma                 }{\mathalpha}{mathematical bold small gamma}%
\UnicodeMathSymbol{"1D6C5}{\mbfdelta                 }{\mathalpha}{mathematical bold small delta}%
\UnicodeMathSymbol{"1D6C6}{\mbfvarepsilon            }{\mathalpha}{mathematical bold small varepsilon    }%
\UnicodeMathSymbol{"1D6C7}{\mbfzeta                  }{\mathalpha}{mathematical bold small zeta}%
\UnicodeMathSymbol{"1D6C8}{\mbfeta                   }{\mathalpha}{mathematical bold small eta}%
\UnicodeMathSymbol{"1D6C9}{\mbftheta                 }{\mathalpha}{mathematical bold small theta}%
\UnicodeMathSymbol{"1D6CA}{\mbfiota                  }{\mathalpha}{mathematical bold small iota}%
\UnicodeMathSymbol{"1D6CB}{\mbfkappa                 }{\mathalpha}{mathematical bold small kappa}%
\UnicodeMathSymbol{"1D6CC}{\mbflambda                }{\mathalpha}{mathematical bold small lambda}%
\UnicodeMathSymbol{"1D6CD}{\mbfmu                    }{\mathalpha}{mathematical bold small mu}%
\UnicodeMathSymbol{"1D6CE}{\mbfnu                    }{\mathalpha}{mathematical bold small nu}%
\UnicodeMathSymbol{"1D6CF}{\mbfxi                    }{\mathalpha}{mathematical bold small xi}%
\UnicodeMathSymbol{"1D6D0}{\mbfomicron               }{\mathalpha}{mathematical bold small omicron}%
\UnicodeMathSymbol{"1D6D1}{\mbfpi                    }{\mathalpha}{mathematical bold small pi}%
\UnicodeMathSymbol{"1D6D2}{\mbfrho                   }{\mathalpha}{mathematical bold small rho}%
\UnicodeMathSymbol{"1D6D3}{\mbfvarsigma              }{\mathalpha}{mathematical bold small final sigma}%
\UnicodeMathSymbol{"1D6D4}{\mbfsigma                 }{\mathalpha}{mathematical bold small sigma}%
\UnicodeMathSymbol{"1D6D5}{\mbftau                   }{\mathalpha}{mathematical bold small tau}%
\UnicodeMathSymbol{"1D6D6}{\mbfupsilon               }{\mathalpha}{mathematical bold small upsilon}%
\UnicodeMathSymbol{"1D6D7}{\mbfvarphi                }{\mathalpha}{mathematical bold small phi}%
\UnicodeMathSymbol{"1D6D8}{\mbfchi                   }{\mathalpha}{mathematical bold small chi}%
\UnicodeMathSymbol{"1D6D9}{\mbfpsi                   }{\mathalpha}{mathematical bold small psi}%
\UnicodeMathSymbol{"1D6DA}{\mbfomega                 }{\mathalpha}{mathematical bold small omega}%
\UnicodeMathSymbol{"1D6DB}{\mbfpartial               }{\mathalpha}{mathematical bold partial differential}%
\UnicodeMathSymbol{"1D6DC}{\mbfepsilon               }{\mathalpha}{mathematical bold varepsilon     symbol}%
\UnicodeMathSymbol{"1D6DD}{\mbfvartheta              }{\mathalpha}{mathematical bold theta symbol}%
\UnicodeMathSymbol{"1D6DE}{\mbfvarkappa              }{\mathalpha}{mathematical bold kappa symbol}%
\UnicodeMathSymbol{"1D6DF}{\mbfphi                   }{\mathalpha}{mathematical bold phi symbol}%
\UnicodeMathSymbol{"1D6E0}{\mbfvarrho                }{\mathalpha}{mathematical bold rho symbol}%
\UnicodeMathSymbol{"1D6E1}{\mbfvarpi                 }{\mathalpha}{mathematical bold pi symbol}%
\UnicodeMathSymbol{"1D6E2}{\mitAlpha                 }{\mathalpha}{mathematical italic capital alpha}%
\UnicodeMathSymbol{"1D6E3}{\mitBeta                  }{\mathalpha}{mathematical italic capital beta}%
\UnicodeMathSymbol{"1D6E4}{\mitGamma                 }{\mathalpha}{mathematical italic capital gamma}%
\UnicodeMathSymbol{"1D6E5}{\mitDelta                 }{\mathalpha}{mathematical italic capital delta}%
\UnicodeMathSymbol{"1D6E6}{\mitEpsilon               }{\mathalpha}{mathematical italic capital epsilon}%
\UnicodeMathSymbol{"1D6E7}{\mitZeta                  }{\mathalpha}{mathematical italic capital zeta}%
\UnicodeMathSymbol{"1D6E8}{\mitEta                   }{\mathalpha}{mathematical italic capital eta}%
\UnicodeMathSymbol{"1D6E9}{\mitTheta                 }{\mathalpha}{mathematical italic capital theta}%
\UnicodeMathSymbol{"1D6EA}{\mitIota                  }{\mathalpha}{mathematical italic capital iota}%
\UnicodeMathSymbol{"1D6EB}{\mitKappa                 }{\mathalpha}{mathematical italic capital kappa}%
\UnicodeMathSymbol{"1D6EC}{\mitLambda                }{\mathalpha}{mathematical italic capital lambda}%
\UnicodeMathSymbol{"1D6ED}{\mitMu                    }{\mathalpha}{mathematical italic capital mu}%
\UnicodeMathSymbol{"1D6EE}{\mitNu                    }{\mathalpha}{mathematical italic capital nu}%
\UnicodeMathSymbol{"1D6EF}{\mitXi                    }{\mathalpha}{mathematical italic capital xi}%
\UnicodeMathSymbol{"1D6F0}{\mitOmicron               }{\mathalpha}{mathematical italic capital omicron}%
\UnicodeMathSymbol{"1D6F1}{\mitPi                    }{\mathalpha}{mathematical italic capital pi}%
\UnicodeMathSymbol{"1D6F2}{\mitRho                   }{\mathalpha}{mathematical italic capital rho}%
\UnicodeMathSymbol{"1D6F3}{\mitvarTheta              }{\mathalpha}{mathematical italic capital theta symbol}%
\UnicodeMathSymbol{"1D6F4}{\mitSigma                 }{\mathalpha}{mathematical italic capital sigma}%
\UnicodeMathSymbol{"1D6F5}{\mitTau                   }{\mathalpha}{mathematical italic capital tau}%
\UnicodeMathSymbol{"1D6F6}{\mitUpsilon               }{\mathalpha}{mathematical italic capital upsilon}%
\UnicodeMathSymbol{"1D6F7}{\mitPhi                   }{\mathalpha}{mathematical italic capital phi}%
\UnicodeMathSymbol{"1D6F8}{\mitChi                   }{\mathalpha}{mathematical italic capital chi}%
\UnicodeMathSymbol{"1D6F9}{\mitPsi                   }{\mathalpha}{mathematical italic capital psi}%
\UnicodeMathSymbol{"1D6FA}{\mitOmega                 }{\mathalpha}{mathematical italic capital omega}%
\UnicodeMathSymbol{"1D6FB}{\mitnabla                 }{\mathalpha}{mathematical italic nabla}%
\UnicodeMathSymbol{"1D6FC}{\mitalpha                 }{\mathalpha}{mathematical italic small alpha}%
\UnicodeMathSymbol{"1D6FD}{\mitbeta                  }{\mathalpha}{mathematical italic small beta}%
\UnicodeMathSymbol{"1D6FE}{\mitgamma                 }{\mathalpha}{mathematical italic small gamma}%
\UnicodeMathSymbol{"1D6FF}{\mitdelta                 }{\mathalpha}{mathematical italic small delta}%
\UnicodeMathSymbol{"1D700}{\mitvarepsilon            }{\mathalpha}{mathematical italic small varepsilon    }%
\UnicodeMathSymbol{"1D701}{\mitzeta                  }{\mathalpha}{mathematical italic small zeta}%
\UnicodeMathSymbol{"1D702}{\miteta                   }{\mathalpha}{mathematical italic small eta}%
\UnicodeMathSymbol{"1D703}{\mittheta                 }{\mathalpha}{mathematical italic small theta}%
\UnicodeMathSymbol{"1D704}{\mitiota                  }{\mathalpha}{mathematical italic small iota}%
\UnicodeMathSymbol{"1D705}{\mitkappa                 }{\mathalpha}{mathematical italic small kappa}%
\UnicodeMathSymbol{"1D706}{\mitlambda                }{\mathalpha}{mathematical italic small lambda}%
\UnicodeMathSymbol{"1D707}{\mitmu                    }{\mathalpha}{mathematical italic small mu}%
\UnicodeMathSymbol{"1D708}{\mitnu                    }{\mathalpha}{mathematical italic small nu}%
\UnicodeMathSymbol{"1D709}{\mitxi                    }{\mathalpha}{mathematical italic small xi}%
\UnicodeMathSymbol{"1D70A}{\mitomicron               }{\mathalpha}{mathematical italic small omicron}%
\UnicodeMathSymbol{"1D70B}{\mitpi                    }{\mathalpha}{mathematical italic small pi}%
\UnicodeMathSymbol{"1D70C}{\mitrho                   }{\mathalpha}{mathematical italic small rho}%
\UnicodeMathSymbol{"1D70D}{\mitvarsigma              }{\mathalpha}{mathematical italic small final sigma}%
\UnicodeMathSymbol{"1D70E}{\mitsigma                 }{\mathalpha}{mathematical italic small sigma}%
\UnicodeMathSymbol{"1D70F}{\mittau                   }{\mathalpha}{mathematical italic small tau}%
\UnicodeMathSymbol{"1D710}{\mitupsilon               }{\mathalpha}{mathematical italic small upsilon}%
\UnicodeMathSymbol{"1D711}{\mitvarphi                }{\mathalpha}{mathematical italic small phi}%
\UnicodeMathSymbol{"1D712}{\mitchi                   }{\mathalpha}{mathematical italic small chi}%
\UnicodeMathSymbol{"1D713}{\mitpsi                   }{\mathalpha}{mathematical italic small psi}%
\UnicodeMathSymbol{"1D714}{\mitomega                 }{\mathalpha}{mathematical italic small omega}%
\UnicodeMathSymbol{"1D715}{\mitpartial               }{\mathalpha}{mathematical italic partial differential}%
\UnicodeMathSymbol{"1D716}{\mitepsilon               }{\mathalpha}{mathematical italic varepsilon     symbol}%
\UnicodeMathSymbol{"1D717}{\mitvartheta              }{\mathalpha}{mathematical italic theta symbol}%
\UnicodeMathSymbol{"1D718}{\mitvarkappa              }{\mathalpha}{mathematical italic kappa symbol}%
\UnicodeMathSymbol{"1D719}{\mitphi                   }{\mathalpha}{mathematical italic phi symbol}%
\UnicodeMathSymbol{"1D71A}{\mitvarrho                }{\mathalpha}{mathematical italic rho symbol}%
\UnicodeMathSymbol{"1D71B}{\mitvarpi                 }{\mathalpha}{mathematical italic pi symbol}%
\UnicodeMathSymbol{"1D71C}{\mbfitAlpha               }{\mathalpha}{mathematical bold italic capital alpha}%
\UnicodeMathSymbol{"1D71D}{\mbfitBeta                }{\mathalpha}{mathematical bold italic capital beta}%
\UnicodeMathSymbol{"1D71E}{\mbfitGamma               }{\mathalpha}{mathematical bold italic capital gamma}%
\UnicodeMathSymbol{"1D71F}{\mbfitDelta               }{\mathalpha}{mathematical bold italic capital delta}%
\UnicodeMathSymbol{"1D720}{\mbfitEpsilon             }{\mathalpha}{mathematical bold italic capital epsilon}%
\UnicodeMathSymbol{"1D721}{\mbfitZeta                }{\mathalpha}{mathematical bold italic capital zeta}%
\UnicodeMathSymbol{"1D722}{\mbfitEta                 }{\mathalpha}{mathematical bold italic capital eta}%
\UnicodeMathSymbol{"1D723}{\mbfitTheta               }{\mathalpha}{mathematical bold italic capital theta}%
\UnicodeMathSymbol{"1D724}{\mbfitIota                }{\mathalpha}{mathematical bold italic capital iota}%
\UnicodeMathSymbol{"1D725}{\mbfitKappa               }{\mathalpha}{mathematical bold italic capital kappa}%
\UnicodeMathSymbol{"1D726}{\mbfitLambda              }{\mathalpha}{mathematical bold italic capital lambda}%
\UnicodeMathSymbol{"1D727}{\mbfitMu                  }{\mathalpha}{mathematical bold italic capital mu}%
\UnicodeMathSymbol{"1D728}{\mbfitNu                  }{\mathalpha}{mathematical bold italic capital nu}%
\UnicodeMathSymbol{"1D729}{\mbfitXi                  }{\mathalpha}{mathematical bold italic capital xi}%
\UnicodeMathSymbol{"1D72A}{\mbfitOmicron             }{\mathalpha}{mathematical bold italic capital omicron}%
\UnicodeMathSymbol{"1D72B}{\mbfitPi                  }{\mathalpha}{mathematical bold italic capital pi}%
\UnicodeMathSymbol{"1D72C}{\mbfitRho                 }{\mathalpha}{mathematical bold italic capital rho}%
\UnicodeMathSymbol{"1D72D}{\mbfitvarTheta            }{\mathalpha}{mathematical bold italic capital theta symbol}%
\UnicodeMathSymbol{"1D72E}{\mbfitSigma               }{\mathalpha}{mathematical bold italic capital sigma}%
\UnicodeMathSymbol{"1D72F}{\mbfitTau                 }{\mathalpha}{mathematical bold italic capital tau}%
\UnicodeMathSymbol{"1D730}{\mbfitUpsilon             }{\mathalpha}{mathematical bold italic capital upsilon}%
\UnicodeMathSymbol{"1D731}{\mbfitPhi                 }{\mathalpha}{mathematical bold italic capital phi}%
\UnicodeMathSymbol{"1D732}{\mbfitChi                 }{\mathalpha}{mathematical bold italic capital chi}%
\UnicodeMathSymbol{"1D733}{\mbfitPsi                 }{\mathalpha}{mathematical bold italic capital psi}%
\UnicodeMathSymbol{"1D734}{\mbfitOmega               }{\mathalpha}{mathematical bold italic capital omega}%
\UnicodeMathSymbol{"1D735}{\mbfitnabla               }{\mathalpha}{mathematical bold italic nabla}%
\UnicodeMathSymbol{"1D736}{\mbfitalpha               }{\mathalpha}{mathematical bold italic small alpha}%
\UnicodeMathSymbol{"1D737}{\mbfitbeta                }{\mathalpha}{mathematical bold italic small beta}%
\UnicodeMathSymbol{"1D738}{\mbfitgamma               }{\mathalpha}{mathematical bold italic small gamma}%
\UnicodeMathSymbol{"1D739}{\mbfitdelta               }{\mathalpha}{mathematical bold italic small delta}%
\UnicodeMathSymbol{"1D73A}{\mbfitvarepsilon          }{\mathalpha}{mathematical bold italic small varepsilon    }%
\UnicodeMathSymbol{"1D73B}{\mbfitzeta                }{\mathalpha}{mathematical bold italic small zeta}%
\UnicodeMathSymbol{"1D73C}{\mbfiteta                 }{\mathalpha}{mathematical bold italic small eta}%
\UnicodeMathSymbol{"1D73D}{\mbfittheta               }{\mathalpha}{mathematical bold italic small theta}%
\UnicodeMathSymbol{"1D73E}{\mbfitiota                }{\mathalpha}{mathematical bold italic small iota}%
\UnicodeMathSymbol{"1D73F}{\mbfitkappa               }{\mathalpha}{mathematical bold italic small kappa}%
\UnicodeMathSymbol{"1D740}{\mbfitlambda              }{\mathalpha}{mathematical bold italic small lambda}%
\UnicodeMathSymbol{"1D741}{\mbfitmu                  }{\mathalpha}{mathematical bold italic small mu}%
\UnicodeMathSymbol{"1D742}{\mbfitnu                  }{\mathalpha}{mathematical bold italic small nu}%
\UnicodeMathSymbol{"1D743}{\mbfitxi                  }{\mathalpha}{mathematical bold italic small xi}%
\UnicodeMathSymbol{"1D744}{\mbfitomicron             }{\mathalpha}{mathematical bold italic small omicron}%
\UnicodeMathSymbol{"1D745}{\mbfitpi                  }{\mathalpha}{mathematical bold italic small pi}%
\UnicodeMathSymbol{"1D746}{\mbfitrho                 }{\mathalpha}{mathematical bold italic small rho}%
\UnicodeMathSymbol{"1D747}{\mbfitvarsigma            }{\mathalpha}{mathematical bold italic small final sigma}%
\UnicodeMathSymbol{"1D748}{\mbfitsigma               }{\mathalpha}{mathematical bold italic small sigma}%
\UnicodeMathSymbol{"1D749}{\mbfittau                 }{\mathalpha}{mathematical bold italic small tau}%
\UnicodeMathSymbol{"1D74A}{\mbfitupsilon             }{\mathalpha}{mathematical bold italic small upsilon}%
\UnicodeMathSymbol{"1D74B}{\mbfitvarphi              }{\mathalpha}{mathematical bold italic small phi}%
\UnicodeMathSymbol{"1D74C}{\mbfitchi                 }{\mathalpha}{mathematical bold italic small chi}%
\UnicodeMathSymbol{"1D74D}{\mbfitpsi                 }{\mathalpha}{mathematical bold italic small psi}%
\UnicodeMathSymbol{"1D74E}{\mbfitomega               }{\mathalpha}{mathematical bold italic small omega}%
\UnicodeMathSymbol{"1D74F}{\mbfitpartial             }{\mathalpha}{mathematical bold italic partial differential}%
\UnicodeMathSymbol{"1D750}{\mbfitepsilon             }{\mathalpha}{mathematical bold italic varepsilon     symbol}%
\UnicodeMathSymbol{"1D751}{\mbfitvartheta            }{\mathalpha}{mathematical bold italic theta symbol}%
\UnicodeMathSymbol{"1D752}{\mbfitvarkappa            }{\mathalpha}{mathematical bold italic kappa symbol}%
\UnicodeMathSymbol{"1D753}{\mbfitphi                 }{\mathalpha}{mathematical bold italic phi symbol}%
\UnicodeMathSymbol{"1D754}{\mbfitvarrho              }{\mathalpha}{mathematical bold italic rho symbol}%
\UnicodeMathSymbol{"1D755}{\mbfitvarpi               }{\mathalpha}{mathematical bold italic pi symbol}%
\UnicodeMathSymbol{"1D756}{\mbfsansAlpha             }{\mathalpha}{mathematical sans-serif bold capital alpha}%
\UnicodeMathSymbol{"1D757}{\mbfsansBeta              }{\mathalpha}{mathematical sans-serif bold capital beta}%
\UnicodeMathSymbol{"1D758}{\mbfsansGamma             }{\mathalpha}{mathematical sans-serif bold capital gamma}%
\UnicodeMathSymbol{"1D759}{\mbfsansDelta             }{\mathalpha}{mathematical sans-serif bold capital delta}%
\UnicodeMathSymbol{"1D75A}{\mbfsansEpsilon           }{\mathalpha}{mathematical sans-serif bold capital epsilon}%
\UnicodeMathSymbol{"1D75B}{\mbfsansZeta              }{\mathalpha}{mathematical sans-serif bold capital zeta}%
\UnicodeMathSymbol{"1D75C}{\mbfsansEta               }{\mathalpha}{mathematical sans-serif bold capital eta}%
\UnicodeMathSymbol{"1D75D}{\mbfsansTheta             }{\mathalpha}{mathematical sans-serif bold capital theta}%
\UnicodeMathSymbol{"1D75E}{\mbfsansIota              }{\mathalpha}{mathematical sans-serif bold capital iota}%
\UnicodeMathSymbol{"1D75F}{\mbfsansKappa             }{\mathalpha}{mathematical sans-serif bold capital kappa}%
\UnicodeMathSymbol{"1D760}{\mbfsansLambda            }{\mathalpha}{mathematical sans-serif bold capital lambda}%
\UnicodeMathSymbol{"1D761}{\mbfsansMu                }{\mathalpha}{mathematical sans-serif bold capital mu}%
\UnicodeMathSymbol{"1D762}{\mbfsansNu                }{\mathalpha}{mathematical sans-serif bold capital nu}%
\UnicodeMathSymbol{"1D763}{\mbfsansXi                }{\mathalpha}{mathematical sans-serif bold capital xi}%
\UnicodeMathSymbol{"1D764}{\mbfsansOmicron           }{\mathalpha}{mathematical sans-serif bold capital omicron}%
\UnicodeMathSymbol{"1D765}{\mbfsansPi                }{\mathalpha}{mathematical sans-serif bold capital pi}%
\UnicodeMathSymbol{"1D766}{\mbfsansRho               }{\mathalpha}{mathematical sans-serif bold capital rho}%
\UnicodeMathSymbol{"1D767}{\mbfsansvarTheta          }{\mathalpha}{mathematical sans-serif bold capital theta symbol}%
\UnicodeMathSymbol{"1D768}{\mbfsansSigma             }{\mathalpha}{mathematical sans-serif bold capital sigma}%
\UnicodeMathSymbol{"1D769}{\mbfsansTau               }{\mathalpha}{mathematical sans-serif bold capital tau}%
\UnicodeMathSymbol{"1D76A}{\mbfsansUpsilon           }{\mathalpha}{mathematical sans-serif bold capital upsilon}%
\UnicodeMathSymbol{"1D76B}{\mbfsansPhi               }{\mathalpha}{mathematical sans-serif bold capital phi}%
\UnicodeMathSymbol{"1D76C}{\mbfsansChi               }{\mathalpha}{mathematical sans-serif bold capital chi}%
\UnicodeMathSymbol{"1D76D}{\mbfsansPsi               }{\mathalpha}{mathematical sans-serif bold capital psi}%
\UnicodeMathSymbol{"1D76E}{\mbfsansOmega             }{\mathalpha}{mathematical sans-serif bold capital omega}%
\UnicodeMathSymbol{"1D76F}{\mbfsansnabla             }{\mathalpha}{mathematical sans-serif bold nabla}%
\UnicodeMathSymbol{"1D770}{\mbfsansalpha             }{\mathalpha}{mathematical sans-serif bold small alpha}%
\UnicodeMathSymbol{"1D771}{\mbfsansbeta              }{\mathalpha}{mathematical sans-serif bold small beta}%
\UnicodeMathSymbol{"1D772}{\mbfsansgamma             }{\mathalpha}{mathematical sans-serif bold small gamma}%
\UnicodeMathSymbol{"1D773}{\mbfsansdelta             }{\mathalpha}{mathematical sans-serif bold small delta}%
\UnicodeMathSymbol{"1D774}{\mbfsansvarepsilon        }{\mathalpha}{mathematical sans-serif bold small varepsilon    }%
\UnicodeMathSymbol{"1D775}{\mbfsanszeta              }{\mathalpha}{mathematical sans-serif bold small zeta}%
\UnicodeMathSymbol{"1D776}{\mbfsanseta               }{\mathalpha}{mathematical sans-serif bold small eta}%
\UnicodeMathSymbol{"1D777}{\mbfsanstheta             }{\mathalpha}{mathematical sans-serif bold small theta}%
\UnicodeMathSymbol{"1D778}{\mbfsansiota              }{\mathalpha}{mathematical sans-serif bold small iota}%
\UnicodeMathSymbol{"1D779}{\mbfsanskappa             }{\mathalpha}{mathematical sans-serif bold small kappa}%
\UnicodeMathSymbol{"1D77A}{\mbfsanslambda            }{\mathalpha}{mathematical sans-serif bold small lambda}%
\UnicodeMathSymbol{"1D77B}{\mbfsansmu                }{\mathalpha}{mathematical sans-serif bold small mu}%
\UnicodeMathSymbol{"1D77C}{\mbfsansnu                }{\mathalpha}{mathematical sans-serif bold small nu}%
\UnicodeMathSymbol{"1D77D}{\mbfsansxi                }{\mathalpha}{mathematical sans-serif bold small xi}%
\UnicodeMathSymbol{"1D77E}{\mbfsansomicron           }{\mathalpha}{mathematical sans-serif bold small omicron}%
\UnicodeMathSymbol{"1D77F}{\mbfsanspi                }{\mathalpha}{mathematical sans-serif bold small pi}%
\UnicodeMathSymbol{"1D780}{\mbfsansrho               }{\mathalpha}{mathematical sans-serif bold small rho}%
\UnicodeMathSymbol{"1D781}{\mbfsansvarsigma          }{\mathalpha}{mathematical sans-serif bold small final sigma}%
\UnicodeMathSymbol{"1D782}{\mbfsanssigma             }{\mathalpha}{mathematical sans-serif bold small sigma}%
\UnicodeMathSymbol{"1D783}{\mbfsanstau               }{\mathalpha}{mathematical sans-serif bold small tau}%
\UnicodeMathSymbol{"1D784}{\mbfsansupsilon           }{\mathalpha}{mathematical sans-serif bold small upsilon}%
\UnicodeMathSymbol{"1D785}{\mbfsansvarphi            }{\mathalpha}{mathematical sans-serif bold small phi}%
\UnicodeMathSymbol{"1D786}{\mbfsanschi               }{\mathalpha}{mathematical sans-serif bold small chi}%
\UnicodeMathSymbol{"1D787}{\mbfsanspsi               }{\mathalpha}{mathematical sans-serif bold small psi}%
\UnicodeMathSymbol{"1D788}{\mbfsansomega             }{\mathalpha}{mathematical sans-serif bold small omega}%
\UnicodeMathSymbol{"1D789}{\mbfsanspartial           }{\mathalpha}{mathematical sans-serif bold partial differential}%
\UnicodeMathSymbol{"1D78A}{\mbfsansepsilon           }{\mathalpha}{mathematical sans-serif bold varepsilon     symbol}%
\UnicodeMathSymbol{"1D78B}{\mbfsansvartheta          }{\mathalpha}{mathematical sans-serif bold theta symbol}%
\UnicodeMathSymbol{"1D78C}{\mbfsansvarkappa          }{\mathalpha}{mathematical sans-serif bold kappa symbol}%
\UnicodeMathSymbol{"1D78D}{\mbfsansphi               }{\mathalpha}{mathematical sans-serif bold phi symbol}%
\UnicodeMathSymbol{"1D78E}{\mbfsansvarrho            }{\mathalpha}{mathematical sans-serif bold rho symbol}%
\UnicodeMathSymbol{"1D78F}{\mbfsansvarpi             }{\mathalpha}{mathematical sans-serif bold pi symbol}%
\UnicodeMathSymbol{"1D790}{\mbfitsansAlpha           }{\mathalpha}{mathematical sans-serif bold italic capital alpha}%
\UnicodeMathSymbol{"1D791}{\mbfitsansBeta            }{\mathalpha}{mathematical sans-serif bold italic capital beta}%
\UnicodeMathSymbol{"1D792}{\mbfitsansGamma           }{\mathalpha}{mathematical sans-serif bold italic capital gamma}%
\UnicodeMathSymbol{"1D793}{\mbfitsansDelta           }{\mathalpha}{mathematical sans-serif bold italic capital delta}%
\UnicodeMathSymbol{"1D794}{\mbfitsansEpsilon         }{\mathalpha}{mathematical sans-serif bold italic capital epsilon}%
\UnicodeMathSymbol{"1D795}{\mbfitsansZeta            }{\mathalpha}{mathematical sans-serif bold italic capital zeta}%
\UnicodeMathSymbol{"1D796}{\mbfitsansEta             }{\mathalpha}{mathematical sans-serif bold italic capital eta}%
\UnicodeMathSymbol{"1D797}{\mbfitsansTheta           }{\mathalpha}{mathematical sans-serif bold italic capital theta}%
\UnicodeMathSymbol{"1D798}{\mbfitsansIota            }{\mathalpha}{mathematical sans-serif bold italic capital iota}%
\UnicodeMathSymbol{"1D799}{\mbfitsansKappa           }{\mathalpha}{mathematical sans-serif bold italic capital kappa}%
\UnicodeMathSymbol{"1D79A}{\mbfitsansLambda          }{\mathalpha}{mathematical sans-serif bold italic capital lambda}%
\UnicodeMathSymbol{"1D79B}{\mbfitsansMu              }{\mathalpha}{mathematical sans-serif bold italic capital mu}%
\UnicodeMathSymbol{"1D79C}{\mbfitsansNu              }{\mathalpha}{mathematical sans-serif bold italic capital nu}%
\UnicodeMathSymbol{"1D79D}{\mbfitsansXi              }{\mathalpha}{mathematical sans-serif bold italic capital xi}%
\UnicodeMathSymbol{"1D79E}{\mbfitsansOmicron         }{\mathalpha}{mathematical sans-serif bold italic capital omicron}%
\UnicodeMathSymbol{"1D79F}{\mbfitsansPi              }{\mathalpha}{mathematical sans-serif bold italic capital pi}%
\UnicodeMathSymbol{"1D7A0}{\mbfitsansRho             }{\mathalpha}{mathematical sans-serif bold italic capital rho}%
\UnicodeMathSymbol{"1D7A1}{\mbfitsansvarTheta        }{\mathalpha}{mathematical sans-serif bold italic capital theta symbol}%
\UnicodeMathSymbol{"1D7A2}{\mbfitsansSigma           }{\mathalpha}{mathematical sans-serif bold italic capital sigma}%
\UnicodeMathSymbol{"1D7A3}{\mbfitsansTau             }{\mathalpha}{mathematical sans-serif bold italic capital tau}%
\UnicodeMathSymbol{"1D7A4}{\mbfitsansUpsilon         }{\mathalpha}{mathematical sans-serif bold italic capital upsilon}%
\UnicodeMathSymbol{"1D7A5}{\mbfitsansPhi             }{\mathalpha}{mathematical sans-serif bold italic capital phi}%
\UnicodeMathSymbol{"1D7A6}{\mbfitsansChi             }{\mathalpha}{mathematical sans-serif bold italic capital chi}%
\UnicodeMathSymbol{"1D7A7}{\mbfitsansPsi             }{\mathalpha}{mathematical sans-serif bold italic capital psi}%
\UnicodeMathSymbol{"1D7A8}{\mbfitsansOmega           }{\mathalpha}{mathematical sans-serif bold italic capital omega}%
\UnicodeMathSymbol{"1D7A9}{\mbfitsansnabla           }{\mathalpha}{mathematical sans-serif bold italic nabla}%
\UnicodeMathSymbol{"1D7AA}{\mbfitsansalpha           }{\mathalpha}{mathematical sans-serif bold italic small alpha}%
\UnicodeMathSymbol{"1D7AB}{\mbfitsansbeta            }{\mathalpha}{mathematical sans-serif bold italic small beta}%
\UnicodeMathSymbol{"1D7AC}{\mbfitsansgamma           }{\mathalpha}{mathematical sans-serif bold italic small gamma}%
\UnicodeMathSymbol{"1D7AD}{\mbfitsansdelta           }{\mathalpha}{mathematical sans-serif bold italic small delta}%
\UnicodeMathSymbol{"1D7AE}{\mbfitsansvarepsilon      }{\mathalpha}{mathematical sans-serif bold italic small varepsilon    }%
\UnicodeMathSymbol{"1D7AF}{\mbfitsanszeta            }{\mathalpha}{mathematical sans-serif bold italic small zeta}%
\UnicodeMathSymbol{"1D7B0}{\mbfitsanseta             }{\mathalpha}{mathematical sans-serif bold italic small eta}%
\UnicodeMathSymbol{"1D7B1}{\mbfitsanstheta           }{\mathalpha}{mathematical sans-serif bold italic small theta}%
\UnicodeMathSymbol{"1D7B2}{\mbfitsansiota            }{\mathalpha}{mathematical sans-serif bold italic small iota}%
\UnicodeMathSymbol{"1D7B3}{\mbfitsanskappa           }{\mathalpha}{mathematical sans-serif bold italic small kappa}%
\UnicodeMathSymbol{"1D7B4}{\mbfitsanslambda          }{\mathalpha}{mathematical sans-serif bold italic small lambda}%
\UnicodeMathSymbol{"1D7B5}{\mbfitsansmu              }{\mathalpha}{mathematical sans-serif bold italic small mu}%
\UnicodeMathSymbol{"1D7B6}{\mbfitsansnu              }{\mathalpha}{mathematical sans-serif bold italic small nu}%
\UnicodeMathSymbol{"1D7B7}{\mbfitsansxi              }{\mathalpha}{mathematical sans-serif bold italic small xi}%
\UnicodeMathSymbol{"1D7B8}{\mbfitsansomicron         }{\mathalpha}{mathematical sans-serif bold italic small omicron}%
\UnicodeMathSymbol{"1D7B9}{\mbfitsanspi              }{\mathalpha}{mathematical sans-serif bold italic small pi}%
\UnicodeMathSymbol{"1D7BA}{\mbfitsansrho             }{\mathalpha}{mathematical sans-serif bold italic small rho}%
\UnicodeMathSymbol{"1D7BB}{\mbfitsansvarsigma        }{\mathalpha}{mathematical sans-serif bold italic small final sigma}%
\UnicodeMathSymbol{"1D7BC}{\mbfitsanssigma           }{\mathalpha}{mathematical sans-serif bold italic small sigma}%
\UnicodeMathSymbol{"1D7BD}{\mbfitsanstau             }{\mathalpha}{mathematical sans-serif bold italic small tau}%
\UnicodeMathSymbol{"1D7BE}{\mbfitsansupsilon         }{\mathalpha}{mathematical sans-serif bold italic small upsilon}%
\UnicodeMathSymbol{"1D7BF}{\mbfitsansvarphi          }{\mathalpha}{mathematical sans-serif bold italic small phi}%
\UnicodeMathSymbol{"1D7C0}{\mbfitsanschi             }{\mathalpha}{mathematical sans-serif bold italic small chi}%
\UnicodeMathSymbol{"1D7C1}{\mbfitsanspsi             }{\mathalpha}{mathematical sans-serif bold italic small psi}%
\UnicodeMathSymbol{"1D7C2}{\mbfitsansomega           }{\mathalpha}{mathematical sans-serif bold italic small omega}%
\UnicodeMathSymbol{"1D7C3}{\mbfitsanspartial         }{\mathalpha}{mathematical sans-serif bold italic partial differential}%
\UnicodeMathSymbol{"1D7C4}{\mbfitsansepsilon         }{\mathalpha}{mathematical sans-serif bold italic varepsilon     symbol}%
\UnicodeMathSymbol{"1D7C5}{\mbfitsansvartheta        }{\mathalpha}{mathematical sans-serif bold italic theta symbol}%
\UnicodeMathSymbol{"1D7C6}{\mbfitsansvarkappa        }{\mathalpha}{mathematical sans-serif bold italic kappa symbol}%
\UnicodeMathSymbol{"1D7C7}{\mbfitsansphi             }{\mathalpha}{mathematical sans-serif bold italic phi symbol}%
\UnicodeMathSymbol{"1D7C8}{\mbfitsansvarrho          }{\mathalpha}{mathematical sans-serif bold italic rho symbol}%
\UnicodeMathSymbol{"1D7C9}{\mbfitsansvarpi           }{\mathalpha}{mathematical sans-serif bold italic pi symbol}%
\UnicodeMathSymbol{"1D7CA}{\mbfDigamma               }{\mathalpha}{mathematical bold capital digamma}%
\UnicodeMathSymbol{"1D7CB}{\mbfdigamma               }{\mathalpha}{mathematical bold small digamma}%
\UnicodeMathSymbol{"1D7CE}{\mbfzero                  }{\mathord}{mathematical bold digit 0}%
\UnicodeMathSymbol{"1D7CF}{\mbfone                   }{\mathord}{mathematical bold digit 1}%
\UnicodeMathSymbol{"1D7D0}{\mbftwo                   }{\mathord}{mathematical bold digit 2}%
\UnicodeMathSymbol{"1D7D1}{\mbfthree                 }{\mathord}{mathematical bold digit 3}%
\UnicodeMathSymbol{"1D7D2}{\mbffour                  }{\mathord}{mathematical bold digit 4}%
\UnicodeMathSymbol{"1D7D3}{\mbffive                  }{\mathord}{mathematical bold digit 5}%
\UnicodeMathSymbol{"1D7D4}{\mbfsix                   }{\mathord}{mathematical bold digit 6}%
\UnicodeMathSymbol{"1D7D5}{\mbfseven                 }{\mathord}{mathematical bold digit 7}%
\UnicodeMathSymbol{"1D7D6}{\mbfeight                 }{\mathord}{mathematical bold digit 8}%
\UnicodeMathSymbol{"1D7D7}{\mbfnine                  }{\mathord}{mathematical bold digit 9}%
\UnicodeMathSymbol{"1D7D8}{\Bbbzero                  }{\mathord}{mathematical double-struck digit 0}%
\UnicodeMathSymbol{"1D7D9}{\Bbbone                   }{\mathord}{mathematical double-struck digit 1}%
\UnicodeMathSymbol{"1D7DA}{\Bbbtwo                   }{\mathord}{mathematical double-struck digit 2}%
\UnicodeMathSymbol{"1D7DB}{\Bbbthree                 }{\mathord}{mathematical double-struck digit 3}%
\UnicodeMathSymbol{"1D7DC}{\Bbbfour                  }{\mathord}{mathematical double-struck digit 4}%
\UnicodeMathSymbol{"1D7DD}{\Bbbfive                  }{\mathord}{mathematical double-struck digit 5}%
\UnicodeMathSymbol{"1D7DE}{\Bbbsix                   }{\mathord}{mathematical double-struck digit 6}%
\UnicodeMathSymbol{"1D7DF}{\Bbbseven                 }{\mathord}{mathematical double-struck digit 7}%
\UnicodeMathSymbol{"1D7E0}{\Bbbeight                 }{\mathord}{mathematical double-struck digit 8}%
\UnicodeMathSymbol{"1D7E1}{\Bbbnine                  }{\mathord}{mathematical double-struck digit 9}%
\UnicodeMathSymbol{"1D7E2}{\msanszero                }{\mathord}{mathematical sans-serif digit 0}%
\UnicodeMathSymbol{"1D7E3}{\msansone                 }{\mathord}{mathematical sans-serif digit 1}%
\UnicodeMathSymbol{"1D7E4}{\msanstwo                 }{\mathord}{mathematical sans-serif digit 2}%
\UnicodeMathSymbol{"1D7E5}{\msansthree               }{\mathord}{mathematical sans-serif digit 3}%
\UnicodeMathSymbol{"1D7E6}{\msansfour                }{\mathord}{mathematical sans-serif digit 4}%
\UnicodeMathSymbol{"1D7E7}{\msansfive                }{\mathord}{mathematical sans-serif digit 5}%
\UnicodeMathSymbol{"1D7E8}{\msanssix                 }{\mathord}{mathematical sans-serif digit 6}%
\UnicodeMathSymbol{"1D7E9}{\msansseven               }{\mathord}{mathematical sans-serif digit 7}%
\UnicodeMathSymbol{"1D7EA}{\msanseight               }{\mathord}{mathematical sans-serif digit 8}%
\UnicodeMathSymbol{"1D7EB}{\msansnine                }{\mathord}{mathematical sans-serif digit 9}%
\UnicodeMathSymbol{"1D7EC}{\mbfsanszero              }{\mathord}{mathematical sans-serif bold digit 0}%
\UnicodeMathSymbol{"1D7ED}{\mbfsansone               }{\mathord}{mathematical sans-serif bold digit 1}%
\UnicodeMathSymbol{"1D7EE}{\mbfsanstwo               }{\mathord}{mathematical sans-serif bold digit 2}%
\UnicodeMathSymbol{"1D7EF}{\mbfsansthree             }{\mathord}{mathematical sans-serif bold digit 3}%
\UnicodeMathSymbol{"1D7F0}{\mbfsansfour              }{\mathord}{mathematical sans-serif bold digit 4}%
\UnicodeMathSymbol{"1D7F1}{\mbfsansfive              }{\mathord}{mathematical sans-serif bold digit 5}%
\UnicodeMathSymbol{"1D7F2}{\mbfsanssix               }{\mathord}{mathematical sans-serif bold digit 6}%
\UnicodeMathSymbol{"1D7F3}{\mbfsansseven             }{\mathord}{mathematical sans-serif bold digit 7}%
\UnicodeMathSymbol{"1D7F4}{\mbfsanseight             }{\mathord}{mathematical sans-serif bold digit 8}%
\UnicodeMathSymbol{"1D7F5}{\mbfsansnine              }{\mathord}{mathematical sans-serif bold digit 9}%
\UnicodeMathSymbol{"1D7F6}{\mttzero                  }{\mathord}{mathematical monospace digit 0}%
\UnicodeMathSymbol{"1D7F7}{\mttone                   }{\mathord}{mathematical monospace digit 1}%
\UnicodeMathSymbol{"1D7F8}{\mtttwo                   }{\mathord}{mathematical monospace digit 2}%
\UnicodeMathSymbol{"1D7F9}{\mttthree                 }{\mathord}{mathematical monospace digit 3}%
\UnicodeMathSymbol{"1D7FA}{\mttfour                  }{\mathord}{mathematical monospace digit 4}%
\UnicodeMathSymbol{"1D7FB}{\mttfive                  }{\mathord}{mathematical monospace digit 5}%
\UnicodeMathSymbol{"1D7FC}{\mttsix                   }{\mathord}{mathematical monospace digit 6}%
\UnicodeMathSymbol{"1D7FD}{\mttseven                 }{\mathord}{mathematical monospace digit 7}%
\UnicodeMathSymbol{"1D7FE}{\mtteight                 }{\mathord}{mathematical monospace digit 8}%
\UnicodeMathSymbol{"1D7FF}{\mttnine                  }{\mathord}{mathematical monospace digit 9}%
\UnicodeMathSymbol{"1EEF0}{\arabicmaj                }{\mathop}{arabic mathematical operator meem with hah with tatweel}%
\UnicodeMathSymbol{"1EEF1}{\arabichad                }{\mathop}{arabic mathematical operator hah with dal}%

% /©
%
% ------------------------------------------------
% The UNICODE-MATH package  <wspr.io/unicode-math>
% ------------------------------------------------
% This package is free software and may be redistributed and/or modified under
% the conditions of the LaTeX Project Public License, version 1.3c or higher
% (your choice): <http://www.latex-project.org/lppl/>.
% ------------------------------------------------
% Copyright 2006-2018  Will Robertson, LPPL "maintainer"
% Copyright 2010-2017  Philipp Stephani
% Copyright 2011-2017  Joseph Wright
% Copyright 2012-2015  Khaled Hosny
% ------------------------------------------------
%
% ©/


